Automating Thinning Theorem: Synthesizing Efficient Dynamic Programming Algorithms

Dynamic programming is an important optimization technique, but designing efficient dynamic programming algorithms can be difficult for even professional programmers. Thinning, a technique developed for systematically deriving efficient dynamic programming algorithms, has received much attention in studies because of its effectiveness for a large class of problems. Despite the success of thinning in theory, its practical usage is still limited because (1) applying thinning requires mathematical and algorithmic background, and (2) applying thinning solely may not be enough to generate algorithms as efficient as proposed by human experts. In this paper, we propose two approaches, MetHyl and MetHyl+, to resolve both problems. First, MetHyl automates the application of thinning via program synthesis and thus eliminates the burden to the user for applying thinning. Second, MetHyl+ integrates three rules into MetHyl that optimize three important factors on the time complexity of dynamic programming algorithms that are ignored by thinning, and thus make it able to automatically generate expert-level dynamic programming algorithms on many tasks. We evaluate our approaches on 37 tasks related to 16 optimization problems collected from Introduction to Algorithm, a popular textbook for algorithm courses. The results show that MetHyl+ achieves exponential speed-ups on 97.3% of tasks with an average time cost of less than one minute. Moreover, MetHyl+ generates algorithms that are as efficient as the reference programs provided by human experts on 70.3% of tasks.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> sections/Background.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Preliminaries} \label{section:background}
In this section, we introduce the background of our paper. 

To operate functions, the following four operators $\circ, +, \times$, and $\triangle$ will be used in the remainder of this paper.
\begin{gather*}
    (f_1 \circ f_2)\ x\coloneqq f_1\ (f_2\ x) \quad (f_1 + f_2)\ (i, x) \coloneqq f_i\ x, i \in \{0, 1\} \\
    (f_1 \times f_2)\ (x, y) \coloneqq (f_1\ x, f_2\ y) \quad (f_1 \triangle f_2) \ x\coloneqq (f_1\ x, f_2\ x)
\end{gather*}
\subsection{Categorical Functors}
\textit{Functor} is an important concept in category theory. A category consists of a set of objects, denoted by uppercase letters such as $A$, and a set of arrows between objects, denoted by lowercase letters such as $f$. In this paper, we focus on category \textbf{Fun}, where an object is a type and arrows from object $A$ to object $B$ includes all total functions mapping $A$ to $B$. 

A functor can be regarded as a higher-order function, which maps objects to objects, arrows to arrows, and keeps both identity and composition.

In a category, a functor $\F$ maps objects to objects, arrows to arrows, and keeps both identity and composition. 
$$
\F id_A = id_{F_A} \qquad \F(f \circ g) = \F f \circ \F g
$$
where $\textit{id}_A$ represents the identity function on set $A$. Intuitively, a functor can be regraded as a higher-order function, which constructs new functions from existing functions.


A functor is a \textit{polynomial functor} if it is constructed by identity functor $\mathsf{I}$, constant functors $!A$, and bifunctors $\times, +$. Their definitions are shown below.
\begin{gather*}
    \mathsf{I}A \coloneqq A\quad \mathsf{I}f \coloneqq f\quad (!A)B \coloneqq A\quad (!A)f \coloneqq id_A \\
    (\F_1 \times \F_2)A \coloneqq \F_1A \times \F_2A \quad (\F_1 + \F_2)f \coloneqq \F_1f + \F_2 f \\
    (\F_1 + \F_2)A \coloneqq (\{1\} \times \F_1A) \cup(\{2\} \times \F_2A) \\ 
    (\F_1 + \F_2)f \coloneqq \F_1 f + \F_2 f
\end{gather*}
where $A \times B$ is the Cartesian product of objects $A$ and $B$.

In this paper, when use symbol $\F$, we inherently assume that $\F$ is polynomial. Besides, we also use the power functor $\mathsf{P}$ to express operations related to power sets.
\begin{align*}
    \mathsf P A \coloneqq \{s\ |\ s \subseteq A\} \quad \mathsf P f\ s \coloneqq \{f\ a\ |\ a \in s\}
\end{align*}

\subsection{Generator, Memoization, and Hylomorphism}
The concept of \textit{relational hylomorphism} originally defined on another category namely \textbf{Rel}. For simplicity, in this paper, we introduce it as its simplified counterpart in category \textbf{Fun}.

\begin{definition}[Recursive Generator] \label{def:rec} Given arrows $\phi: \mathsf {PF}A \rightarrow \mathsf P A$ and $\psi: B \rightarrow \mathsf P\F B$, recursive generator $rg(\phi, \psi)_{\F}: A \rightarrow \mathsf PB$ is the smallest solution of the following equation, where arrow $r_1$ is smaller than $r_2$ if $\forall i, r_1\ i \subseteq r_2\ i$.
    $$
    rg(\phi, \psi)_{\F} = \phi \circ \textit{cup} \circ \mathsf P \textit{car}[\mathsf F] \circ \mathsf {PF}rg(\phi, \psi)_{\F} \circ \psi
    $$
In this equation, $\textit{car}[\F]: \mathsf{FP}A \rightarrow \mathsf{PF}A$ is defined as the following, which operates similarly with the Cartesian product, and $\textit{cup}: \mathsf{PP}A \rightarrow \mathsf{P}A$ is defined as $\textit{cup}\ x \coloneqq \cup_{s \in x} s$, which unions all sets in a set of sets. {\small
\begin{gather*}
\textit{car}[\mathsf I]\ x \coloneqq x \quad
\textit{car}[\F_1 \times \F_2]\ (x_1, x_2) \coloneqq (\textit{car}[\F_1]\ x_1) \times (\textit{car}[\F_2]\ x_2) \\
\textit{car}[!A]\ x \coloneqq x \quad\textit{car}[\F_1 + \F_2]\ (i, x) \coloneqq \{(i, a)\ |\ a \in x\}
\end{gather*}}
\end{definition}

\SetKwFunction{Prog}{Prog}
\begin{figure*}
    \begin{minipage}{.31\linewidth}{
        {\centering
        \removelatexerror
    \begin{algorithm}[H]
        \small
        \caption{\small Program for $rg(\phi, \psi)_{\F}$.}
        \label{alg:rg}
        \LinesNumbered
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{$\Prog\ s$}{
            $\textit{subRes} \gets \emptyset$ \\
            \ForEach{$t \in (\psi\ s)$}{
                $\textit{tRes} \gets \textit{car}[\F]\ (\F \Prog\ t)$; \\
                $\textit{subRes} \gets \textit{subRes} \cup \textit{tRes}$;
            } 
            $\textit{sols} \gets \phi\ \textit{subRes}$; \\
            \Return $\textit{sols}$; 
        }
    \end{algorithm}
    }}
\end{minipage} \ \ 
\begin{minipage}{.32\linewidth}{
    {\centering
    \removelatexerror
\begin{algorithm}[H]
    \small
    \caption{\small Program for $rg(\phi, \psi)_{\F}^{m}$.}
    \label{alg:rgm}
    \LinesNumbered
    \SetKwProg{Fn}{Function}{:}{}
    $\textit{Mem} \gets \emptyset$; \\ 
    \Fn{$\Prog\ s$}{
        $key \gets m\ s$; \\
        \If{$key \in \textit{Mem}$}{\Return $\textit{Mem}[key]$}
        Lines 2-7 in Algorithm \ref{alg:rg}; \\
        $\textit{Mem}[key] \gets \textit{sols}$; \\
        \Return $\textit{sols}$; 
    }
\end{algorithm}
}}
\end{minipage}\ \ \ 
    \begin{minipage}{.31\linewidth}{
        {\centering
        \removelatexerror
    \begin{algorithm}[H]
        \small
        \caption{\small Program for $\hylo{\phi, \psi}_{\F}$.}
        \label{alg:hylo}
        \LinesNumbered
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{$\Prog\ s$}{
            $\textit{sols} \gets \emptyset$ \\
            \ForEach{$t \in (\psi\ s)$}{
                $\textit{tRes} \gets \textit{car}[\F]\ (\F\Prog\ \textit{t})$; \\
                \ForEach{$\textit{res} \gets \textit{tRes}$}{
                    $\textit{sols} \gets \textit{sols} \cup (\phi\ \textit{res})$;
                }
            } 
            \Return $\textit{sols}$; 
        }
    \end{algorithm}
    }}
\end{minipage}
\end{figure*}

The concept of recursive generator corresponds to recursive programs in \textbf{Rel}. Algorithm \ref{alg:rg} shows a program corresponding to $rg(\phi, \psi)$. Given a state $s$, $rg(\phi, \psi)$ invokes $\psi$ to generate a set of \textit{transitions} (Line 3), where each transition may involve several substates. $rg(\phi, \psi)$ recurses into substates via $\F rg(\phi, \psi)$ and partial solutions are combined via $\textit{car}[\F]$ (Line 4). The results of transitions are merged (Line 5), and $\phi$ are invoked to generate solutions for $s$. 

For a recursive program $r$, we use $r^m$ to represent the result of memoizing $r$ via key function $m$. Algorithm \ref{alg:rgm} shows a program corresponding to $rg(\phi, \psi)_{\F}^m$. In this program, input $s$ is related to a memory unit with key $(m\ s)$. For each invocation $rg(\phi, \psi)_{\F}^{m}\ s$, $\textit{Mem}[m\ s]$ will be directly returned if there has been results in it (Lines 4-6). Otherwise, the results of $rg(\phi, \psi)_{\F}^{m}\ s$ will be stored into $\textit{Mem}[m\ s]$ (Line 8).

\begin{definition} [Relational Hylomorphism]\label{def:hylo} Given two arrows $\phi: \mathsf F A\rightarrow \mathsf P A$ and $\psi: B \rightarrow \mathsf P\F B$, relational hylomorphism $\hylo{\phi, \psi}_{\F}: B \rightarrow \mathsf P A$ is defined as $rg(\textit{cup} \circ \mathsf P\phi, \psi)$.
\end{definition}

Algorithm \ref{alg:hylo} shows a program corresponding to $\hylo{\phi, \psi}_{\F}$. $\hylo{\phi, \psi}_{\F}$ invokes $\phi$ to generate solutions for each transition result (Line 6) and returns their union (Line 9).

Relational hylomorphisms are natural for specifying COPs, where $\psi$ and $\phi$ specify the decision procedure and the construction of solutions respectively. However, relational hylomorphism cannot express optimizations (e.g., thinning and branch-and-bound), because it simply returns the union of all possible solutions (Line 6 in Algorithm \ref{alg:hylo}). Therefore, the same as related studies in program calculus, \mainname takes a relational hylomorphism as the input but expresses the internal optimized programs via recursive generators.

\subsection{Programs}
In \mainname, a program is represented by a pair $(P, S)$. Given an instance $i$, the output of $(P, S)$ is equal to $\arg \max (S\ p), p \in (P\ i)$. In terms of solving COPs, two programs are equivalent if they achieve the same objective value.

\begin{definition}[Equivalence] Two programs $(P_1, S_1)$ and $(P_2, S_2)$ are equivalence on instance $i$, denoted as $(P_1,S_1) \sim_{i} (P_2, S_2)$, if $\max(S_1\ p), p \in (P_1\ i) = \max(S_2\ p), p \in (P_2\ i)$.
\end{definition}

In this paper, we provide a simple language $\mathcal L_H$ for specifying COPs via relational hylomorphisms. The syntax of this language is shown as Figure \ref{fig:syntax}.

%In our language, a program is a pair, where the two components correspond to the plan generator, a relational hylomorphism, and the scorer. Given an instance $i$ of a COP, the output of program $(P, S)$ is $\arg \max (S\ p), p \in (P\ i)$. 

Because both functions $\phi, \psi$ in a relational hylomorphism return a set, $\mathcal L_H$ uses |collect| instead of |return| to express this behavior, where each execution of $|\textit{collect}\ e|$ will insert the result of expression $e$ to the returning set.
\begin{figure*}[t]
      \begin{minipage}{.48\linewidth}
        \centering
            {\small
                \begin{tabular}{cccl} 
                    \toprule 
                    Program& $\mathbb P$& $\rightarrow$ & $(\mathbb H, \mathbb E)$ \\
                    Hylomorphism & $\mathbb H$ & $\rightarrow $ & $\hylo{\lambda x. \mathbb S, \lambda x. \mathbb S}_{\mathbb F}$ \\
                    Functor& $\mathbb F$& $\rightarrow$& $\mathsf I\ |\ !\texttt{Void}\ |\ !\texttt{Int}\ |\ \mathbb F \times \mathbb F\ |\ \mathbb F + \mathbb F $ \\
                    Statement & $\mathbb S$ & $\rightarrow$ & $\text{skip};\ |\ \mathbb S\ \mathbb S\ |\ \text{if }\mathbb E\text{ then }\mathbb S\text{ else }\mathbb S$ \\
                    & & $|$ & $\text{collect }\mathbb E;\ |\ \text{foreach }x \in \mathbb E \text{ in }\mathbb S$ \\
                    Expression & $\mathbb E$ & $\rightarrow$ & $x \ |\ \text{const}\ |\ \lambda x. \mathbb E \ |\ \oplus\ \mathbb E\dots\mathbb E$\\
                    \bottomrule
            \end{tabular}}
            \caption{The syntax of language $\mathcal L_H$, where $x$ represents a variable, and $\oplus$ represents a black-box operator.} 
            \label{fig:syntax}\centering
            {\small 
            \begin{align*}
            &\textit{prog}_2 = (\hylo{\phi, \psi}_{\mathsf F}, S), \text{ where }\\
            &\quad\F = !\texttt{Void} + \mathsf I + ((!\texttt{Int} \times !\texttt{Int}) \times \mathsf I) \\
            &\quad \psi = \lambda (is, p). \text{ if }|is| = 0\text{ then collect } (1, \bot); \\
            &\quad \quad \text{else }\{ \text{collect }(2, (\textit{tail}\ is, p));\\
            & \quad \quad \quad \text{if } (\textit{sumw}\ p) + (\textit{head}\ is).1 \leq W \text{ then} \\
            & \quad \quad \quad \quad \text{collect }(3, (\textit{head}\ is, (\textit{tail}\ is, (\textit{head}\ is)::p))); \}\\
            &\quad \phi = \lambda (\textit{tag}, p). \text{if }\textit{tag} = 1\text{ then collect }[]; \\ 
            &\quad \quad \text{else if }\textit{tag} = 2 \text{ then collect }p;\text{ else collect }(p.1::p.2);\\
            &\quad S = \lambda p. \textit{sumv}\ p
            \end{align*}
            }
            \vspace{-17pt}
            \caption{A valid program for 0/1 knapsack in $\mathcal L_H$. The input of $\psi$ is a pair $(is, p)$, where $is$ is the list of remaining items, $p$ is the list of selected items.}
            \label{fig:p2}
      \end{minipage} \quad \quad 
      \begin{minipage}{.4\linewidth}
        \centering
            {\small 
            \begin{align*}
            &\textit{prog} = (\hylo{\phi, \psi}_{\mathsf F}, S), \text{ where }\\
            &\quad\F = !\texttt{Void} + \mathsf I +  ((!\texttt{Int} \times !\texttt{Int}) \times \mathsf I) \\
            &\quad \psi = \lambda is. \text{ if }|is| = 0\text{ then collect } (1, \bot); \\
            &\quad \quad \text{else }\{\text{collect }(2, \textit{tail}\ is);\\\
            & \quad \quad \quad \text{collect } (3, (\textit{head}\ is, \textit{tail}\ is));\}\\
            &\quad \phi = \lambda (\textit{tag}, p). \text{ if }\textit{tag} = 1\text{ then collect } []; \\
            &\quad \quad \text{else if } tag = 2 \text{ then }\text{collect }p.2; \\
            &\quad \quad \text{else if }(\textit{sumw}\ p.2) + p.1.1 \leq W\text{ then} \\
            & \quad \quad \quad \quad \text{collect } (p.1 :: p.2); \\
            &\quad S = \lambda p. \textit{sumv}\ p
            \end{align*}
            }
            \vspace{-17pt}
            \caption{The program corresponding to $(P_1, S_1)$.}
            \label{fig:p1}
            {\small 
            \begin{align*}
            &\textit{prog}_3 = (\hylo{\phi, \psi}_{\mathsf F}, S), \text{ where }\\
            &\quad\F = !\texttt{Void} + ((!\texttt{Int} \times !\texttt{Int}) \times \mathsf I) \\
            &\quad \psi = \lambda is. \text{ if }|is| = 0\text{ then collect } (1, \bot); \\
            &\quad \quad \text{else collect } (2, (\textit{head}\ is, \textit{tail}\ is)); \\
            &\quad \phi = \lambda (\textit{tag}, p). \text{ if }\textit{tag} = 1\text{ then collect } []; \\
            &\quad \quad \text{else }\{\text{collect }(p.1::p.2);\ \text{collect }p.2;\} \\
            & \quad S = \lambda p. (\textit{sumw}\ p \leq W)\ ?\ (\textit{sumv}\ p) :-\infty;
            \end{align*}
            }
            \vspace{-17pt}
            \caption{A valid program for 0/1 knapsack in $\mathcal L_H$. In this program, $-\infty$ is a small enough integer that is used to exclude invalid programs.}
            \label{fig:p3}
      \end{minipage} \\
\end{figure*}

Figure \ref{fig:p1} shows a program \textit{prog} in $\mathcal L_H$ corresponding to program $(P_1, S_1)$ discussed in Section \ref{section:overview}\footnote{For simplicity, we ignore the memoization part (i.e., key function $m_1$) here.}, where operator $+$ is naturally extended to three operands, $|\text{if }\mathbb E \text{ then }$ $\mathbb S \text{ else }\mathbb S$| is a sugar of $|\text{if }\mathbb E \text{ then }\mathbb S \text{ else skip};|$, and $|\lambda (x_1, x_2). \mathbb S$| is a sugar of extracting components in the input for $|\lambda x. \mathbb S|$. 

Note that the program in $\mathcal L_H$ for describing 0/1 knapsack is not unique. Figure \ref{fig:p2} and \ref{fig:p3} show two other valid programs $\textit{prog}_2$ and $\textit{prog}_3$ for 0/1 knapsack. 

\subsection{Thinning}
The definition of thinning is based on \textit{preorders}. A preorder on object $A$ is a relation that is reflexive and transitive. 
$$
\forall a \in A, a R a \quad \forall a,b,c \in A, aRb \wedge bRc \rightarrow aRc
$$

\begin{definition} \label{def:thin}Given a preorder $R$ on $A$, $\textit{thin}\ R: \mathsf PA \rightarrow \mathsf PA$ is an arrow such that for any set $s \subseteq A$, $\textit{thin}\ R\ s$ is the smallest subset of $s$ satisfying $\forall a \in s, \exists b \in \textit{thin}\ R\ s, aRb$.
\end{definition}

One noticeable special case of $\textit{thin}$ is when $R$ is the conjunction of several comparisons on several key functions.

\begin{definition}[Keyword Preorder] A keyword preorder $R$ of comparisons $\{(op_i, k_i)\}$ on $A$ is defined as the following.
    $$
    aRb \iff \wedge_{i} (k_i\ a)\ op_i (k_i\ b)
    $$
where $k_i$ is an arrow from $A$ to $\texttt{Int}$ and $op_i \in \{\leq, =\}$.
\end{definition}

\begin{theorem} \label{theorem:thinning}Given a keyword preorder $R$ of $\{(op_i, k_i)\}$, define function $N_R(s)$ as the following, where $\textit{range}(k, s)$ is the range of  $k$ on set $s$, i.e., $\max_{a \in s}(k\ a) - \min_{a \in s}(k \ a)$, and $\max(s)$ returns the largest element in $s$ with default value $1$.
$$
N_R(s) \coloneqq \left( \prod_{i}\textit{range}(k_i, s)\right) \big/ \max_i\big(\textit{range}(k_i, s)\ \big|\ op_i \in \{\leq\}\big)  
$$
\begin{itemize}[leftmargin=*]
\item For any set $s$, $|\textit{thin}\ R\ s| \leq N_R(s)$.
\item There is an implementation of $(\textit{thin}\ R)$ with time complexity $O(N_R(s)|R| + T_R(s))$, where $s$ is the input set, $T_R(s)$ is the time complexity of evaluating all key functions in $R$ for all elements in $s$.
\end{itemize}
\end{theorem}

\subsection{Lifting and Partial Lifting} 
Lifting problems and partial lifting problems are two classes of synthesis tasks studied by \citet{lifting}. They are generalized from the task of parallelizing a given program.

\begin{definition} \label{def:lifting}Given arrows $p, h$ starting from object $A$, a set $M$ including $n$ arrows $m_i: \mathsf F_{m_i}A \rightarrow A$, and example space $E$ attaching a set of examples $E[m_i]$ to each $m_i \in M$, lifting problem $\mathsf{LP}(M, p, h, E)$ and partial lifting problem $\mathsf{PLP}(M,p,h, E)$ are to find $\red{?f}, \red{?c_1}, \dots, \red{?c_n}$ such that Equation \ref{formula:lp} and \ref{formula:plp} are satisfied for all $m_i \in M$, respectively.
    \begin{gather}
    \forall e \in E[m_i], ((p \triangle \red{?f}) \circ m_i)\ e = (\red{?c_i} \circ \mathsf F_{m_i}(h \triangle \red{?f}))\ e \label{formula:lp}\\
    \forall e \in E[m_i], (p \circ m_i)\ e = (\red{?c_i} \circ \mathsf F_{m_i}(h \triangle \red{?f}))\ e \label{formula:plp}
    \end{gather}
\end{definition}

\textit{AutoLifter}~\cite{lifting} is an efficient synthesizer for these two tasks, which cares only those solutions where the output of $\red{?f}$ is a tuple of scalar values. 

==> sections/Draw.tex <==
%!TEX root = ../Dgoynthesxs.tex
% 80
\begin{figure*}[t]
	\centering

    \begin{align*}
        {\small
    R = \lambda p_1. \lambda p_2. (\textit{sumw}\ p_1 \geq \textit{sumw}\ p_2 \wedge \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2)
        }
    \end{align*}

    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g_1 =  \lambda xs. \text{ if }|xs| = 0\text{ then } [\blue{[]}] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g_1\ (\textit{tail}\ xs)) \cat \\
                &\qquad \quad \big[\blue{(head\ xs)::p}\ \big|\ p \in g_1\ (\textit{tail}\ xs), \\
                &\qquad \quad \qquad (\blue{\textit{sumw}\ p}) + (head\ xs).1 \leq W\big]\big) \\
                &o_1 =  \lambda p. (\blue{\textit{sumv}\ p})\quad m_1 = \lambda xs. xs \\
            & 
            R = \lambda p_1. \lambda p_2. (\blue{\textit{sumw}\ p_1} \geq \blue{\textit{sumw}\ p_2} \wedge\\
            & \qquad \qquad \quad \ \ \blue{\textit{sumv}\ p_1} \leq \blue{\textit{sumv}\ p_2})
            \end{align*}
        }
    \end{minipage} 


    $$ \small
         p \Rightarrow \red{?f_p}\ p
    $$


    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g_1' =  \lambda xs. \text{ if }|xs| = 0\text{ then } [\red{?c_{\bot}}] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g_1'\ (\textit{tail}\ xs)) \cat \\
                &\qquad \quad \big[\red{?c}\ (\textit{head}\ xs)\ p\ \big|\ p \in g_1'\ (\textit{tail}\ xs), \\
                &\qquad \qquad \quad (\red{?q_w}\ p) + (head\ xs).1 \leq W\big]\big) \\
                &o_1' = \lambda p. (\red{?q_v}\ p)\quad m_1' = \lambda xs. xs\\
            &R = \lambda p_1. \lambda p_2. (\red{?q_w}\ p_1 \geq \red{?q_w}\ p_2 \wedge\\ 
            &\qquad \qquad \quad \ \ \red{?q_v}\ p_1 \leq \red{?q_v}\ p_2) \\
            \end{align*}
        }
    \end{minipage} 

    $$ \small
    f_p = \lambda p. (\textit{sumw}\ p, \textit{sumv}\ p)\quad c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) \quad q_w = \lambda p. (p.1) \quad q_v = \lambda p. (p.2)\quad c_\bot = (0, 0)
    $$ 


    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g_2 =  \lambda xs. \text{ if }|xs| = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g_2\ (\textit{tail}\ xs)) \cat \\
                &\qquad \quad \big[c\ (\textit{head}\ xs)\ p\ \big|\ p \in g_2\ (\textit{tail}\ xs),\\ 
                &\qquad \qquad \quad p.1 + (head\ xs).1 \leq W\big]\big) \\
                &o_2 = \lambda p. (p.2) \quad m_2 = \lambda xs. xs\\
            &R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) 
            \end{align*}
        }
    \end{minipage} 

    \begin{align*}
    \textit{buffer}[\red{?f_m}\ xs] 
    \end{align*}
\end{figure*}
 
    \newpage

    \begin{figure*}[t]
        \centering
    $$ \small
    f_m = \lambda xs. |xs| 
    $$

    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g_2' =  \lambda xs. \text{ if }|xs| = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g_2'\ (\textit{tail}\ xs)) \cat \\
                &\qquad \quad \big[c\ (\textit{head}\ xs)\ p\ \big|\ p \in g_2'\ (\textit{tail}\ xs),\\ 
                &\qquad \qquad \quad p.1 + (head\ xs).1 \leq W\big]\big) \\
                &o_2' = \lambda p. (p.2)\quad m_2' = \lambda xs. (\red{?f_m}\
                 xs)\\
            &R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) 
            \end{align*}
        }
    \end{minipage} 
    
    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g_3 =  \lambda xs. \text{ if }\blue{|xs|} = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g_3\ (\blue{\textit{tail}\ xs})) \cat \\
                &\qquad \quad \big[c\ (\blue{\textit{head}\ xs})\ p\ \big|\ p \in g_3\ (\blue{\textit{tail}\ xs}), \\
                &\qquad \quad \qquad p.1 + (\blue{head\ xs}).1 \leq W\big]\big) \\
                &o_3 = \lambda p. (p.2)\quad m_3 = \lambda xs. \blue{|xs|} \\
            &R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2)
            \end{align*}
        }
    \end{minipage} 
    
    $$ \small
    xs \Rightarrow \red{?f_s}\ xs\ (\text{denoted as }i)
    $$
    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g_3' = \lambda i. \text{ if }\red{?ql}\ i = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g_3'\ (\red{?c_t}\ i)) \cat \\
                &\qquad \quad \big[c\ (\red{?q_h}\ i)\ p\ \big|\ p \in g_3'\ (\red{?c_t}\ i),\\
                &\qquad \qquad \quad p.1 + (\red{?q_h}\ i).1 \leq W\big]\big) \\
                &o_3' = \lambda p. (p.2) \quad m_3' = \lambda i. (\red{?q_l}\ i)\\
            &    R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) \quad 
            \end{align*}
        }
    \end{minipage} 

    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &g^* =\  \lambda i. \text{ if }i = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}[R]\ \big((g^*\ (i - 1)) \cat \\
                &\qquad \quad \big[c\ xs[-i]\ p\ \big|\ p \in g^*\ (i - 1),\\
                &\qquad \qquad \quad p.1 + xs[-i].1 \leq W\big]\big) \\
                &o^* = \ \lambda p. (p.2) \quad m^*= \lambda i. i\\
            &    R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) \quad 
            \end{align*}
        }
    \end{minipage} 
    $$\small
    f_s = \lambda xs. |xs| \quad q_l = \lambda i. i \quad q_h = \lambda i. xs[-i] \quad c_t = \lambda i.  (i - 1)
    $$
\end{figure*}
\begin{figure*}
    {\small
    \begin{align*}
    \neg([(2, 3)]\red{?R}[(1, 2)])
    \end{align*}}

    {\small
    \begin{align*}
        \red{?c}\ (3, 3)\ (\red{?f_p}\ [(1, 2)]) \\
        = \red{?f_p}\ [(3, 3), (1, 2)]
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?c_\bot} = \red{?f_p}\ []
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?q_w}\ (\red{?f_p}\ [(1, 2)]) = 1 \\
        \red{?q_v}\ (\red{?f_p}\ [(1, 2)]) = 2
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?f_m}\ [(2, 2), (1, 2)] \\
        \neq \red{?f_m}\ [(1, 2)]
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?f_m}\ [(2, 2), (1, 2)] \\
        \neq \red{?f_m}\ [(1, 2)]
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?q_l}\ (\red{?f_s}\ [(1, 2)]) = 1 \\
        \red{?q_h}\ (\red{?f_s}\ [(1, 2)]) = (1, 2) \\
        \red{?c_t}\ (\red{?f_s}\ [(1, 2)]) = \red{?f_s}\ []
    \end{align*}
    }
\end{figure*}

==> sections/Draw_pre.tex <==
%!TEX root = ../DPSynthesis.tex
% 100
\begin{figure*}[t]
	\centering
    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
            &g_1 =  \lambda g_1. \lambda is. \text{ if }|is| = 0\text{ then } [[]] \\
            & \qquad \text{else } \textit{cat}\ [ \text{if}\ (\textit{sumw}\ f) + (\textit{sumw}\ s) \leq W \\
            &\qquad \quad \big[(head\ is)::p\ \big|\ p \in P_1\ (\textit{tail}\ is), \\
            & \quad \qquad \qquad (\textit{sumw}\ p) + (head\ is).1 \leq W\big] \\
            &S_1 =  \lambda p. (\textit{sumv}\ p)\quad m_1 = \lambda is. is
            \end{align*}
        }
    \end{minipage} 


    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}            
                &P_1' =  \lambda is. \text{ if }|is| = 0\text{ then } [[]] \\
                & \qquad \text{else } \textit{thin}\ \red{?R}\ \big((P_1'\ (\textit{tail}\ is)) \cat \\
                &\qquad \quad \big[(head\ is)::p\ \big|\ p \in P_1'\ (\textit{tail}\ is), \\
                &\qquad \qquad \quad (\textit{sumw}\ p) + (head\ is).1 \leq W\big]\big) \\
                &S_1' =  \lambda p. (\textit{sumv}\ p)\quad m_1' = \lambda is. is
            \end{align*}
        }
    \end{minipage} 

    \begin{align*}
        {\small
    R = \lambda p_1. \lambda p_2. (\textit{sumw}\ p_1 \geq \textit{sumw}\ p_2 \wedge \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2)
        }
    \end{align*}

    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P_2 =  \lambda is. \text{ if }|is| = 0\text{ then } [\green{[]}] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P_2\ (\textit{tail}\ is)) \cat \\
                &\qquad \quad \big[\green{(head\ is)::p}\ \big|\ p \in P_2\ (\textit{tail}\ is), \\
                &\qquad \quad \qquad (\blue{\textit{sumw}\ p}) + (head\ is).1 \leq W\big]\big) \\
                &S_2 =  \lambda p. (\blue{\textit{sumv}\ p})\quad m_2 = \lambda is. is \\
            & 
            R = \lambda p_1. \lambda p_2. (\blue{\textit{sumw}\ p_1} \geq \blue{\textit{sumw}\ p_2} \wedge\\
            & \qquad \qquad \quad \ \ \blue{\textit{sumv}\ p_1} \leq \blue{\textit{sumv}\ p_2})
            \end{align*}
        }
    \end{minipage} 


    $$ \small
         p \Rightarrow \red{?f_p}\ p
    $$


    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P_2' =  \lambda is. \text{ if }|is| = 0\text{ then } [\red{?f_p}\ []] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P_2'\ (\textit{tail}\ is)) \cat \\
                &\qquad \quad \big[\red{?c}\ (\textit{head}\ is)\ p\ \big|\ p \in P_2'\ (\textit{tail}\ is), \\
                &\qquad \qquad \quad (\red{?q_w}\ p) + (head\ is).1 \leq W\big]\big) \\
                &S_2' = \lambda p. (\red{?q_v}\ p)\quad m_2' = \lambda is. is\\
            &R = \lambda p_1. \lambda p_2. (\red{?q_w}\ p_1 \geq \red{?q_w}\ p_2 \wedge\\ 
            &\qquad \qquad \quad \ \ \red{?q_v}\ p_1 \leq \red{?q_v}\ p_2) \\
            \end{align*}
        }
    \end{minipage} 

    $$ \small
    f_p = \lambda p. (\textit{sumw}\ p, \textit{sumv}\ p)\quad c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) \quad q_w = \lambda p. (p.1) \quad q_v = \lambda p. (p.2)
    $$ 


    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P_3 =  \lambda is. \text{ if }|is| = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P_3\ (\textit{tail}\ is)) \cat \\
                &\qquad \quad \big[c\ (\textit{head}\ is)\ p\ \big|\ p \in P_3\ (\textit{tail}\ is),\\ 
                &\qquad \qquad \quad p.1 + (head\ is).1 \leq W\big]\big) \\
                &S_3 = \lambda p. (p.2) \quad m_3 = \lambda is. is\\
            &R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) 
            \end{align*}
        }
    \end{minipage} 

    \begin{align*}
    \textit{Mem}[\red{?f_m}\ is] 
    \end{align*}
\end{figure*}
 
    \newpage

    \begin{figure*}[t]
        \centering
    $$ \small
    f_m = \lambda is. |is| 
    $$

    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P_3' =  \lambda is. \text{ if }|is| = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P_3'\ (\textit{tail}\ is)) \cat \\
                &\qquad \quad \big[c\ (\textit{head}\ is)\ p\ \big|\ p \in P_3'\ (\textit{tail}\ is),\\ 
                &\qquad \qquad \quad p.1 + (head\ is).1 \leq W\big]\big) \\
                &S_3' = \lambda p. (p.2)\quad m_3' = \lambda is. (\red{?f_m}\
                 is)\\
            &R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) 
            \end{align*}
        }
    \end{minipage} 
    
    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P_4 =  \lambda is. \text{ if }\blue{|is|} = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P_4\ (\green{\textit{tail}\ is})) \cat \\
                &\qquad \quad \big[c\ (\blue{\textit{head}\ is})\ p\ \big|\ p \in P_4\ (\green{\textit{tail}\ is}), \\
                &\qquad \quad \qquad p.1 + (\blue{head\ is}).1 \leq W\big]\big) \\
                &S_4 = \lambda p. (p.2)\quad m_4 = \lambda is. \blue{|is|} \\
            &R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2)
            \end{align*}
        }
    \end{minipage} 
    
    $$ \small
    is \Rightarrow \red{?f_s}\ is\ (\text{denoted as }i)
    $$
    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P_4' = \lambda i. \text{ if }\red{?ql}\ i = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P_4'\ (\red{?c_t}\ i)) \cat \\
                &\qquad \quad \big[c\ (\red{?q_h}\ i)\ p\ \big|\ p \in P_4'\ (\red{?c_t}\ i),\\
                &\qquad \qquad \quad p.1 + (\red{?q_h}\ i).1 \leq W\big]\big) \\
                &S_4' = \lambda p. (p.2) \quad m_4' = \lambda i. (\red{?q_l}\ i)\\
            &    R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) \quad 
            \end{align*}
        }
    \end{minipage} 

    \begin{minipage}[h]{0.45\linewidth}
        {
            \small
            \begin{align*}
                &P^* =\  \lambda i. \text{ if }i = 0\text{ then } [(0, 0)] \\
                & \qquad \text{else } \textit{thin}\ R\ \big((P^*\ (i - 1)) \cat \\
                &\qquad \quad \big[c\ is[-i]\ p\ \big|\ p \in P^*\ (i - 1),\\
                &\qquad \qquad \quad p.1 + is[-i].1 \leq W\big]\big) \\
                &S^* = \ \lambda p. (p.2) \quad m^*= \lambda i. i\\
            &    R = \lambda p_1. \lambda p_2. (p_1.1 \geq p_2.1 \wedge p_1.2 \leq p_2.2) \\
            & c = \lambda i. \lambda p. (p .1 + i.1, p.2 + i.2) \quad 
            \end{align*}
        }
    \end{minipage} 

    $$\small
    f_s = \lambda is. |is| \quad q_l = \lambda i. i \quad q_h = \lambda i. is[-i] \quad c_t = \lambda i.  (i - 1)
    $$

    {\small
    \begin{align*}
    \neg([(2, 3)]\red{?R}[(1, 2)])
    \end{align*}}

    {\small
    \begin{align*}
        \red{?c}\ (3, 3)\ (\red{?f_p}\ [(1, 2)]) \\
        = \red{?f_p}\ [(3, 3), (1, 2)]
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?q_w}\ (\red{?f_p}\ [(1, 2)]) = 1 \\
        \red{?q_v}\ (\red{?f_p}\ [(1, 2)]) = 2
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?f_m}\ [(2, 3), (1, 2)] \\
        \neq \red{?f_m}\ [(1, 2)]
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?f_m}\ [(2, 3), (1, 2)] \\
        \neq \red{?f_m}\ [(1, 2)]
    \end{align*}
    }
    {\small
    \begin{align*}
        \red{?q_l}\ (\red{?f_s}\ [(1, 2)]) = 1 \\
        \red{?q_h}\ (\red{?f_s}\ [(1, 2)]) = (1, 2) \\
        \red{?c_t}\ (\red{?f_s}\ [(1, 2)]) = \red{?f_s}\ []
    \end{align*}
    }
\end{figure*}

==> sections/Evaluation.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Evaluation} \label{section:evaluation}
%To evaluate \mainname, we design an experiment to answer the following two research questions.
Our evaluation answers two research questions.
\begin{itemize}[leftmargin=*]
\item \textbf{RQ1}: How is the overall performance of \mainname?
\item \textbf{RQ2}: How do the transformation steps in \mainname perform?
\end{itemize}

\subsection{Dataset}
Our evaluation is conducted on a dataset including $37$ input programs for $17$ different COPs. Besides problem \textit{0/1 knapsack} discussed in Section \ref{section:overview}, the other COPs are collected from \textit{Introduction to Algorithms}~\cite{cormen2009introduction}, a widely-used textbook for algorithm courses. This book introduces dynamic programming in its 15th chapter with $4$ example COPs and provides $12$ other COPs as the exercise. We include all these $16$ COPs in our dataset.

To construct input programs, we divide the COPs into two categories according to whether solutions are constrained. 

The first category includes COPs where solutions are not constrained. A representative COP here is \textit{rod cutting}, which is the first example in \textit{Introduction to Algorithms}. 
\begin{center}
    \it
    Known that a rod of length $i$ worth $w_i$, the task is to cut a rod of length $n$ into several pieces and maximize the total value.
\end{center}
In this task, all possible ways to cut the rod are valid solutions. For each COP in this category (7 in total), we implement an input program as natural, where the generator $g$ generates all solutions and the scorer $o$ calculates the objective value.

The second category includes COPs where solutions are constrained. A representative COP is \textit{0/1 knapsack}, where a solution is valid only when the total weight is no more than the capacity. For each COP in this category (10 in total), we implement three input programs $(g = \hylo{\phi, \psi}_{\F}, o)$ according to three extreme principles, which correspond to the three programs in Figures
~\ref{fig:p2}, \ref{fig:p1}, \ref{fig:p3}, respectively.
\begin{itemize}[leftmargin=*]
\item The first program keeps all information in the input of $\psi$ and filters out invalid solutions while deciding transitions.
\item The second program tries all possibilities of constructing solutions in $\psi$ and lets $\phi$ filter out invalid ones.
\item The last program uses $g$ to generate all solutions and excludes invalid ones via a small enough objective value.
\end{itemize}
% For \textit{0/1 knapsack}, these three programs are $\textit{prog}_2$ in Figure \ref{fig:p2}, \textit{prog} in Figure \ref{fig:p1}, and $\textit{prog}_3$ in Figure \ref{fig:p3} respectively.

\subsection{Experiment Setup}
We run \mainname on all $37$ tasks in the dataset and set a time limit of $120$ seconds for each step in \mainname. If a step in \mainname times out, \mainname skips this step and goes on to the next. For each execution, we record the time cost and the transformation result for each step in \mainname. 

\subsection{RQ1: Overall Performance of \mainname} \label{section:rq1}
\newcommand{\tc}[1]{\tilde O({#1})}
\begin{table*}[t]
	\caption{The overall performance of \mainname on all tasks in the dataset.}
    \renewcommand\arraystretch{1.1}
	\begin{spacing}{1}
		\small

        \begin{threeparttable}
		\begin{tabular}{|c|c|c|c|c!{\vrule width 1.5pt}c|c|c|c| c!{\vrule width 1.5pt}c|c|c|c|c|}
			\Xhline{1pt}
            \hline
            COP & Imp & $T_{\text{inp}}$ & $T_{\text{res}}$ & $\text{Time} (s)$ & COP & Imp & $T_{\text{inp}}$ & $T_{\text{res}}$ & $\text{Time} (s)$& COP & Imp & $T_{\text{inp}}$ & $T_{\text{res}}$ & $\text{Time} (s)$\\
            \hline
            \Xhline{1pt}
            \multirow{2}{*}{0/1} & 1 & \multirow{3}{*}{$2^n$} & \multirow{3}{*}{$n^2$}& $25.9$& \multicolumn{2}{c|}{15-3} & $2^n$ & $n^3\dag$ & $133.4$& \multirow{3}{*}{15-8} & 1 & $2^n$&$n^2$  &$31.3$\\
            \cline{2-2} \cline{5-10} \cline{12-15}
            \multirow{2}{*}{Knapsack}& 2 & & & $11.9$& \multirow{3}{*}{15-4}& 1 & \multirow{3}{*}{$2^n$}& \multirow{3}{*}{$n^3\dag$}& $141.4$& & 2 & \multirow{2}{*}{$n^n$}& \multirow{2}{*}{$n^3\dag$} & $25.5$\\
            \cline{2-2} \cline{5-5} \cline{7-7} \cline{10-10} \cline{12-12} \cline{15-15}
            & 3 & & & $23.8$& & 2&& & $240.5$& & 3 & & & $12.1$\\
            \cline{1-3} \cline{4-5} \cline{7-7} \cline{10-15} 
            \multicolumn{2}{|c|}{Rod Cutting} & $2^n$&$n^{2}$ & $18.4$& & 3& & & $240.5$& \multicolumn{2}{c|}{15-9} & $4^n$& $n^3$ & $4.8$\\
            \hline 
            \multicolumn{2}{|c|}{Matrix Chain} & $4^n$& $n^{3}$& $15.4$& \multirow{3}{*}{15-5} & 1 & \multirow{2}{*}{$7.6^n$}& \multirow{2}{*}{$n^2$}& $40.1$& \multicolumn{2}{c|}{15-10} & $n^n$ & $n^4 \dag$ & $34.1$\\
            \cline{1-3} \cline{4-5} \cline{7-7} \cline{10-15}
            \multirow{3}{*}{LCS} & 1 & \multirow{3}{*}{$5.8^n$} & \multirow{3}{*}{$n^{2}$}& $6.9$& & 2 & & & $41.3$& \multirow{3}{*}{15-11} & 1 & \multirow{3}{*}{$n^n$} & \multirow{1}{*}{$n^3$} & $142.0$\\
            \cline{2-2} \cline{5-5} \cline{7-8} \cline{9-10} \cline{12-12} \cline{14-15}
            & 2& & &$5.9$ & & 3 & \multicolumn{2}{c|}{$ \approx7.6^n\dag\ddag$}& $274.9$& & 2 & & \multirow{2}{*}{$n^4\dag$}& $137.5$\\
            \cline{2-2} \cline{5-10} \cline{12-12} \cline{15-15}
            &3& & & $24.3$& \multirow{3}{*}{15-6} & 1 & \multirow{3}{*}{$2^n$} & \multirow{3}{*}{$n$} & $41.2$& & 3 & &  & $137.1$\\
            \cline{1-5} \cline{7-7} \cline{10-15}
            \multicolumn{2}{|c|}{Optimal BST} & $4^n$ & $n^3$& $24.5$& & 2 & & &$28.1$ & \multirow{3}{*}{15-12} & 1 & \multirow{3}{*}{$n^n$} & \multirow{3}{*}{$n^3$} & $54.9$
            \\
            \cline{1-5} \cline{7-7} \cline{10-10} \cline{12-12} \cline{15-15}
            \multicolumn{2}{|c|}{15-1} & $2^n$& $n^{4}\dag$ & $123.7$& & 3 & & & $31.4$& & 2 & & & $27.6$\\
            \cline{1-3} \cline{4-10} \cline{12-12} \cline{15-15}
            \multirow{3}{*}{15-2} & 1 & \multirow{3}{*}{$2^n$}&\multirow{3}{*}{$n^2$} &$8.7$ & \multirow{3}{*}{15-7} & 1 & \multirow{3}{*}{$n^n$}& \multirow{3}{*}{$n^3$} & $3.6$& & 3 & & & $31.6$\\
            \cline{2-2} \cline{5-5} \cline{7-7} \cline{10-15} \Xcline{11-15}{1pt}
            & 2& & & $5.6$& & 2 & & & $10.5$& \multicolumn{5}{l}{
            }\\
            \cline{2-2} \cline{5-5} \cline{7-7} \cline{10-10}
            &3& & & $20.9$& & 3 & & & $8.9$& \multicolumn{5}{c}{}\\
            \cline{1-10}
            \Xcline{1-10}{1pt}
		\end{tabular}
        \begin{tablenotes}[para]
        \small
          %\item[1] The time complexities of the input with memoization $k = \lambda s. s$ and the result are $\tilde \Omega(T_{\text{inp}})$ and $O(T_{\text{res}})$ respectively.\yxcomment{please remove this item.}\\
          \item[\dag] The result does not achieve the same time complexity as the reference algorithm for the corresponding COP.
          \item[\ddag] The time complexities of both programs are $\tilde \Theta(a^n)$, where $\sqrt a \approx 2.77$ is the largest real root of $x^4 - 2x^3 -2x^2 - 1$.
        \end{tablenotes}
    \end{threeparttable}
    \label{table:rq1}
	\end{spacing}
\end{table*}
We manually verify the results of \mainname and confirm that all synthesized programs are completely correct. The performance of \mainname is summarized in Table \ref{table:rq1}. For each problem, \textit{COP} lists its name as in \textit{Introduction to Algorithm}, \textit{Imp} lists the index of the principle if the problem is in the second category, $T_{\textit{inp}}$ lists the time complexity of the input program in $\tilde \Omega$ notation, $T_{\textit{res}}$ lists the time complexity of the result program in $O$ notation, and \textit{Time} lists the total time used by \mainname.
%\begin{itemize}[leftmargin=*]
%\item Column \textit{COP} lists the names of the problems, where 15-$i$ represents the $i$th exercise in Chapter 15 used by \textit{Introduction to Algorithm}.
%\item For each COP in the second category, \textit{Imp} presents the index of the principle used while constructing the input.
%\item \textit{Time} presents the total time used by \mainname. 
%\end{itemize}

Table \ref{table:rq1} demonstrates both the effectiveness and efficiency of \mainname. On effectiveness, \mainname achieves exponential speed-ups against the input program on $36$ out of $37$ tasks, accounting for $97.3\%$. Besides, we compare the synthesis results with the reference algorithms provided by \textit{Introduction to Algorithm} and a solution to its exercises~\cite{algsolutions}, and find that \mainname achieves the same complexity on $26$ out of $37$ tasks, accounting for $70.3\%$. On efficiency, the average time cost of \mainname to process a program is only $59.2$ seconds.

\mainname fails in achieving the same complexity as the reference algorithms on $11$ tasks because of three reasons.

For task (15-5, 3), \mainname fails because the scorer in this task provides little information. In COP 15-5, a solution is a sequence of editions, and a solution is valid if the results of these editions are equal to the target. In this sense, almost all partial solutions are invalid, on which the scorer in (15-5, 3) simply returns $-\infty$. At this time, \mainname can hardly extract examples for $\red{?R}$ and thus fails in the first step. Therefore, the number of solutions remains exponential in the result.

For tasks (15-8, 2) and (15-8, 3), \mainname fails because of useless transitions. %$\psi$ generates too many useless transitions. 
In both tasks, $\psi$ generates $O(n)$ transitions but %the number of transitions that can lead to valid solutions is always at most $2$. 
only $O(1)$ among them can lead to valid solutions.
However, as \mainname does not change the recursive structure, this non-optimal performance remains in the result and thus leads to extra time costs. Optimizing the recursive structure of hylomorphism is future work.

For the other $8$ tasks, \mainname fails because of the enumerative solver. Because the scalability of \textit{observational equivalence} is limited, \mainname times out in Step 2 and 4 when the target program is a complex non-linear program, e.g., $x_1 - \text{dis}(p_1, p_2) + \text{dis}(p_1, p_3) + \text{dis}(p_2, p_3)$ in Task 15-3, where $\text{dis}(p,q)$ is the abbreviation of $(p.x-q.x)^2 + (p.y-q.y)^2$. This fact shows that the effectiveness of \mainname can be further improved by designing efficient solvers for synthesizing $\red{?c}$.

\subsection{RQ2: Performance of Transformation Steps}
\begin{table}[t]
	\caption{The performance of each transformation step.}
    \renewcommand\arraystretch{1.1}
	\begin{spacing}{1}
		\small
		\begin{tabular}{|c|c|c|c|c!{\vrule width 1.5pt}c|c|c|c|c|}
			\Xhline{1pt}
            \hline
            ID& Exp & Poly & $\bot$ & Time & ID& Exp & Poly & $\bot$ & Time \\
			\Xhline{1pt}
            \hline
            1 & $31$& $0$&$1$ & $4.2$  &$2$ & $0$& $3$& $7$&$32.8$\\
            \hline
            3 & $5$& $0$ & $0$& $5.1$ & 4& $0$& $24$& $3$&$59.2$\\
            \hline
            \Xhline{1pt}
		\end{tabular}
    \label{table:rq2}
	\end{spacing}
\end{table}
We manually analyze all intermediate results of \mainname and confirm that on our dataset, all four steps in the transformation system never increase the time complexity. The performance of each step is summarized in Table \ref{table:rq2}. For each step, \textit{ID} lists the index, \textit{Exp} lists the number of tasks on which the step achieves an exponential speed-up, \textit{Poly} lists the number of tasks on which the step achieves a polynomial speed-up, $\bot$ lists the number of failed tasks, and \textit{Time} records the average time cost (seconds) on all tasks.

According to Table \ref{table:rq2}, Step 1 and 3 produce all exponential speed-ups, while Step 2 and 4 produce all polynomial ones. This result matches the target of each step, where the number of solutions (Step 1) and states (Step 3) can be exponential and their scales (Step 2 and 4) are usually polynomial.

Note that the effects of Step 2 and 3 seem to be insignificant in Table \ref{table:rq2} because they are usually \textit{delayed} by Step 4. In many cases, the time cost of operating states forms a bottleneck of the time complexity and thus the effects of Step 2 and 3 will not be revealed until Step 4 is finished. For instance, in the example discussed in Section \ref{section:overview}, %the time costs of operating solutions, performing memoization, and operating states are all $O(n^3)$, 
% and thus the overall time complexity will not change until all the three steps are finished.
Steps 2, 3, and 4 each reduces an $O(n)$ component to $O(1)$, but the overall time complexity would not change if any of the components remains.


==> sections/Implementation.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Implementation} \label{section:implementation}
% Due to the space limit, we introduce our implementation in brief. A more detailed description and our implementation can be found in the supplementary material.
Our implementation is available online~\cite{appendix}.

\noindent \textbf{Generating instances}. In \mainname, a set of instances is required to (1) extract examples for each synthesis task, and (2) evaluate the efficiency of synthesized preorders.

\mainname generates instances by sampling. It describes an instance space by assigning each integer with a range and each recursive data structure with an upperbound on the size. Given such a space, \mainname samples instances according to a uniform distribution. 

To limit the time cost of executing the input program, \mainname decides this space by iteratively squeezing from a default space until the time cost of the input program on a random instance is smaller than a threshold.

\noindent \textbf{Verifying the result}. Due to the complexity of the synthesis result, which involves self-recursion, data structures, and memoization, it is difficult to verify the complete correctness. In our implementation, we use an iterative verifier proposed by \citet{lifting} and guarantee that the probability for the generation error of the synthesis result to be more than $10^{-3}$ is at most $1.82 \times 10^{-4}$.

\noindent \textbf{Grammar}. \mainname uses a grammar to describe the space of possible synthesis results. In our implementation, we extended the CLIA grammar in SyGuS-Comp~\cite{padhisygus} with the following operators related to lists and binary trees.
\begin{itemize}[leftmargin=*]
\item Accumulate operator \textit{fold} and lambda expressions.
\item Access operators \textit{access} for lists, and \textit{value}, \textit{lchild}, \textit{rchild}, \textit{isleaf} for binary trees.
\item Match operator \textit{match} for lists and binary trees, which returns the first occurrence of a sublist (subtree) on a given list (tree). This operator is useful in Step 4, which can correspond the search state to some global data structure.
\end{itemize}

\noindent \textbf{Others}. The original implementation of \textit{AutoLifter} uses \textit{PolyGen}~\cite{DBLP:journals/pacmpl/JiXXH21}, a specialized solver for conditional linear expressions, is used to synthesize $\red{?c}$ for lifting problems. Therefore, in our implementation, when the input program uses non-linear operators, we will replace \textit{PolyGen} with a SOTA enumerative solver, \textit{observational equivalence}~\cite{DBLP:conf/pldi/UdupaRDMMA13}, to make \textit{AutoLifter} applicable.

To implement the preorder synthesizer introduced in Section \ref{section:psolver}, we set $n_c^*$ to $2$ and $s_c^*$ to $10^{5}$, which are enough for most known tasks, and set $n_t$ to $8$, which ensures that the error rate of $\CC$ is at most $e^{-1} \approx 37\%$.

==> sections/Introduction.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Introduction} \label{section:introduction}
\textit{Combinatorial Optimization} is a topic on finding the optimal plan from a finite set of valid plans. Problems of combinatorial optimization widely exists in many domains. In general, such a problem can be expressed via the following template. 
\begin{equation}opt = \lambda i. \big(\arg \max (S\ p), p \in (P\ i)\big)\label{equation:opt-spec}\end{equation}
where program $P$ is a \textit{plan generator} that constructs possible plans for input $i$, and function $S$ is a \textit{scorer} that calculates the objective function for each valid plan.

\textit{Memoization}, or \textit{Dynamic Programming}, is an important technique for combinatorial optimization. It stores the results of expensive function calls and directly returns the cached results when the same inputs occur again. With memoization, the time cost of a recursive function call can be greatly reduced if the number of different inputs are limited, sometimes from exponential-time to polynomial-time. 

However, it is usually difficult to find an efficient scheme for memoization. Let us take a classical problem \textit{0/1 Knapsack}~\cite{mathews1896partition} as an example. 
\begin{center}
    \it
    Given a set of items, each with a value $v_i$ and a weight $w_i$, put a subset of them in a knapsack of capacity $W$ to get the maximum total value in the knapsack.
\end{center}
Figure \ref{fig:1a} shows one possible specification $(P, S)$ for 0/1 knapsack. Given a list $is$ of items, plan generator $P$ finds all the sub-lists of $x$ where the weight sum is no more than $W$, and scorer $S$ calculates the value sum for each plan. Because the number of valid plans is exponential to the number of items, directly memoizing the results of $P$ is still inefficient. 

Figure \ref{fig:1b} shows a more efficient scheme $(P', S')$. Comparing with $(P, S)$, there are two major differences. 
\begin{itemize}[leftmargin=*] 
\item $P'$ takes an integer as the input, representing the number of remaining items, and stores only the weight sum and the value sum for each plan. In this way, time-consuming calculations in $(P, S)$, such as $\textit{sumw}\ p$ are eliminated.
\item $P'$ reduce the number of plans via \textit{thin}'. Though the number of plans returned by each invocation of $P$ can be large, many of them are non-optimal. For two plans $p_1$ and $p_2$, if $p_1$ uses more capacity but achieves a smaller value sum comparing with $p_2$, $p_1$ must not be transferred into the optimal: Replacing items used in $p_1$ with items used in $p_2$ can always lead into a better plan. 

Utilizing this property, $P'$ uses function $\textit{thin}'$ to remove all those non-optimal plans. In this way, the number of plans returned by $P'$ is bounded by $W + 1$.
\end{itemize} 
$\textit{thin}'$ can be implemented as $O(W)$-time, and thus memoizing the results of $P'$ leads to an $O(W|is|)$-time algorithm\footnote{Note that though $P'$ does not return the actual list of selected items, it can be determined by tracing back the calculation that lead to the optimal plan. This is a standard technique, and thus we omit it throughout this paper.}.

\begin{figure*}[t]
	\centering
    \subfloat[One specification for 0/1 Knapsack.]{\label{fig:1a}
    \begin{minipage}[h]{0.45\linewidth}
        {\small
        \begin{align*}
        &W: \ \textsf{Int} \\
        &P =\  \lambda \textit{is}. \text{ if }|\textit{is}| = 0\text{ then } [[]] \\
        & \qquad \text{else } (P\ (\textit{tail}\ \textit{is})) \cat \\
        &\qquad \quad \big[(\textit{head}\ \textit{is})::p\ \big|\ p \in P\ (\textit{tail}\ \textit{is}), \\
        &\qquad \qquad \qquad(\textit{sumw}\ p) + (\textit{head}\ \textit{is}).1 \leq W\big] \\
        &S = \ \lambda p. (\textit{sumv}\ p) \\
        & \text{where} \\
        & \qquad \textit{sumw}\ p = \sum_{(w,v) \in p} w,\  \textit{sumv}\ p = \sum_{(w,v) \in p} v
        \end{align*}
        }
    \end{minipage}} %\hfill\vline\hfill
	\subfloat[One efficient scheme of memoization for 0/1 Knapsack. Given a set $s$, function $\textit{unique}$ removes all duplicated objects from $s$.]{ \label{fig:1b}
    \begin{minipage}[h]{0.53\linewidth}
        {
            \small
        \begin{align*}
        &is:\ \textsf{List}(\textsf{Int}\times\textsf{Int})\qquad W: \textsf{Int}\\
        &P' =\  \lambda i.\ \text{if }i = 0\text{ then } [(0, 0)] \\
        &\qquad \text{else let }ps = P'\ (i - 1) \cat \\
        & \qquad \quad \big[(is[-i].1 + w, is[-i].2 + v)\ \big|\ (w, v) \in P'\ (i - 1)\big]\text{ in}\\
        & \qquad \quad \quad \textit{thin}'\ ps \\
        &S' =\ \lambda p. (p.2) \\
        &\text{where}  \\
        &\qquad \textit{thin}'\ ps = \textit{unique}\ [(w,v) \in ps\ |\ \forall (w', v') \in ps, \neg (w, v) \prec (w', v')] \\
        &\qquad (w, v) \prec (w', v') = (w' < w \wedge v' \geq v) \vee (w' = w \wedge v' > v)
        \end{align*}
        \vspace{-10pt}
        }
    \end{minipage} 
    } \\
	\subfloat[The procedure for our transformation system to derive scheme $(P', S')$ (Figure \ref{fig:1b}) from specification $(P, S)$ (Figure \ref{fig:1a}). In each step, examples for unknown program fragments are extracted from the case where three items $(3, 3), (2, 3), (1, 2)$ are available and the capacity of the knapsack is $4$.]{ \label{fig:1c}
    \begin{minipage}[h]{1\linewidth}
        {
            \includegraphics[width=1\textwidth]{fig/overview.png}
        
        }
    \end{minipage} 
    }
    \caption{A running example for our approach to synthesize efficient memoization for 0/1 knapsack.}
\end{figure*}

Motivating by the importance of memoization and its difficulty for designing, we study the problem of \textit{automatically synthesizing efficient memoization}.
The difficulty of this task comes from different aspects, including the large scale of the result, the complex control flow leaded by self-recursion and memoization, and the objective on the efficiency.

\noindent \textbf{Hylomorphism}. To alleviate these challenges, our paper utilizes related studies in \textit{program calculus}~\cite{DBLP:books/daglib/0096998}, a domain aiming to establish an algebra for \textit{human users} to derive programs. In this domain, varies theorems and principles have been developed for capturing the common ideas in designing efficient memoization. Many of them are under the assumption that the plan generator $P$ is given as a \textit{relational hylomorphism} or its special case~\cite{DBLP:conf/plilp/Moor95, DBLP:journals/mscs/Moor94, DBLP:conf/flops/MorihataKO14, DBLP:journals/scp/GiegerichMS04}. 

A hylomorphism is a recursive function, which is the fusion of an \textit{anamorphism} (or \textit{unfold}), which constructs an intermediate structure from the input, and a \textit{catamorphism} (or \textit{fold}), which calculates the result via a structural recursion on the intermediate structure. The most significant advantage of hylomorphisms is that it provides a regular program structure for formalize and perform optimizations. In addition, the loss of generality led by the restriction on hylomorphisms is slight. It has been proven that every recursion of interest (e.g., primitive recursions) can be specified by hylomorphisms~\cite{bird1994relational}, and such a process can be automated~\cite{DBLP:conf/icfp/HuIT96}. 

Following these previous studies in program calculus, our paper retains the assumption that generator $P$ is given as a relational hylomorphism. For simplicity, we continue using recursive programs to illustrate our main ideas in the remainder of this section. The formal definition of relational hylomorphisms will be introduced in Section \ref{section:background}.

\noindent \textbf{Transformation System}. \textit{The first contribution of this paper is a transformation system for deriving efficient memoization from hylomorphisms.} The time cost of a memoization scheme for a hylomorphism is related to four factors: (1) the number of returned plans, (2) the cost of transferring the plans, (3) the number of different search states, and (4) the cost of transferring the search states. Our transformation system uses four sequential steps to optimize each of these factors for the initial hylomorphism. In each step, only several non-recursive program fragment are introduced, and thus the complexity for program synthesis is limited. 

The transformation system is based on previous studies in program calculus. However, because these studies focus on only specific steps and specific subclasses of hylomorphisms, we summarize and generalize their results such that our system can capture the whole derivation from a hylomorphism to an efficient scheme of memoization. 

%Figure \ref{fig:1c} shows the procedure for our system to derive $(P', S')$ (Figure \ref{fig:1b}) from specification $(P, S)$ (Figure \ref{fig:1a}). 

%\textit{Step 1}. In the first step, we reduce the number of returned plans by \textit{thinning}. Function \textit{thin} takes a preorder $R$ and a set of objects as the input and removes all those objects that are non-maximal in the sense of $R$. \citet{DBLP:journals/mscs/Moor94} shows that \textit{thin} can express the idea of pruning off non-optimal plans. When $R\ p_1\ p_2$ represents that the effectiveness of plan $p_1$ is always worse than plan $p_2$, $\textit{thin}\ R\ ps$ naturally filters out all those non-optimal plans from plan set $ps$.

%In our example of 0/1 Knapsack, let $p_1$ and $p_2$ be two plans returned The transformation system is based on previous studies in program calculus. However, because these studies focus on only specific steps and specific subclasses of hylomorphisms, we summarize and generalize their results such that our system can capture the whole derivation from a hylomorphism to an efficient scheme of memoization. 

Figure \ref{fig:1c} shows the procedure for our system to derive $(P', S')$ (Figure \ref{fig:1b}) from specification $(P, S)$ (Figure \ref{fig:1a}). 

{\bf Step 1}. In the first step, we reduce the number of returned plans by \textit{thinning}. Function \textit{thin} takes a preorder $R$ and a set of objects as the input and removes all those objects that are non-maximal in the sense of $R$. \citet{DBLP:journals/mscs/Moor94} shows that \textit{thin} can express the idea of pruning off non-optimal plans. When $p_1\ R\ p_2$ represents that the effectiveness of plan $p_1$ is dominated by plan $p_2$, $\textit{thin}\ R\ ps$ naturally filters out all those non-optimal plans from plan set $ps$.
$$
p_1\ R\ p_2 \iff \textit{sumw}\ p_1 \geq \textit{sumw}\ p_2 \wedge \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2
$$

To apply thinning, our system insert an invocation of \textit{thin} at the end of generator $P$, where the preorder is an unknown fragment $\red{?R}$. Then, the remaining task is to synthesize proper $\red{?R}$ that guarantees both the correctness and the efficiency. 

{\bf Step 2}. In the second step, we reduce the cost of transferring plans via \textit{incrementalization}~\cite{DBLP:journals/lisp/LiuS03, DBLP:conf/flops/MorihataKO14}. A plan for an optimization problem is usually a complex data structure, and thus it costs a lot of time to calculate some functions over plans. Incrementalization improves this point by caching cared values for each plan and converting the inputs of the calculations from cached values instead of the whole plan.

In our example of 0/1 Knapsack, each plan is a list of items where the size can be as large as $|is|$. Therefore, it is time-consuming to calculate $\textit{sumw}$ and $\textit{sumv}$ used in $P$ and $S$. Scheme $(P', S')$ improves this point by directly storing the outputs of $\textit{sumw}$ and $\textit{sumv}$ for each plan. In this way, the time complexity of querying the outputs of these two functions is reduced from $O(|is|)$ to $O(1)$. 

To apply incrementalization, our system tries to rewrite all usages of plan $p$ with $\red{?f_p}\ p$, where $\red{?f_p}$ is an unknown fragment mapping from plans to a tuple of scalar values. The system identifies all queries (marked as \blue{blue}), which calculate cared values for plans, and modifications (marked as \green{green}), which generate new plans, and replaces them with unknown fragments $\red{?q}$ and $\red{?c}$ respectively. 
Then, the remaining task of incrementalization is to synthesize these fragments. 

{\bf Step 3}. In the third step, we reduce the number of different search states by finding a compact way of storing results. Memoization is usually performed according to the inputs. 
\begin{itemize}[leftmargin=*]
\item The results of $P$ on search state $s$ is stored in $\textit{Mem}[i]$, the unit in the memoization space with key $s$.
\item For each invocation $P\ s$, $\textit{Mem}[s]$ is queried, and the stored results will be returned if it exists. 
\end{itemize}

However, in practice, the search state $s$ usually includes unnecessary information. At this time, this direct method of memoization has two main shortages.
\begin{itemize}[leftmargin=*]
\item The results of $P$ may be the same on different inputs, but the direct method will treat them separately. 
\item State $s$ may be complex, and thus it may be time-consuming to update/query the memoization space with key $s$.  
\end{itemize}

In our example of 0/1 Knapsack, the search state of the initial generator $P$ (Figure \ref{fig:1a}) is a list of items. However, only the size of the search state matters, because search states in $P$ must be suffices of the whole item list.

To improve this point, our system replace the default key $s$ with $\red{?f_m}\ s$, where $\red{?f_m}$ is an unknown fragment mapping from search states to a tuple of scalar values. After that, the results of $P\ s$ will be stored in $\textit{Mem}[\red{?f_m}\ s]$ instead of $\textit{Mem}[s]$.

Then, the remaining task is to synthesize proper $\red{?f_m}$ that guarantees both the correctness and the efficiency.

{\bf Step 4}. Similar to the second step, we reduce the cost of transferring search state via \textit{incrementalization}. Our system tries to rewrite all usages of search state $s$ with $\red{?f_s}\ s$, where $\red{?f_s}$ is an unknown fragment mapping from search states to a tuple of scalar values. To do so, the system identifies all queries and modifications related to search states and rewrites them by introducing unknown fragments. 

\noindent \textbf{Specification Extraction}. To automate the transformation system, we use program synthesizers the find proper assignments to the fragments introduced in each step.

Program synthesis requires a specification on the synthesis target. A natural specification here is to ensure the \textit{correctness} of the transformation result in each step.
\begin{itemize}[leftmargin=*]
\item \textit{In each step, for all instances of the target optimization problem, the score of the plan returned by the resulting scheme should always be the same as that of the input scheme.}
\end{itemize}

However, such a specification is too complex for synthesis. First, because the fragments are recursively invoked in the plan generator $P$, it is difficult for the synthesizer to make optimizations. Second, because complex operators on recursive data structures are usually involved in a scheme, it is difficult to verify the correctness of the result.

We use two methods to simplify the specification.
\begin{itemize}[leftmargin=*]
\item To remove the recursion in the specification, for each step, we construct a stronger specification that (1) implies the correctness of the resulting scheme, and (2) constraints on every single recursion of generator $P$.
\item We make a trade-off between the difficulty of the verification and the guarantee on the correctness. We evaluate the synthesis result only on a sampled set of concrete instances and establish a probabilistic guarantee on the correctness using the theory of \textit{Occam learning}~\cite{DBLP:journals/pacmpl/JiXXH21}.
\end{itemize}

In this way, we get simple specifications for fragments, which are in the form of examples. We use an instance of 0/1 Knapsack to illustrate this process, where \textbf{items $\mathbf{(3, 3), (2, 3),}$ $\mathbf{(1, 2)}$ are available, and the capacity is $\mathbf{4}$}. Some results are shown as the forth column in Figure \ref{fig:1c}.

\textbf{Step 1}. The specification on $\red{?R}$ is two-fold.
\begin{enumerate}[leftmargin=*]
    \item For any set of plans $ps$, the plan with the largest value sum in $ps$ is reserved in $\textit{thin}\ \red{?R}\ ps$.
\item For any two consecutive invocations $(P\ is)$ and $(P\ (\textit{tail}\ is))$, for any two plans $p_1, p_2$ returned by $(P\ (\textit{tail}\ is))$, $p_1\ \red{?R}\ p_2$ implies that all plans in $(P\ is)$ constructed from $p_1$ are worse than plans constructed from $p_2$ in the sense of $\red{?R}$. 
\end{enumerate}

Let $P_1$ be the result generator of this step. The second constraint ensures that $(P_1\ is)$ is always equal to $(\textit{thin}\ \red{?R}\ (P\ is))$, and the first constraint ensures that the plan with the largest value sum is always reserved by $\textit{thin}\ \red{?R}$. Therefore, they together imply the correctness of the resulting scheme.

To satisfy the first constraint, we limit the form of $\red{?R}$ to be $\lambda p_1. \lambda p_2. \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2 \wedge p_1\red{?R'}p_2$, where $\red{?R'}$ is another unknown preorder, and then we can extract examples for $\red{?R}$ (or $\red{R'}$) according to the second constraint. 

In our example, let us consider consecutive invocations $P\ [(3, 3), (2, 3), (1, 2)]$ and $P\ [(2, 3), (1, 2)]$, denoted as $P_x$ and $P_y$ respective, and plans $p_1 = [(1, 2)]$ and $p_2 = [(2, 3)]$ returned by $P_y$. In invocation $P_x$, $p_1$ is extended to two plans $p_{1,1} = [(1, 2)]$ and $p_{1, 2} = [(3, 3), (1, 2)]$, while $p_2$ is extended to plan $p_{2,1} = [(2, 3)]$ only. Note that the value sum of $p_{1, 2}$ is $4$ while the value sum of $p_{2, 1}$ is only $2$. Therefore, no matter what $\red{R'}$ is, $p_{1, 2}$ is always no worse than $p_{2,1}$ in the sense of $\red{R}$. At this time, to satisfy the second constraint, $p_1$ must be no worse than $p_2$ in the sense of $\red{R}$. In this way, example $\neg ([(1, 2)]\ \red{?R}\ [(2, 3)])$ for $\red{?R}$ is obtained. 

\textbf{Step 2}. The specification of $\red{?f_p}$, $\red{?q}$ and $\red{?c}$ is to keep the running procedure of $P$ unchanged except all plans are replaced by the corresponding outputs of $\red{?f_p}$. Using this property, examples for these fragments can be directly extracted from the execution of the original scheme. 

We take modification $\green{(\textit{head}\ is):: p}$ as an example, which is replaced with $(\red{?c}\ (\textit{head}\ is)\ p)$ by the transformation system. In invocation $P\ [(3, 3), (2, 3), (1, 2)]$, this modification constructs plan $[(3, 3), (1, 2)]$ from plan $p = [(1, 2)]$. Because the running procedure is unchanged, we know that there will be a corresponding invocation of $\red{?c}$ where the input is $(3, 3)$ and $\red{?f_p}\ [1, 2]$ and the output is $\red{?f_p}\ [(3, 3), (1, 2)]$. In this way, an example on $\red{?c}$ is obtained. 

\textbf{Step 3}. The specification of $\red{?f_m}$ is that its outputs on two search states, where the results of $P$ differ, are always different. This constraint ensures that when $\textit{Mem}[\red{?f_m}\ s]$ exists, it is always equal to the actual results of $P$ on $s$. 

Extracting examples for $\red{?f_m}$ is direct. In our example, let us consider two search states $[(2, 3), (1, 2)]$ and $[(1, 2)]$. After the first steps, the results of $P$ on these two states are $[(0,0), (1, 2), (2, 3), (3,5)]$ and $[(0, 0), (1, 2)]$ respectively, which are different. Therefore, example ${\red ?f_m}\ [(2, 3), (1, 2)] \neq {\red ?f_m}\ [(1, 2)]$ is obtained.

\textbf{Step 4}. Similar with the second step, the specification here is to keep the running procedure of $P$ unchanged except all states are replaced by the corresponding outputs of $\red{?f_s}$, and the examples can also be extracted similarly. 

\noindent \textbf{Synthesizers}. 



==> sections/Introduction2.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Introduction} \label{section:introduction}
\textit{Combinatorial Optimization} is a topic on finding an optimal solution from a finite set of valid solutions~\cite{schrijver2003combinatorial}. Combinatorial optimization problems (COPs), such as the knapsack problem and the traveling salesman problem, widely exist in various domains. Solving a COP is usually difficult as the number of solutions can be extremely large. 

\textit{Memoization}~\cite{michie1968memo}, or \textit{dynamic programming}, is an important technique for solving COPs. It stores the results of expensive function invocations and directly returns the stored results when the same invocations occur again. In this way, the time complexity of a recursive function can be greatly reduced when the number of different inputs of the function is limited. Such a property is known as \textit{overlapping subproblems}. Since identifying overlapping subproblems for a COP is usually non-trivial, implementing a program that is efficient for memoization can be difficult.

Motivated by the importance \yxmodify{of memoization and its difficulty for designing}{and difficulty of designing memoization}, in this paper, we study the task of \textbf{automatically synthesizing efficient memoization for COPs}. The difficulty of this task comes from (1) the complexity of the result, including its large scale and its complex control flow led by self-recursion and memoization, and (2) the objective of maximizing the efficiency of the result. These two properties make it unrealistic to directly synthesize efficient memoization from the start. 

To simplify this task, we utilize related studies in \textit{program calculus}~\cite{DBLP:books/daglib/0096998}. \textit{Program calculus} is a domain aiming to establish an algebra for \textbf{human users} to derive programs, where various theorems and principles have been developed for manually deriving efficient memoization. In this paper, we use these results in program calculus to decompose the whole synthesis task into simpler subtasks that are treatable by synthesis techniques.

\yxcomment{An example may be needed as an average reader will totally get lost.}
As the first step, we keep the setting consistent with most related studies in program calculus, where a COP is described by \textit{relational hylomorphisms}~\cite{DBLP:conf/plilp/Moor95, DBLP:journals/mscs/Moor94, DBLP:conf/flops/MorihataKO14, DBLP:journals/scp/GiegerichMS04}. In this setting, a COP is described by two functions, a generator, and a scorer. 
\begin{itemize}[leftmargin=*]
\item The generator is required to be a \textit{relational hylomorphism}, and its usage is to generate the set of valid solutions.
\item The scorer evaluates the objective function for each plan.
\end{itemize}

A hylomorphism is a recursive function, which is the fusion of an \textit{anamorphism} (or \textit{unfold}), which constructs an intermediate structure from the input, and a \textit{catamorphism} (or \textit{fold}), which calculates the result via a structural recursion on the intermediate structure. The expressiveness of hylomorphisms is powerful. \citet{bird1994relational, DBLP:conf/icfp/HuIT96} show that every recursion of interest (e.g., primitive recursions) can be automatically converted to hylomorphisms. In program calculus, hylomorphisms provide a regular program structure for formalizing and performing optimizations.

\textit{The first contribution of this paper is a transformation system that converts the derivation of efficient memoization into four synthesis tasks.} Starting from the trivial combination of the plan generator and the scorer, our system uses four steps to derive an efficient program for memoization. In each step, the system rewrites the current program with some new program fragments and thus optimizes one factor related to the time cost of memoization. Each step in the system corresponds to a synthesis task for finding proper program fragments, in which both the scale of the target programs and the complexity of related control flow are limited. 

Our system utilizes two techniques in program calculus.
\begin{itemize}[leftmargin=*]
\item \textit{Thinning}~\cite{DBLP:journals/mscs/Moor94} uses a preorder over solutions to represent the process of pruning off non-optimal partial solutions. For a set of solutions, it only reserves those that are local maxima in the sense of the preorder.
\item \textit{Incrementalization}~\cite{DBLP:journals/lisp/LiuS03} avoids expensive function calls on solutions (states) by storing the results of functions for each solution (state) and incrementally calculates them when new solutions (states) are constructed. 
\end{itemize}
Because both techniques are proposed only for a subclass of hylomorphisms, we generalize them in our system. 

To form synthesis tasks, it is necessary to get specifications for these introduced program fragments. One trivial specification is that the fragments should keep the semantics of the whole program unchanged. However, since the fragments are wrapped in the recursive structure of the generator, such a specification is indirect and makes it difficult to synthesize. To get simpler specifications, we (1) construct stronger specifications that constraint on every single recursion, and (2) extract examples for fragments from running procedures on concrete instances of the COP. 

\textit{The second contribution of this paper is an efficient synthesizer for solving the synthesis tasks generated by the transformation system}. We conclude the four synthesis tasks into two categories and deal with them separately. 
\begin{itemize}[leftmargin=*]
\item For the two tasks from incrementalization, we reduce them into \textit{lifting problems}~\cite{lifting} and use \textit{AutoLifter}, a SOTA solver for lifting problems, to solve them. 
%\item The other two tasks are to find a preorder satisfying several negative examples and minimize the number of local maxima. For simplicity, we assume the preorder is a conjunction of comparisons on several key functions.  \rycomment{It is too detailed?}

%To synthesize valid preorders, we synthesize key functions in turns and ensure that a considerable number of examples are satisfied in each turn. 

%To minimize the number of local maxima, we use the range of key functions to approximate the number of local maxima and use branch-and-bound to find the optimal.
\item The other two tasks are to find a preorder satisfying several negative examples and maximize the efficiency of the result program. We synthesize the preorder as a conjunction of comparisons on several key functions and decide the comparisons one by one. W e set up an objective function on preorders that approximates the efficiency of the result program and use branch-and-bound to find the optimal.
\end{itemize}

We implement our transformation system and the synthesizer into an approach namely \mainname and evaluate its effectiveness on a dataset. \todo{Details on evaluation}

In summary, this paper explores the problem of synthesizing efficient memoization for COPs described by hylomorphisms and makes the following contributions. 
\begin{itemize}[leftmargin=*]
\item Proposing a transformation system that derives efficient memoization for a hylomorphism via four synthesis tasks.
\item Proposing an efficient synthesizer for incrementalization and synthesizing preorders from negative examples.
\item Conducting an evaluation on \todo{description} and showing the effectiveness of our approach \mainname.
\end{itemize} 

==> sections/Introduction3-Yingfei.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Introduction} \label{section:introduction}
\textit{Combinatorial Optimization} is a topic on finding an optimal solution from a finite set of valid solutions~\cite{schrijver2003combinatorial}. Combinatorial optimization problems (COPs), such as the knapsack problem and the traveling salesman problem, widely exist in various domains. Solving a COP is usually difficult as the number of solutions can be extremely large. 

\textit{Dynamic programming} is an important technique for solving COPs. A dynamic programming algorithm can be implemented in the top-down approach or the bottom-up approach, and the top-down approach is also known as \emph{memoization}. %Designing an efficient memoization algorithm is challenging, as we need to identify overlapping subproblems that can be efficiently solved and reused.
Given a recursive function, memoization can be easily implemented by caching the results of existing calls. Though obtaining an arbitrary memoization algorithm is not difficult, different memoization algorithms could have huge performance differences, and it is challenging to find an \emph{efficient} memoization algorithm for a specific problem. 

% \textit{Memoization}~\cite{michie1968memo}, or \textit{dynamic programming}, is an important technique for solving COPs. It stores the results of expensive function invocations and directly returns the stored results when the same invocations occur again. In this way, the time complexity of a recursive function can be greatly reduced when the number of different inputs of the function is limited. Such a property is known as \textit{overlapping subproblems}. Since identifying overlapping subproblems for a COP is usually non-trivial, implementing a program that is efficient for memoization can be difficult.

Motivated by the importance and difficulty of designing memoization, in this paper, we propose a novel approach, \mainname, to \textbf{automatically synthesizing efficient memoization for COPs}. %The difficulty of this task comes from (1) the complexity of the result, including its large scale and its complex control flow led by self-recursion and memoization, and (2) the objective of maximizing the efficiency of the result. These two properties make it unrealistic to directly synthesize efficient memoization from the start. 
This task is challenging because (1) the result program is large and involves complex control flow, and (2) its efficiency needs to be ensured. %we need to ensure the efficiency of the synthesized program.

To simplify this task, we utilize the theory of \textit{program calculation}~\cite{DBLP:books/daglib/0096998}. The theory establishes an algebra for \textbf{human users} to derive programs, where various theorems and principles have been developed for manually deriving efficient memoization. In this paper, we use these results to decompose the whole synthesis task into simpler subtasks that are tractable by synthesis techniques.

% \yxcomment{An example may be needed as an average reader will totally get lost.}
% As the first step, we keep the setting consistent with most related studies in program calculus, where a COP is described by \textit{relational hylomorphisms}~\cite{DBLP:conf/plilp/Moor95, DBLP:journals/mscs/Moor94, DBLP:conf/flops/MorihataKO14, DBLP:journals/scp/GiegerichMS04}. In this setting, a COP is described by two functions, a generator, and a scorer. 
% \begin{itemize}[leftmargin=*]
% \item The generator is required to be a \textit{relational hylomorphism}, and its usage is to generate the set of valid solutions.
% \item The scorer evaluates the objective function for each plan.
% \end{itemize}

% A hylomorphism is a recursive function, which is the fusion of an \textit{anamorphism} (or \textit{unfold}), which constructs an intermediate structure from the input, and a \textit{catamorphism} (or \textit{fold}), which calculates the result via a structural recursion on the intermediate structure. The expressiveness of hylomorphisms is powerful. \citet{bird1994relational, DBLP:conf/icfp/HuIT96} show that every recursion of interest (e.g., primitive recursions) can be automatically converted to hylomorphisms. In program calculus, hylomorphisms provide a regular program structure for formalizing and performing optimizations.

Concretely, our approach takes a (possibly inefficient) recursive program specified as a (relational) hylomorphism and produces an efficient memoization program. A hylomorphism is a program written in a specific yet general recursive pattern. \citet{DBLP:conf/fpca/MeijerFP91} show that every primitive recursive function can be written in a hylomorphism. Different approaches for automatically deriving hylomorphisms have been proposed, including generating a hylomorphism from a recursive program~\cite{bird1994relational, DBLP:conf/icfp/HuIT96} or from a logic specification~\cite{DBLP:conf/sigsoft/0003ML21}.

\textit{The first contribution of this paper is a transformation system that transforms a hylomorphism into an efficient memoization through four synthesis subtasks.} %Starting from the trivial combination of the plan generator and the scorer, our system uses four steps to derive an efficient program for memoization. In each step, the system rewrites the current program with some new program fragments and thus optimizes one factor related to the time cost of memoization. Each step in the system corresponds to a synthesis task for finding proper program fragments, in which both the scale of the target programs and the complexity of related control flow are limited. 
The transformation is a combination of two existing techniques in program calculation, namely \emph{thinning}~\cite{DBLP:journals/mscs/Moor94} and \emph{incrementalization}~\cite{DBLP:journals/lisp/LiuS03}. Both techniques were proposed only for a subclass of hylomorphisms, we generalize them to hylomorphisms in our system. The four synthesis subtasks involve only subparts of the program that do not have complex control structures, and thus are tractable. 

% Our system utilizes two techniques in program calculus.
% \begin{itemize}[leftmargin=*]
% \item \textit{Thinning}~\cite{DBLP:journals/mscs/Moor94} uses a preorder over solutions to represent the process of pruning off non-optimal partial solutions. For a set of solutions, it only reserves those that are local maxima in the sense of the preorder.
% \item \textit{Incrementalization}~\cite{DBLP:journals/lisp/LiuS03} avoids expensive function calls on solutions (states) by storing the results of functions for each solution (state) and incrementally calculates them when new solutions (states) are constructed. 
% \end{itemize}
% Because both techniques are proposed only for a subclass of hylomorphisms, we generalize them in our system. 

% To form synthesis tasks, it is necessary to get specifications for these introduced program fragments. One trivial specification is that the fragments should keep the semantics of the whole program unchanged. However, since the fragments are wrapped in the recursive structure of the generator, such a specification is indirect and makes it difficult to synthesize. To get simpler specifications, we (1) construct stronger specifications that constraint on every single recursion, and (2) extract examples for fragments from running procedures on concrete instances of the COP. 

\textit{The second contribution of this paper is efficient synthesis algorithms for solving the four synthesis subtasks}. We classify the four subtasks into two categories, and solve them by reducing to a problem that an existing synthesizer can handle, or proposing a new synthesis algorithm for the subtasks.

% \textit{The second contribution of this paper is an efficient synthesizer for solving the synthesis tasks generated by the transformation system}. We conclude the four synthesis tasks into two categories and deal with them separately. 
% \begin{itemize}[leftmargin=*]
% \item For the two tasks from incrementalization, we reduce them into \textit{lifting problems}~\cite{lifting} and use \textit{AutoLifter}, a SOTA solver for lifting problems, to solve them. 
% \item The other two tasks are to find a preorder satisfying several negative examples and maximize the efficiency of the result program. We synthesize the preorder as a conjunction of comparisons on several key functions and decide the comparisons one by one. We set up an objective function on preorders that approximates the efficiency of the result program and use branch-and-bound to find the optimal.
% \end{itemize}

We implement %our transformation system and the synthesis algorithms into an approach namely 
\mainname and evaluate \mainname on $37$ tasks related to $16$ COPs collected from \textit{Introduction to Algorithm}~\cite{cormen2009introduction}, a popular textbook for algorithm courses. The results show that \mainname achieves exponential speed-ups on $97.3\%$ tasks with an average time cost of $59.2$ seconds. Moreover, on $70.3\%$ tasks, \mainname achieves the same time complexities as the solutions provided by %\textit{Introduction to Algorithm} and a solution to its exercises~
\citet{cormen2009introduction} and \citet{algsolutions}.

% In summary, this paper explores the problem of synthesizing efficient memoization for COPs described by hylomorphisms and makes the following contributions. 
% \begin{itemize}[leftmargin=*]
% \item Proposing a transformation system that derives efficient memoization via four synthesis subtasks.
% \item Proposing efficient synthesis algorithms for solving the synthesis subtasks.
% \item Conducting an evaluation on $37$ tasks related to $16$ COPs and showing the effectiveness of our approach \mainname.
% \end{itemize} 

==> sections/MotivatingExample.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Overview} \label{section:overview}
In this section, we introduce the main idea of \mainname using a classical COP namely \textit{0/1 knapsack}~\cite{mathews1896partition}. 
\begin{center}
    \it
    Given a set of items, each with a weight $w_i$ and a value $v_i$, put a subset of them in a knapsack of capacity $W$ to get the maximum total value in the knapsack.
\end{center}
For example, $is = [(3, 3), (2, 3), (1, 2)], W = 4$ describes an instance of 0/1 knapsack, where three items are available, their weights are $3, 2, 1$ respectively, their values are $3, 3, 2$ respectively, and the capacity of the knapsack is $4$. At this time, the optimal solution is to put the first and the third items, i.e., $[(3, 3), (1,2)]$, where the value sum is $5$. 


Figure \ref{fig:overview} shows the whole procedure for \mainname to synthesize efficient memoization for this problem, where each row describes one step of the transformation system and the corresponding synthesis task. 
\begin{itemize}[leftmargin=*]
\item \textit{Initial Program} lists the program to be optimized.
\item \textit{Intermediate Program} lists the result of rewriting the initial program with the new program fragments (marked as \red{red}). 
\item \textit{Example} lists some examples for the fragments, which are extracted from the running procedure on instance $(is, W)$.
\item \textit{Synthesis Result} lists the assignment to the program fragments found by the synthesizer.  
\end{itemize}

In Figure \ref{fig:overview}, a program is described by a triple $(P, S, m)$, where generator $P$ constructs a set of solutions, scorer $S$ evaluates the objective function for solutions, and key function $m$ describes how the results of $P$ is memoized. Given instance $i$, $(P, S, m)$ executes as the following.
\begin{itemize}[leftmargin=*]
\item $(P\ i)$ is invoked to generate a set of solutions. During this process, each invocation $(P\ s)$ is related to a memory unit via key $(m\ s)$. the result of $(P\ s)$ will be stored in this unit, and $(P\ s)$ will be skipped if the result already exists.
\item $S$ calculates the objective value for each valid solution.
\item The solution with the largest objective value is returned.
\end{itemize}
Following studies in program calculus, \mainname requires $P$ to be a relational hylomorphism. For simplicity, in this section, we still use recursive programs to illustrate our main idea. Relational hylomorphisms will be introduced in Section \ref{section:background}.

In our example, \mainname starts from program $(P_1, S_1, m_1)$ in Figure \ref{fig:overview}, where $P_1$ and $S_1$ are provided by the user to describe the COP, and identity function $m_1$ represents a default way of memoization. Such a program is ineffective, as its time complexity is exponential to the number of items. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{fig/overview.png}
    \caption{The running procedure for \mainname to synthesize efficient memoization for 0/1 knapsack, where $\textit{sumw}\ is$ and $\textit{sumv}\ is$ calculates the weight sum and the value sum for item list $is$ respectively, and the capacity of the knapsack and the whole item list can be referred via global variable $W$ and $is$ respectively.}
    \label{fig:overview}
\end{figure*}

\subsection{Transformation System}
There are four factors that possibly lead to the inefficiency of the input program $(P_1, S_1, m_1)$.
\begin{enumerate}[leftmargin=*]
\item $(P_1\ is)$ may return many non-optimal solutions.
\item The solutions returned by $P\ is$ is a list such that operations on it (e.g.,  calculating $(\textit{sumw}\ p)$) may be costly.
\item Search state $is$ for $P$ may include redundant information and thus the default memoization may be ineffective.
\item Search state $is$ is a list such that operations on it (e.g., calculating $(\textit{tail}\ is)$) may be costly.
\end{enumerate}

\mainname optimizes these four factors one by one. 

\noindent \textbf{Step 1}. \mainname uses \textit{thinning}~\cite{DBLP:journals/mscs/Moor94} to reduce the number of solutions generated by $P$. To distinguish, we use \textit{partial solutions} to denote the plans constructed by a recursive invocation of generator $P$. A partial solution will be transferred to several \textit{global solutions} for the instance.

Thinning uses a preorder $R$ to represent the dominant relationship between partial solutions, where $p_1\ R\ p_2$ represents that partial solution $p_1$ can never lead to the global optimal solution if partial solution $p_2$ exists. If such a preorder exists, the result of $(P\ is)$ can be simplified to $(\textit{thin}\ R\ (P\ is))$, where $\textit{thin}$ returns all local maxima in $(P\ is)$ in the sense of $R$. 

In program $(P_1, S_1, m_1)$, partial solution $p_1$ is dominated by $p_2$ if $p_1$ not only consumes more capacity but also gains smaller value. For any global solution leaded by $p_1$, a better solution can be obtained by replacing items in $p_1$ with $p_2$. Such a relation can be described by the following preorder.
$$
p_1\ R\ p_2 \iff \textit{sumw}\ p_1 \geq \textit{sumw}\ p_2 \wedge \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2
$$

Because the weight sum of partial solutions must be integers in $[0, W]$, the size of $(\textit{thin}\ R\ (P\ is))$ is at most $W + 1$. Therefore, thinning could exponentially reduce the number of returned solutions if $W$ and $|is|$ are in the same order. 

As shown in Figure \ref{fig:overview}, \mainname applies thinning by inserting an invocation of \textit{thin} with an unknown preorder $\red{?R}$ to $P_1$, which is found via program synthesis.

\noindent \textbf{Step 2}. \mainname uses \textit{incrementalization}~\cite{DBLP:journals/lisp/LiuS03} to remove costly operations on solution in $(P_2, S_2, m_2)$. 

Concretely, \mainname tries to rewrite all usages of solution $p$ with $(\red{?f_p}\ p)$, where $\red{?f_p}$ is an unknown fragment mapping solutions, which are lists of items, to simpler structures, such as tuples of scalar values. To do so, \mainname identifies all queries (marked as \blue{blue}), which calculate cared values for solutions, and modifications (marked as \green{green}), which generate new solutions, in program $(P_2, S_2, m_2)$ and replaces them with unknown fragments $\red{?q}$ and $\red{?c}$ respectively\footnote{Though $P_2'$ does not return concrete solutions, the optimal solution can be determined by tracing back the calculation that lead to the optimal solution. This is a standard technique, and thus we omit it throughout this paper.}. \mainname uses synthesizers to find proper assignments to these fragments.

\noindent \textbf{Step 3}. To remove redundant information, \mainname synthesizes a new key function $\red{?f_m}$ and thus allows sharing results between different search states of $P$. 

In program $(P_3, S_3, m_3)$, the search state is a list of items. However, only the size of the search states matters, and the contents are redundant, as search states in $P_3$ must be suffixes of the whole item list. \mainname removes this redundancy for memoization by synthesizing $\red{?f_m}$ as $\lambda is. |is|$.

\noindent \textbf{Step 4}. Similar to Step 2, \mainname uses \textit{incrementalization} to remove costly operations on states in program $(P_4, S_4, m_4)$. \mainname tries to rewrite search states with $\red{?f_s}$, related queries with $\red{?q}$, and related modifications with $\red{?c}$. \mainname uses synthesizers to find proper assignments to these fragments.

At last, an efficient program $(P^*, S^*, m^*)$ is obtained.
\begin{itemize}[leftmargin=*]
\item The number of solutions returned by $P^*$ is $O(W)$.
\item After memoization, $P^*$ is invoked at most $O(|is|)$ times.
\item Operators on solutions and states run in constant time.
\end{itemize}
Because function $\textit{thin}$ in $P^*$ can be implemented as linear time, the time complexity of $(P^*, S^*, m^*)$ is $O(W|is|)$. When $W$ and $|is|$ are in the same order, $(P^*, S*, m^*)$ is exponentially faster than the input program $(P_1, S_1, m_1)$. 

\subsection{Specification Extraction for Program Synthesis}
To use synthesizers, a specification on the introduced fragments is necessary. A natural specification here is to ensure the correctness of the transformation result: The resulting program should always find a solution with the largest possible value sum for all instances of 0/1 knapsack.

However, such a specification is too complex for program synthesis, where the synthesis targets are wrapped in the recursive structure of the plan generator $P$. To extract simpler specifications, \mainname decomposes the correctness requirement to each step of the recursion and collects direct examples for the introduced program fragments from the running procedure on concrete instances. 

We still use instance $([(3, 3), (2, 3), (1, 2)], 4)$ of 0/1 knapsack to show how these examples are extracted.

\noindent \textbf{Step 1}. To ensure the correctness of $(P_1', S_1', m_1')$, \mainname requires $\red{?R}$ to satisfy the following two conditions. 
\begin{enumerate}[leftmargin=*]
    \item For any two consecutive invocations $(P_1\ is), (P_1\ (\textit{tail}\ is))$, for any partial solutions $p_1, p_2$ returned by $(P_1\ (\textit{tail}\ is))$, $p_1\ \red{?R}\ p_2$ implies that solutions in $(P_1\ is)$ constructed from $p_1$ are worse than solutions constructed from $p_2$ in $\red{?R}$. 
\item For any set of solutions $ps$, the solution with the largest value sum in $ps$ is always a local maximum in $\red{?R}$.
\end{enumerate}

The first condition ensures that $(P_1'\ is)$ is always equal to $(\textit{thin}\ \red{?R}\ (P_1\ is))$, and the second condition ensures that the solution with the largest value sum is always reserved. Therefore, they together imply the correctness of $(P_1', S_1', m_1')$.

For the first condition, \mainname limits the form of $\red{?R}$ to be $\lambda p_1. \lambda p_2. \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2 \wedge p_1\red{?R'}p_2$, where $\red{?R'}$ is another unknown preorder, and then extracts examples for $\red{?R'}$ according to the second condition.

Let us consider two consecutive invocations $P_x = P\ [(3, 3),
$ $(2,3), (1,2)]$ and $P_y = P\ [(2, 3), (1, 2)]$, and partial solutions $p_1 = [(1, 2)]$ and $p_2 = [(2, 3)]$ generated by $P_y$. In $P_x$, $p_1$ is extended to two solutions $p_{1,1} = [(1, 2)]$ and $p_{1, 2} = [(3, 3), (1, 2)]$, while $p_2$ is extended to $p_{2,1} = [(2, 3)]$ only. 

Note that the value sum of $p_{1,2}$, which is equal to $4$, is larger than the value sum $p_{2,1}$, which is equal to $2$. Therefore, no matter what $\red{R'}$ is, $p_{1, 2}$ is always no worse than $p_{2,1}$ in the sense of $\red{R}$. At this time, according to the second constraint, $p_1$ must be no worse than $p_2$ in the sense of $\red{R}$. In this way, example $\neg ([(1, 2)]\ \red{?R}\ [(2, 3)])$ for preorder $\red{?R}$ is obtained. 

\noindent \textbf{Step 2}. To ensure the correctness of $(P_2', S_2', m_2')$, \mainname requires $\red{?f_p}, \red{?q}$ and $\red{?c}$ to keep the running procedure of $(P_2, S_2, m_2)$ unchanged, except each solution is replaced by the corresponding output of $\red{?f_p}$. At this time, examples can be extracted from the execution of $(P_2, S_2, m_2)$.

Let us consider modification $\green{(\textit{head}\ is):: p}$, which is replaced with $(\red{?c}\ (\textit{head}\ is)\ p)$ in $P_2'$. In $(P_2\ [(3, 3), $ $(2, 3), (1, 2)])$, this modification constructs solution $[(3, 3), (1, 2)]$ from solution $[(1, 2)]$. Because the running procedure is unchanged, we know that there will be a corresponding invocation of $\red{?c}$ where the input is $(3, 3)$ and $\red{?f_p}\ [1, 2]$, and the output is $\red{?f_p}\ [(3, 3), (1, 2)]$. In this way, an example on $\red{?c}$ is obtained. 

\noindent \textbf{Step 3}. To ensure the correctness of $(P_3', S_3', m_3')$, \mainname requires that only search states where the results are exactly the same are mapped into the same key via $\red{?f_m}$.  

Extracting examples for $\red{?f_m}$ is direct. For example, the result of $P_3\ [(2, 3), (1, 2)]$, which is $[(0,0), (1, 2), (2, 3), (3,5)]$, is different from the result of $P_3\ [(1, 2)]$, which is $[(0, 0), (1, 2)]$. Therefore, $\red{?f_m}\ [(2, 3), (1, 2)] \neq \red{?f_m}\ [(1, 2)]$ is obtained.

\textbf{Step 4}. Similar with the Step 2, to ensure the correctness of $(P_4', S_4', m_4')$, \mainname requires $\red{?f_s}, \red{?q}$ and $\red{?c}$ to keep the running procedure of $(P_4, S_4, m_4)$ unchanged, except each state is replaced by the corresponding output of $\red{?f_s}$. The examples here can be extracted similarly with Step 2. 

\subsection{Synthesizing Fragments from Examples}
The four synthesis tasks can be divided into two categories. 

\noindent \textbf{Step 1 and Step 3}. The task in this category is to synthesize a preorder $\red{?R}$ satisfying the following two conditions.
\begin{itemize}[leftmargin=*]
\item (Correctness) $\red{?R}$ satisfies a set of negative examples $(a_i, b_i)$, which represent that $\neg (a_i\red{?R}b_i)$.
\item (Efficiency) The time complexity of the result program should be as small as possible.
\end{itemize}
The synthesis task for Step 3 can be unified into this form because key function $\red{?f_m}$ can be regraded as an equivalence relation for states, which is a special case of preorders.

\mainname synthesizes $R$ in the following form, which is a conjunction of comparisons on several key functions. 
$$
a\ R\ b \iff \wedge_{i} (\red{?key_i}\ a)\ \red{?op_i}\ (\red{?key_i}\ b)
$$
where $\red{?op_i}$ is in $\{\leq, =\}$ and $\{=\}$ in Step 1 and 3 respectively. Besides, for simplicity, we temporarily assume that $\red{?key_i}$ is taken from a finite program space. 

In this form, $\red{?R}$ satisfies a negative example $(a_i, b_i)$ if and only if at least one comparison is evaluated to be false on $(a_i, b_i)$. Therefore, for any preorder that satisfies all examples with $n_c$ comparisons, there must be a comparison that is evaluated to false on at least $1/n_c$ portion of examples. 

Motivated by this property, \mainname synthesizes with a limit $n_c$ on the number of comparisons. While determining the $i$th comparison, only those that are evaluated to false on at least $1/(n_c-i+1)$ portion of examples are considered. In this way, the search space of preorders is greatly reduced. 

To find a preorder leading to an efficient result, \mainname designs objective functions for preorders that approximate the time cost. For Step 1, the objective function comes from the time cost of implementing $\textit{thin}\ R$, which is related to the ranges of the key functions. For Step 3, the objective function is naturally set to the number of equivalence classes of states. Both objective functions increase monotonically while enlarging the set of comparisons such that it can be efficiently optimized via \textit{branch-and-bound}.


%To efficiently find a preorder with a few local minima, \mainname uses the range of each key function to approximate the number of local minima. The following are two examples.
%\begin{itemize}[leftmargin=*]
%\item For the preorder $R$ used in $(P_2, S_2, m_2)$, the number of local minima is at most $\max(\textit{range}(\textit{maxw}), \textit{range}(\textit{maxv}))$. 
%\item For the equivalence relation induced by the key function $m_4$, the number of local minima is at most $\textit{range}(m_4)$.
%\end{itemize}

%On the one hand, such an approximation is effective in practice: It is accurate in both above examples. On the other hand, this approximation monotonically increases while enlarging the set of comparisons such that it can be efficiently optimized via \textit{branch-and-bound}. \rycomment{Make this story consistent with Approach, which starts directly from the time cost instead of approximation.}

\mainname selects $n_c$ and deals with infinite program space by iteration, which will be discussed in Section \ref{section:synthesizer}.

\noindent \textbf{Step 2 and Step 4}. Both of these two tasks are for applying \textit{incrementalization}. The unified characterization of these two tasks refers to functors in the category theory. Therefore, we leave it to Section \ref{section:trans} and illustrate the idea of \mainname using the specific task generated from $(P_4, S_4, m_4)$. 

The task here is about rewriting queries $q_l = \lambda s. |s|$,  $q_h = \lambda s. (\textit{head}\ s)$, and modification $c_t = \lambda s. (\textit{tail}\ s)$. Given three set of examples $E_1, E_2, E_3$, the task is to find $\red{?f_s}, \red{?q_l}, \red{?q_h}$ and $\red{?c_t}$ satisfying the following conditions.
\begin{gather*}
\forall s \in E_1, \red{?q_l}\ (\red{?f_s}\ s) = q_l\ s \qquad 
\forall s \in E_2, \red{?q_h}\ (\red{?f_s}\ s) = q_h\ s \\
\forall s \in E_3, \red{?c_t}\ (\red{?f_s}\ s) = \red{?f_s}\ (c_t\ s)
\end{gather*}

First, the tasks for $q_l$ and $q_r$ are about synthesizing two functions from their composition. These tasks are instances of \textit{partial lifting problems} studied by \citet{lifting}. Therefore, \mainname invokes their approach, \textit{AutoLifter}, on these two tasks and thus gets a solution where $\red{?f_s} = \lambda s. |s|$, $\red{?q_l} = \lambda s. s$ and $\red{?q_h} = \lambda s. is[-s]$.

To make this solution valid for the third task,  \mainname fixes $\red{?f_s}$ to $\red{?f_s}\ s \coloneq (f_s, \red{?f_s'})\ s$, where $f_s$ is $\lambda s. |s|$ found in the previous step. At this time, $\red{?f_s}$, $\red{?q_l} = \lambda s. (s.1)$ and $\red{?q_h} = \lambda s. is[-s.1]$ must be a solution for the first two tasks.

Now, the remaining task is to synthesize $\red{?f_s'}$ and $\red{?c_t}$.
$$\forall s \in E_3, \red{?c_t}\ (f_s\ s, \red{?f_s'}\ s) = (f_s\ (c_t\ s), \red{?f_s'}\ (c_t\ s))
$$
This task can be regarded as to make the calculation of $f_s$ incremental with respect to modification $c_t$ via $\red{?c_t}$ and $\red{?f_s'}$. Such a problem has also been studied by \citet{lifting} as \textit{lifting problems}. Therefore, \mainname invokes \textit{AutoLifter} again and thus gets a solution where $\red{?f_s'}$ is an empty program and $\red{?c_t} = \lambda s. (s.1 - 1)$. \mainname simplifies this solution by removing the empty component induced by $\red{?f_s'}$, resulting in the solution reported in Figure \ref{fig:overview}.

==> sections/MotivatingExample2-Yingfei.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Overview} \label{section:overview}
In this section, we introduce the main idea of \mainname using a classical COP namely \textit{0/1 knapsack}~\cite{mathews1896partition}. 
\begin{center}
    \it
    Given a set of items, each with a weight $w_i$ and a value $v_i$, put a subset of them in a knapsack of capacity $W$ to get the maximum total value in the knapsack.
\end{center}
For example, $is = [(3, 3), (2, 3), (1, 2)], W = 4$ describes an instance of 0/1 knapsack, where three items are available, their weights are $3, 2, 1$ respectively, their values are $3, 3, 2$ respectively, and the capacity of the knapsack is $4$. At this time, the optimal solution is to put the first and the third items, i.e., $[(3, 3), (1,2)]$, where the value sum is $5$. 

To formally describe this COP, we need to specify (1) the set of valid solutions (in this case, subsets of items whose total weight is within the capacity) and (2) the objective value of each solution (in this case, the total value of each subset). In \mainname, the user writes two programs, $g$ and $o$, to specify the two parts. The program $g$ takes the parameters of the problem (in this case, the list of items \yxcomment{it is better to rename $is$ as it confuses with the English word}) as input and generates all valid solutions for the problem. The program $o$ is an objective function that maps each solution to its objective value.  

Figure~\ref{fig:input} shows the two programs for our example. Function $g$ exhaustively returns all sublists and $o$ calculates the total value of the input list. The first parameter $g$ of function $g$ is itself to enable recursion later with a fixed-point combinator and the second parameter $is$ is the list of items. Functions {\it sumw} and {\it sumv} are used to calculate the sum of the weights and the values for a list of items, respectively. Function {\it cup} is used to flatten a list of lists by concatenating the inner lists.
\yxcomment{I suggest to remove the term "partial solution", and use $s$ to represent a solution.}
\begin{figure}
    \small
    \begin{align*}
        &g =  \lambda g. \lambda is. \text{ if }|is| = 0\text{ then } [[]] \\
        & \hspace{1.6cm} \text{else } \text{let }(\textit{frags}, \textit{rest}) = \textit{ana}\ is \text{ in }\\
        & \hspace{2.25cm}\text{let }\textit{sols} = g \textit{ rest} \text{ in }\\    
        & \hspace{2.25cm}\textit{cup }\big[\textit{cata}\ f\ s\mid f \in \textit{frags}, s \in \textit{sols}\big],\\
        & \quad \textit{where} \\
        & \qquad \textit{ana } is = (\big[[], [\textit{head }is]\big], \textit{tail }is) \\
        & \qquad \textit{cata } f\ s = \left\{
            \begin{array}{ll}
                \,[f\cat s] & \text{if }\textit{sumw}\ f + \textit{sumw}\ s \leq W\\ 
                \,[ ]\, & \text{ otherwise}
            \end{array}\right.\\
        &o =  \lambda p. (\textit{sumv}\ p)
    \end{align*}
    \caption{Example Input Programs \label{fig:input}}        
\end{figure}

% \begin{align*}
%     &g =  \lambda g. \lambda is. \text{ if }|is| = 0\text{ then } [[]] \\
%     & \hspace{1.6cm} \text{else } \text{let }\textit{frags} = [[], [head\ is]] \text{ in }\\
%     & \hspace{2.25cm}\text{let }\textit{sols} = g\ (\textit{tail}\ is) \text{ in }\\    
%     & \hspace{2.25cm}\big[p \cat q \mid p \in \textit{frags}, q \in \textit{sols},\\
%     & \hspace{3.4cm} (\textit{sumw}\ p) + (head\ is).1 \leq W\big] \\
%     &o =  \lambda p. (\textit{sumv}\ p)
% \end{align*}

\mainname requires $g$ to be a (relational) hylomorphism. The above program demonstrates a simplified version of a hylomorphism on list, and the full definition of hylomorphisms can be found in Section~\ref{section:background}. In a nutshell, a hylomorphism consists of two main components: anamorphism ({\it ana}) and catamorphism ({\it cata}). The anamorphism splits the input into two parts ($\textit{head}\ is$ and $\textit{tail}\ is$), processes the first part to produce solution fragments (\textit{frags}). Then $g$ is recursively applied to the second part to produce partial solutions (\textit{sols}). Finally, catamorphism is used to produce a complete solution from each pair of a fragment and a partial solution. 
As mentioned before, hylomorphisms could represent a wide range of programs and can be automatically converted from recursive programs or logic specifications. 

\begin{figure}
    \small \yxcomment{I suggest renaming $m$ to $k$ to represent ``key''.} 
    \begin{alignat*}{2}
        &k &=\,& \lambda is. is \\
        &mem &\,=\,& \lambda m. \lambda is.  \text{ if } \textit{buffer}[k\ is] = \bot \text{ then } \textit{buffer}[k\ is] \leftarrow g\ m\ is;  \\
        &&& \textit{buffer}[k\ is] \\
        &prog &\,=\,& \lambda is. \textit{argmax}\ o\ (\textit{fix}\ mem\ is)
    \end{alignat*}
    \caption{Default Memoization Algorithm \label{fig:default-memoization}}
\end{figure}
    
We can easily build a memoization algorithm based on the two input programs, shown in Figure~\ref{fig:default-memoization}. In the program, $k$ is a function that returns a key for each input argument. Two inputs have the same key only if they lead to the same output. Currently $k$ is the identify function to trivially ensure this property. Function $m$ implements the memoization algorithm and \textit{buffer} is a global map that stores the result for each key. Finally, $prog$ returns the optimal solution from all solutions. Here $argmax\ o\ ps$ chooses the optimal solution in a list of solutions $ps$ based on the objective function $o$, and $\textit{fix}$ is the fixed-point combinator.

% Following studies in program calculus, \mainname requires $P$ to be a relational hylomorphism. For simplicity, in this section, we still use recursive programs to illustrate our main idea. Relational hylomorphisms will be introduced in Section \ref{section:background}.

% In our example, \mainname starts from program $(P_1, S_1, m_1)$ in Figure \ref{fig:overview}, where $P_1$ and $S_1$ are provided by the user to describe the COP, and identity function $m_1$ represents a default way of memoization. Such a program is ineffective, as its time complexity is exponential to the number of items. 

Though $prog$ is already a memoization algorithm, its time complexity is still exponential to the number of items. The goal of our approach is to optimize this inefficient memoization algorithm into an efficient algorithm.

\subsection{Transformation System}

To ensure the optimized program is still a memoization, we retain the recursive and memoization structure and optimize the operations performed within.%, i.e., functions \textit{ana, cata, o} and $k$. 
\newcommand{\nk}{\ensuremath{n_{\textit{keys}}}\xspace}
\newcommand{\szi}{\ensuremath{s_{\textit{in}}}\xspace}
\newcommand{\nf}{\ensuremath{n_{\textit{frags}}(\szi)}\xspace}
\newcommand{\ns}{\ensuremath{n_{\textit{sols}}}\xspace}
\newcommand{\szf}{\ensuremath{s_{\textit{frag}}}\xspace}
\newcommand{\szs}{\ensuremath{s_{\textit{sol}}}\xspace}
\newcommand{\Ta}{\ensuremath{T_{\textit{ana}}}\xspace}
\newcommand{\Tc}{\ensuremath{T_{\textit{cata}}}\xspace}

\begin{figure}
    \begin{align*}
        T(n) &= \nk T_{g}(\szi)\\
        &= \nk \left(\Ta(\szi)+\nf \ns \Tc(\szf, \szs)\right)
    \end{align*}
    
    \footnotesize
    \begin{tabular}{|l|p{3.5cm}|l|l|}
        \hline
        Symbol & Description & Before$^1$ & After$^2$ \\
        \hline
        $n$ & Length of the input list & $O(n)$ & $O(n)$\\
        $\nk$ & Number of keys & $O(n)$ & $O(n)$\\
        $\szi$ & Size of the input to $g$ & $O(n)$ & $O(1)$\\
        $T_g(\szi)$ & Execution time of $g$ excluding the recursive calls & $O(2^n)$ & $O(n)$\\
        $\Ta(\szi)$ & Execution time of {\it ana} & $O(1)$ & $O(1)$\\
        $\nf$ & Number of solution fragments returned by {\it ana} & $O(1)$ & $O(1)$\\
        $\ns$ & Number of partial solutions returned by {\it g}& $O(2^n)$ & $O(n)$\\
        $\szf$ & Size of a fragment & $O(1)$ & $O(1)$\\
        $\szs$ & Size of a solution & $O(n)$ & $O(1)$\\
        $\Tc(\szf+\szs)$ & Execution time of {\it cata} & $O(n)$ & $O(1)$\\
        $T(n)$ & Total time of all invocations & $O(n^2 2^n)$ & $O(n^2)$ \\
        \hline
    \end{tabular}
    {
        1. The time complexity before our optimization. \\
        2. The time complexity after our optimization.
    }
    \caption{Time Complexity of All Invocations to $g$ \label{fig:complexity}}    
\end{figure}

We first analyze the factors affect the performance of \textit{prog} along the recursive structure. Since most of the execution time is spent on $g$, we focus on the total time spent on all invocations to $g$, as shown in Figure~\ref{fig:complexity}. The total time is a product of the execution time of a single invocation to $g$, $T_g(\szi)$, and the number of executions, which is confined by the number of keys, \nk. Within $g$, \textit{ana} is invoked once and \textit{cata} is invoked $\nf \ns$ times. Also, the time complexity of \textit{ana} and \textit{cata} are also decided by the size of their arguments. Therefore, to optimize \textit{prog}, we need to optimize the five factors in the formula: \nk, $\Ta(\szi)$, $\nf$, \ns, and $\Tc(\szf, \szs)$. As we can see, optimizing these factors could reduce the time complexity from $O(n^2 2^n)$ to $O(n^2)$.

% There are four factors that possibly lead to the inefficiency of the input program $(P_1, S_1, m_1)$.
% \begin{enumerate}[leftmargin=*]
% \item $(P_1\ is)$ may return many non-optimal solutions.
% \item The solutions returned by $P\ is$ is a list such that operations on it (e.g.,  calculating $(\textit{sumw}\ p)$) may be costly.
% \item Search state $is$ for $P$ may include redundant information and thus the default memoization may be ineffective.
% \item Search state $is$ is a list such that operations on it (e.g., calculating $(\textit{tail}\ is)$) may be costly.
% \end{enumerate}


% Figure \ref{fig:overview} shows the whole procedure for \mainname to synthesize efficient memoization for this problem, where each row describes one step of the transformation system and the corresponding synthesis task. 
% \begin{itemize}[leftmargin=*]
% \item \textit{Initial Program} lists the program to be optimized.
% \item \textit{Intermediate Program} lists the result of rewriting the initial program with the new program fragments (marked as \red{red}). 
% \item \textit{Example} lists some examples for the fragments, which are extracted from the running procedure on instance $(is, W)$.
% \item \textit{Synthesis Result} lists the assignment to the program fragments found by the synthesizer.  
% \end{itemize}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\textwidth]{fig/overview.png}
    \caption{The running procedure for \mainname to synthesize efficient memoization for 0/1 knapsack}%, where $\textit{sumw}\ is$ and $\textit{sumv}\ is$ calculates the weight sum and the value sum for item list $is$ respectively, and the capacity of the knapsack and the whole item list can be referred via global variable $W$ and $is$ respectively.}
    \label{fig:overview}
\end{figure*}

\yxcomment{The figure should be updated. (1) renaming P, S, m. (2) rewriting the body of P to be consistent with the previous example, as follows.
}
\begin{verbatim}
g = \g. \is. if |is| = 0 then [[]]
    else cup [ if sumw f + sumw s <= W then [f++s] else []
        | f in [[head is], []], s in g (tail is)]
\end{verbatim}   
    


%\mainname optimizes these four factors one by one. 

% \mainname optimizes the four numbers one by one. 
Figure \ref{fig:overview} shows the process of optimizing the example in \mainname. For compactness, we inlined the variables and functions in $g$. As we can see, \mainname has four steps, each optimizes some of the factors.

% to synthesize efficient memoization for this problem, where each row describes one step of the transformation system and the corresponding synthesis task. 
% \begin{itemize}[leftmargin=*]
% \item \textit{Initial Program} lists the program to be optimized.
% \item \textit{Intermediate Program} lists the result of rewriting the initial program with the new program fragments (marked as \red{red}). 
% \item \textit{Example} lists some examples for the fragments, which are extracted from the running procedure on instance $(is, W)$.
% \item \textit{Synthesis Result} lists the assignment to the program fragments found by the synthesizer.  
% \end{itemize}


\noindent \textbf{Step 1}. This step optimizes \ns using \textit{thinning} proposed by \citet{DBLP:journals/mscs/Moor94}. %To distinguish, we use \textit{partial solutions} to denote the solutions constructed by a recursive invocation of generator $P$. A partial solution will be transferred to several \textit{global solutions} for the instance.
Thinning uses a preorder $R$ to represent the dominant relationship between partial solutions returned by the recursive invocation to $g$, where $p_1\ R\ p_2$ represents that partial solution $p_1$ can never lead to the global optimal solution if partial solution $p_2$ exists. If such a preorder exists, the result of $(g\ is)$ can be simplified to $(\textit{thin}\ R\ (g\ is))$, where $\textit{thin}$ returns all local maxima in $(P\ is)$ in the sense of $R$. 

In program $(g_1, o_1, k_1)$, partial solution $p_1$ is dominated by $p_2$ if $p_1$ not only consumes more capacity but also gains smaller value. For any global solution leaded by $p_1$, a better solution can be obtained by replacing items in $p_1$ with $p_2$. Such a relation can be described by the following preorder.
$$
p_1\ R\ p_2 \iff \textit{sumw}\ p_1 \geq \textit{sumw}\ p_2 \wedge \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2
$$

Because the weight sum of partial solutions must be integers in $[0, W]$, the size of $(\textit{thin}\ R\ (P\ is))$ is at most $W + 1$. Therefore, thinning could exponentially reduce \ns if $W$ and $|is|$ are in the same order. Furthermore, for our example, $\textit{thin}\ R$ could be implemented in linear time, and thus does not increase the time complexity. 

As shown in Figure \ref{fig:overview}, \mainname applies thinning by inserting an invocation of \textit{thin} with an unknown preorder $\red{?R}$ to $P_1$, which is found via program synthesis.

\noindent \textbf{Step 2}. This step optimizes $\Tc(\szf, \szs)$ uses \textit{incrementalization}~\cite{DBLP:journals/lisp/LiuS03} to remove costly operations on solution in $(P_2, S_2, m_2)$. 

Concretely, \mainname tries to rewrite all usages of solution $p$ with $(\red{?f_p}\ p)$, where $\red{?f_p}$ is an unknown fragment mapping solutions, which are lists of items, to simpler structures, such as tuples of scalar values. To do so, \mainname identifies all queries (marked as \blue{blue}), which calculate cared values for solutions, and modifications (marked as \green{green}), which generate new solutions, in program $(P_2, S_2, m_2)$ and replaces them with unknown fragments $\red{?q}$ and $\red{?c}$ respectively\footnote{Though $P_2'$ does not return concrete solutions, the optimal solution can be determined by tracing back the calculation that lead to the optimal solution. This is a standard technique, and thus we omit it throughout this paper.}. \mainname uses synthesizers to find proper assignments to these fragments.

\noindent \textbf{Step 3}. To remove redundant information, \mainname synthesizes a new key function $\red{?f_m}$ and thus allows sharing results between different search states of $P$. 

In program $(P_3, S_3, m_3)$, the search state is a list of items. However, only the size of the search states matters, and the contents are redundant, as search states in $P_3$ must be suffixes of the whole item list. \mainname removes this redundancy for memoization by synthesizing $\red{?f_m}$ as $\lambda is. |is|$.

\noindent \textbf{Step 4}. Similar to Step 2, \mainname uses \textit{incrementalization} to remove costly operations on states in program $(P_4, S_4, m_4)$. \mainname tries to rewrite search states with $\red{?f_s}$, related queries with $\red{?q}$, and related modifications with $\red{?c}$. \mainname uses synthesizers to find proper assignments to these fragments.

At last, an efficient program $(P^*, S^*, m^*)$ is obtained.
\begin{itemize}[leftmargin=*]
\item The number of solutions returned by $P^*$ is $O(W)$.
\item After memoization, $P^*$ is invoked at most $O(|is|)$ times.
\item Operators on solutions and states run in constant time.
\end{itemize}
Because function $\textit{thin}$ in $P^*$ can be implemented as linear time, the time complexity of $(P^*, S^*, m^*)$ is $O(W|is|)$. When $W$ and $|is|$ are in the same order, $(P^*, S*, m^*)$ is exponentially faster than the input program $(P_1, S_1, m_1)$. 

\subsection{Specification Extraction for Program Synthesis}
To use synthesizers, a specification on the introduced fragments is necessary. A natural specification here is to ensure the correctness of the transformation result: The resulting program should always find a solution with the largest possible value sum for all instances of 0/1 knapsack.

However, such a specification is too complex for program synthesis, where the synthesis targets are wrapped in the recursive structure of the plan generator $P$. To extract simpler specifications, \mainname decomposes the correctness requirement to each step of the recursion and collects direct examples for the introduced program fragments from the running procedure on concrete instances. 

We still use instance $([(3, 3), (2, 3), (1, 2)], 4)$ of 0/1 knapsack to show how these examples are extracted.

\noindent \textbf{Step 1}. To ensure the correctness of $(P_1', S_1', m_1')$, \mainname requires $\red{?R}$ to satisfy the following two conditions. 
\begin{enumerate}[leftmargin=*]
    \item For any two consecutive invocations $(P_1\ is), (P_1\ (\textit{tail}\ is))$, for any partial solutions $p_1, p_2$ returned by $(P_1\ (\textit{tail}\ is))$, $p_1\ \red{?R}\ p_2$ implies that solutions in $(P_1\ is)$ constructed from $p_1$ are worse than solutions constructed from $p_2$ in $\red{?R}$. 
\item For any set of solutions $ps$, the solution with the largest value sum in $ps$ is always a local maximum in $\red{?R}$.
\end{enumerate}

The first condition ensures that $(P_1'\ is)$ is always equal to $(\textit{thin}\ \red{?R}\ (P_1\ is))$, and the second condition ensures that the solution with the largest value sum is always reserved. Therefore, they together imply the correctness of $(P_1', S_1', m_1')$.

For the first condition, \mainname limits the form of $\red{?R}$ to be $\lambda p_1. \lambda p_2. \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2 \wedge p_1\red{?R'}p_2$, where $\red{?R'}$ is another unknown preorder, and then extracts examples for $\red{?R'}$ according to the second condition.

Let us consider two consecutive invocations $P_x = P\ [(3, 3),
$ $(2,3), (1,2)]$ and $P_y = P\ [(2, 3), (1, 2)]$, and partial solutions $p_1 = [(1, 2)]$ and $p_2 = [(2, 3)]$ generated by $P_y$. In $P_x$, $p_1$ is extended to two solutions $p_{1,1} = [(1, 2)]$ and $p_{1, 2} = [(3, 3), (1, 2)]$, while $p_2$ is extended to $p_{2,1} = [(2, 3)]$ only. 

Note that the value sum of $p_{1,2}$, which is equal to $4$, is larger than the value sum $p_{2,1}$, which is equal to $2$. Therefore, no matter what $\red{R'}$ is, $p_{1, 2}$ is always no worse than $p_{2,1}$ in the sense of $\red{R}$. At this time, according to the second constraint, $p_1$ must be no worse than $p_2$ in the sense of $\red{R}$. In this way, example $\neg ([(1, 2)]\ \red{?R}\ [(2, 3)])$ for preorder $\red{?R}$ is obtained. 

\noindent \textbf{Step 2}. To ensure the correctness of $(P_2', S_2', m_2')$, \mainname requires $\red{?f_p}, \red{?q}$ and $\red{?c}$ to keep the running procedure of $(P_2, S_2, m_2)$ unchanged, except each solution is replaced by the corresponding output of $\red{?f_p}$. At this time, examples can be extracted from the execution of $(P_2, S_2, m_2)$.

Let us consider modification $\green{(\textit{head}\ is):: p}$, which is replaced with $(\red{?c}\ (\textit{head}\ is)\ p)$ in $P_2'$. In $(P_2\ [(3, 3), $ $(2, 3), (1, 2)])$, this modification constructs solution $[(3, 3), (1, 2)]$ from solution $[(1, 2)]$. Because the running procedure is unchanged, we know that there will be a corresponding invocation of $\red{?c}$ where the input is $(3, 3)$ and $\red{?f_p}\ [1, 2]$, and the output is $\red{?f_p}\ [(3, 3), (1, 2)]$. In this way, an example on $\red{?c}$ is obtained. 

\noindent \textbf{Step 3}. To ensure the correctness of $(P_3', S_3', m_3')$, \mainname requires that only search states where the results are exactly the same are mapped into the same key via $\red{?f_m}$.  

Extracting examples for $\red{?f_m}$ is direct. For example, the result of $P_3\ [(2, 3), (1, 2)]$, which is $[(0,0), (1, 2), (2, 3), (3,5)]$, is different from the result of $P_3\ [(1, 2)]$, which is $[(0, 0), (1, 2)]$. Therefore, $\red{?f_m}\ [(2, 3), (1, 2)] \neq \red{?f_m}\ [(1, 2)]$ is obtained.

\textbf{Step 4}. Similar with the Step 2, to ensure the correctness of $(P_4', S_4', m_4')$, \mainname requires $\red{?f_s}, \red{?q}$ and $\red{?c}$ to keep the running procedure of $(P_4, S_4, m_4)$ unchanged, except each state is replaced by the corresponding output of $\red{?f_s}$. The examples here can be extracted similarly with Step 2. 

\subsection{Synthesizing Fragments from Examples}
The four synthesis tasks can be divided into two categories. 

\noindent \textbf{Step 1 and Step 3}. The task in this category is to synthesize a preorder $\red{?R}$ satisfying the following two conditions.
\begin{itemize}[leftmargin=*]
\item (Correctness) $\red{?R}$ satisfies a set of negative examples $(a_i, b_i)$, which represent that $\neg (a_i\red{?R}b_i)$.
\item (Efficiency) The time complexity of the result program should be as small as possible.
\end{itemize}
The synthesis task for Step 3 can be unified into this form because key function $\red{?f_m}$ can be regraded as an equivalence relation for states, which is a special case of preorders.

\mainname synthesizes $R$ in the following form, which is a conjunction of comparisons on several key functions. 
$$
a\ R\ b \iff \wedge_{i} (\red{?key_i}\ a)\ \red{?op_i}\ (\red{?key_i}\ b)
$$
where $\red{?op_i}$ is in $\{\leq, =\}$ and $\{=\}$ in Step 1 and 3 respectively. Besides, for simplicity, we temporarily assume that $\red{?key_i}$ is taken from a finite program space. 

In this form, $\red{?R}$ satisfies a negative example $(a_i, b_i)$ if and only if at least one comparison is evaluated to be false on $(a_i, b_i)$. Therefore, for any preorder that satisfies all examples with $n_c$ comparisons, there must be a comparison that is evaluated to false on at least $1/n_c$ portion of examples. 

Motivated by this property, \mainname synthesizes with a limit $n_c$ on the number of comparisons. While determining the $i$th comparison, only those that are evaluated to false on at least $1/(n_c-i+1)$ portion of examples are considered. In this way, the search space of preorders is greatly reduced. 

To find a preorder leading to an efficient result, \mainname designs objective functions for preorders that approximate the time cost. For Step 1, the objective function comes from the time cost of implementing $\textit{thin}\ R$, which is related to the ranges of the key functions. For Step 3, the objective function is naturally set to the number of equivalence classes of states. Both objective functions increase monotonically while enlarging the set of comparisons such that it can be efficiently optimized via \textit{branch-and-bound}.


%To efficiently find a preorder with a few local minima, \mainname uses the range of each key function to approximate the number of local minima. The following are two examples.
%\begin{itemize}[leftmargin=*]
%\item For the preorder $R$ used in $(P_2, S_2, m_2)$, the number of local minima is at most $\max(\textit{range}(\textit{maxw}), \textit{range}(\textit{maxv}))$. 
%\item For the equivalence relation induced by the key function $m_4$, the number of local minima is at most $\textit{range}(m_4)$.
%\end{itemize}

%On the one hand, such an approximation is effective in practice: It is accurate in both above examples. On the other hand, this approximation monotonically increases while enlarging the set of comparisons such that it can be efficiently optimized via \textit{branch-and-bound}. \rycomment{Make this story consistent with Approach, which starts directly from the time cost instead of approximation.}

\mainname selects $n_c$ and deals with infinite program space by iteration, which will be discussed in Section \ref{section:synthesizer}.

\noindent \textbf{Step 2 and Step 4}. Both of these two tasks are for applying \textit{incrementalization}. The unified characterization of these two tasks refers to functors in the category theory. Therefore, we leave it to Section \ref{section:trans} and illustrate the idea of \mainname using the specific task generated from $(P_4, S_4, m_4)$. 

The task here is about rewriting queries $q_l = \lambda s. |s|$,  $q_h = \lambda s. (\textit{head}\ s)$, and modification $c_t = \lambda s. (\textit{tail}\ s)$. Given three set of examples $E_1, E_2, E_3$, the task is to find $\red{?f_s}, \red{?q_l}, \red{?q_h}$ and $\red{?c_t}$ satisfying the following conditions.
\begin{gather*}
\forall s \in E_1, \red{?q_l}\ (\red{?f_s}\ s) = q_l\ s \qquad 
\forall s \in E_2, \red{?q_h}\ (\red{?f_s}\ s) = q_h\ s \\
\forall s \in E_3, \red{?c_t}\ (\red{?f_s}\ s) = \red{?f_s}\ (c_t\ s)
\end{gather*}

First, the tasks for $q_l$ and $q_r$ are about synthesizing two functions from their composition. These tasks are instances of \textit{partial lifting problems} studied by \citet{lifting}. Therefore, \mainname invokes their approach, \textit{AutoLifter}, on these two tasks and thus gets a solution where $\red{?f_s} = \lambda s. |s|$, $\red{?q_l} = \lambda s. s$ and $\red{?q_h} = \lambda s. is[-s]$.

To make this solution valid for the third task,  \mainname fixes $\red{?f_s}$ to $\red{?f_s}\ s \coloneq (f_s, \red{?f_s'})\ s$, where $f_s$ is $\lambda s. |s|$ found in the previous step. At this time, $\red{?f_s}$, $\red{?q_l} = \lambda s. (s.1)$ and $\red{?q_h} = \lambda s. is[-s.1]$ must be a solution for the first two tasks.

Now, the remaining task is to synthesize $\red{?f_s'}$ and $\red{?c_t}$.
$$\forall s \in E_3, \red{?c_t}\ (f_s\ s, \red{?f_s'}\ s) = (f_s\ (c_t\ s), \red{?f_s'}\ (c_t\ s))
$$
This task can be regarded as to make the calculation of $f_s$ incremental with respect to modification $c_t$ via $\red{?c_t}$ and $\red{?f_s'}$. Such a problem has also been studied by \citet{lifting} as \textit{lifting problems}. Therefore, \mainname invokes \textit{AutoLifter} again and thus gets a solution where $\red{?f_s'}$ is an empty program and $\red{?c_t} = \lambda s. (s.1 - 1)$. \mainname simplifies this solution by removing the empty component induced by $\red{?f_s'}$, resulting in the solution reported in Figure \ref{fig:overview}.

==> sections/MotivatingExample3-Yingfei.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Overview} \label{section:overview}
In this section, we introduce the main idea of \mainname using a classical COP namely \textit{0/1 knapsack}~\cite{mathews1896partition}. 

\smallskip
\parbox{0.9\columnwidth}{\it \noindent 
    Given a set of items, each with a weight $w_i$ and a value $v_i$, put a subset of them in a knapsack of capacity $W$ to get the maximum total value in the knapsack.
}
\smallskip

\noindent For example, $xs = [(3, 3), (2, 3), (1, 2)], W = 4$ describes an instance of 0/1 knapsack, where three items are available, their weights are $3, 2, 1$ respectively, their values are $3, 3, 2$ respectively, and the capacity of the knapsack is $4$. At this time, the optimal solution is to put the first and the third items, i.e., $[(3, 3), (1,2)]$, where the value sum is $5$. 

To formally describe this COP, we need to specify (1) the set of valid solutions (in this case, subsets of items whose total weight is within the capacity) and (2) the objective value of each solution (in this case, the total value of each subset). In \mainname, the user writes two programs, generator $g$ and scorer $o$, to specify the two parts. The generator $g$ takes the parameters of the problem (in this case, the list of items) as input and generates all valid solutions for the problem. The scorer $o$ is an objective function that maps each solution to its objective value.  

%Figure~\ref{fig:input} shows
The code below shows
the two programs for our example. The parameter $g$ of function $g$ is itself to enable recursion later with a fixed-point combinator and the parameter $is$ is the list of items. Functions {\it sumw} and {\it sumv} are used to calculate the sum of weights and values for a list of items, respectively. Given a fixed-point combinator \textit{fix}, $\textit{fix}\ g$ exhaustively returns all sublists, and $o$ calculates the total value of the input list. For simplicity, we shall directly use $g$ to refer to the recursive version, i.e., the first parameter is given. 

{
\vspace{-2mm}
\centering
\small
\begin{align*}
    &g =  \lambda g. \lambda xs. \text{ if }|xs| = 0\text{ then } [[]] \\
    & \qquad \text{else } (g\ (\textit{tail}\ xs)) \cat \\
    &\qquad \quad \big[(head\ xs)::p\ \big|\ p \in g\ (\textit{tail}\ xs), \\
    &\qquad \qquad \quad (\textit{sumw}\ p) + (head\ xs).1 \leq W\big] \\
    &o =  \lambda p. (\textit{sumv}\ p)%\quad m_1 = \lambda is. is
\end{align*}
\vspace{-2mm}
}

%Function {\it concat} is used to flatten a list of lists by concatenating the inner lists.
% \begin{figure}
%     \small
%     \begin{align*}
%         &g =  \lambda g. \lambda xs. \text{ if }|xs| = 0\text{ then } [[]] \\
%         & \hspace{1.6cm} \text{else } \text{let }(\textit{frags}, \textit{rest}) = \textit{ana}\ xs \text{ in }\\
%         & \hspace{2.25cm}\text{let }\textit{sols} = g \textit{ rest} \text{ in }\\    
%         & \hspace{2.25cm}\textit{concat }\big[\textit{cata}\ f\ p\mid f \in \textit{frags}, p \in \textit{sols}\big],\\
%         & \quad \textit{where} \\
%         & \qquad \textit{ana } xs = (\big[[], [\textit{head }xs]\big], \textit{tail }xs) \\
%         & \qquad \textit{cata } f\ s = \left\{
%             \begin{array}{ll}
%                 \,[f\cat p] & \text{if }\textit{sumw}\ f + \textit{sumw}\ p \leq W\\ 
%                 \,[ ]\, & \text{ otherwise}
%             \end{array}\right.\\
%         &o =  \lambda p. (\textit{sumv}\ p)
%     \end{align*}
%     \caption{Example Input Programs \label{fig:input}}        
% \end{figure}

% \begin{figure}
%     \small
% \begin{align*}
%     &g =  \lambda g. \lambda is. \text{ if }|is| = 0\text{ then } [[]] \\
%     & \hspace{1.6cm} \text{else } \text{let }\textit{frags} = [[], [head\ is]] \text{ in }\\
%     & \hspace{2.25cm}\text{let }\textit{sols} = g\ (\textit{tail}\ is) \text{ in }\\    
%     & \hspace{2.25cm}\big[p \cat q \mid p \in \textit{frags}, q \in \textit{sols},\\
%     & \hspace{3.4cm} (\textit{sumw}\ p) + (head\ is).1 \leq W\big] \\
%     &o =  \lambda p. (\textit{sumv}\ p)
% \end{align*}
% \caption{Example Input Programs \label{fig:input}}        
% \end{figure}

% \begin{figure}
%     \small
%     \begin{align*}
%         &g =  \lambda g. \lambda xs. \text{ if }|xs| = 0\text{ then } [[]] \\
%         & \qquad \text{else } (g\ (\textit{tail}\ xs)) \cat \\
%         &\qquad \quad \big[(head\ xs)::p\ \big|\ p \in g\ (\textit{tail}\ xs), (\textit{sumw}\ p) + (head\ xs).1 \leq W\big] \\
%         &o =  \lambda p. (\textit{sumv}\ p)\quad m_1 = \lambda is. is
%         \end{align*}
% \caption{Example Input Programs \label{fig:input}}        
% \end{figure}


\mainname requires $g$ to be a (relational) hylomorphism. The above program demonstrates a simplified version of a hylomorphism on list, and the full definition of hylomorphisms can be found in Section~\ref{section:background}. 
% In a nutshell, a hylomorphism consists of two main components: anamorphism ({\it ana}) and catamorphism ({\it cata}). The anamorphism splits the input into two parts ($\textit{head}\ xs$ and $\textit{tail}\ xs$), processes the first part to produce solution fragments (\textit{frags}). Then $g$ is recursively applied to the second part to produce partial solutions (\textit{sols}). Finally, catamorphism is used to produce a complete solution from each pair of a fragment and a partial solution. 
In a nutshell, a hylomorphism on input type $A$ first produces a value from the input (in this case, \textit{head xs}), then recursively applies itself to another value of type $A$ constructed from the input (\textit{tail xs}), and finally combines the results to form the final result.
As mentioned before, hylomorphisms could represent a wide range of programs and can be automatically converted from recursive programs or logic specifications. 

%To distinguish the input of the outermost invocation to $g$ from other invocations, we call the input of an arbitrary invocation to $g$ a \emph{search state} (or \emph{state}), as an invocation represents a step in a depth-first search.


To distinguish the input and output of the outermost invocation to $g$ and those of other invocations, we call the input of an arbitrary invocation to $g$ a \emph{search state}, as an invocation represents a step in a depth-first search, and call the output of a recursive invocation to $g$ a \emph{partial solution}, as it is not a full solution yet.

% \begin{figure}
%     \small
%     \begin{alignat*}{2}
%         &m &=\,& \lambda xs. xs \\
%         &mem &\,=\,& \lambda mem. \lambda xs.  \text{ if } \textit{buffer}[m\ xs] = \bot \text{ then } \\
%         & && \quad\textit{buffer}[m\ xs] \leftarrow g\ mem\ xs;  \\
%         &&& \textit{buffer}[m\ xs] \\
%         &prog &\,=\,& \lambda xs. \textit{argmax}\ o\ ((\textit{fix}\ mem)\ xs)
%     \end{alignat*}
%     \caption{Default Memoization Algorithm \label{fig:default-memoization}}
% \end{figure}
     
We can easily build a memoization algorithm based on the two input programs, as shown 
%in Figure~\ref{fig:default-memoization}. 
below.
In the program, $m$ is a function that returns a key for each search state. Two states have the same key only if they lead to the same output. Currently, $m$ is the identity function to trivially ensure this property. Function $mem$ implements the memoization algorithm and \textit{buffer} is a global map that stores the result for each key. Finally, $prog$ returns the optimal solution from all solutions. Here $\textit{argmax}\ o\ ps$ chooses the optimal solution in a list of solutions $ps$ based on the objective function $o$, and $\textit{fix}$ is a fixed-point combinator.
\begin{center}
    \vspace{-2mm}
    \small
    \begin{alignat*}{2}
        &m &=\,& \lambda xs. xs \\
        &mem &\,=\,& \lambda mem. \lambda xs.  \text{ if } \textit{buffer}[m\ xs] = \bot \text{ then } \\
        & && \quad\textit{buffer}[m\ xs] \leftarrow g\ mem\ xs;  \\
        &&& \textit{buffer}[m\ xs] \\
        &prog &\,=\,& \lambda xs. \textit{argmax}\ o\ ((\textit{fix}\ mem)\ xs)
    \end{alignat*}
    \vspace{-2mm}
\end{center}


% \begin{figure}
%     \small
%     \begin{alignat*}{2}
%         &m &=\,& \lambda xs. xs \\
%         &mem &\,=\,& \lambda mem. \lambda xs.  \text{ if } \textit{buffer}[m\ xs] = \bot \text{ then } \\
%         & && \quad\textit{buffer}[m\ xs] \leftarrow g\ mem\ xs;  \\
%         &&& \textit{buffer}[m\ xs] \\
%         &prog &\,=\,& \lambda xs. \textit{argmax}\ o\ ((\textit{fix}\ mem)\ xs)
%     \end{alignat*}
%     \caption{Default Memoization Algorithm \label{fig:default-memoization}}
% \end{figure}

% Following studies in program calculus, \mainname requires $P$ to be a relational hylomorphism. For simplicity, in this section, we still use recursive programs to illustrate our main idea. Relational hylomorphisms will be introduced in Section \ref{section:background}.

% In our example, \mainname starts from program $(P_1, S_1, m_1)$ in Figure \ref{fig:overview}, where $P_1$ and $S_1$ are provided by the user to describe the COP, and identity function $m_1$ represents a default way of memoization. Such a program is ineffective, as its time complexity is exponential to the number of items. 

Though the memoization algorithm $prog$ has effectively reused the repeated invocations to $g$, its time complexity is still exponential to the number of items. The goal of our approach is to optimize this inefficient memoization algorithm into an efficient algorithm.

\subsection{Transformation System} 

\newcommand{\nk}{\ensuremath{n_{\textit{keys}}}\xspace}
\newcommand{\szi}{\ensuremath{s_{\textit{st}}}\xspace}
\newcommand{\nf}{\ensuremath{n_{\textit{frags}}(\szi)}\xspace}
\newcommand{\ns}{\ensuremath{n_{\textit{sols}}}\xspace}
\newcommand{\szf}{\ensuremath{s_{\textit{frag}}}\xspace}
\newcommand{\szs}{\ensuremath{s_{\textit{sol}}}\xspace}
\newcommand{\Ta}{\ensuremath{T_{\textit{ana}}}\xspace}
\newcommand{\Tc}{\ensuremath{T_{\textit{cata}}}\xspace}

% \begin{figure}
%     \begin{align*}
%         T(n) &= \nk T_{g}(\szi)\\
%         &= \nk \left(\Ta(\szi)+\nf \ns \Tc(\szf, \szs)\right)
%     \end{align*}
    
%     \footnotesize
%     \begin{tabular}{|l|p{3.5cm}|l|l|}
%         \hline
%         Symbol & Description & Before$^1$ & After$^2$ \\
%         \hline
%         $n$ & Length of the input list & $O(n)$ & $O(n)$\\
%         $\nk$ & Number of keys & $O(n)$ & $O(n)$\\
%         $\szi$ & Size of the input to $g$ & $O(n)$ & $O(1)$\\
%         $T_g(\szi)$ & Execution time of $g$ excluding the recursive calls & $O(2^n)$ & $O(n)$\\
%         $\Ta(\szi)$ & Execution time of {\it ana} & $O(1)$ & $O(1)$\\
%         $\nf$ & Number of solution fragments returned by {\it ana} & $O(1)$ & $O(1)$\\
%         $\ns$ & Number of partial solutions returned by {\it g}& $O(2^n)$ & $O(n)$\\
%         $\szf$ & Size of a fragment & $O(1)$ & $O(1)$\\
%         $\szs$ & Size of a solution & $O(n)$ & $O(1)$\\
%         $\Tc(\szf+\szs)$ & Execution time of {\it cata} & $O(n)$ & $O(1)$\\
%         $T(n)$ & Total time of all invocations & $O(n^2 2^n)$ & $O(n^2)$ \\
%         \hline
%     \end{tabular}
%     {
%         1. The time complexity before our optimization. \\
%         2. The time complexity after our optimization.
%     }
%     \caption{Time Complexity of All Invocations to $g$ \label{fig:complexity}}    
% \end{figure}

% To ensure the optimized program is still a memoization, we retain the recursive and memoization structure and optimize the operations performed within.
% We first analyze the factors affect the performance of \textit{prog}. 
% Since most of the execution time is spent on $g$, we focus on the total time spent on all invocations to $g$, as shown in Figure~\ref{fig:complexity}. The total time is a product of the execution time of a single invocation to $g$, $T_g(\szi)$, and the number of executions, which is confined by the number of keys, \nk. Within $g$, \textit{ana} is invoked once and \textit{cata} is invoked $\nf \ns$ times. Also, the time complexity of \textit{ana} and \textit{cata} are also decided by the size of their arguments. Therefore, to optimize \textit{prog}, we need to optimize the five factors in the formula: \nk, $\Ta(\szi)$, $\nf$, \ns, and $\Tc(\szf, \szs)$. As we can see, optimizing these factors could reduce the time complexity from $O(n^2 2^n)$ to $O(n^2)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We first analyze the factors that affect the performance of $g$, the function consuming most of the execution time. The time complexity of $g$ is as follows.
\[
    O\left(\nk \left(\szi+ \ns \szs\right)\right)
\] 
Here \nk denotes the number of keys that $m$ could possibly return, \ns denotes the number of solutions returned by a recursive call, \szi denotes the size of the search state, and \szs denote the size of a partial solution.
The execution time of $g$ is a product of the number of invocations and the execution time of a single invocation excluding the recursive call. The former is further confined by \nk. The latter consists of the execution time of processing the input ($|xs|$ takes $O(n)$) and the execution time of producing the solution, where there are $\ns$ solutions, and each takes $O(\szs)$ to process. Though this analysis is specific to this input program, the four variables also dominate the performance in general cases.

Our approach reduces the four variables in the above formula, namely, \ns, \szs, \nk, \szi. Our goal is to reduce \szs and \szi to $O(1)$, and reduce \ns and \nk as much as possible.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We first introduce two assumptions on \textit{ana} and \textit{cata}: (1) the time complexity of \textit{ana} and \textit{cata} are polynomial to their inputs, and (2) the total size of solution fragments returned by \textit{ana} has constant complexity. The two assumptions are reasonable because operations with exponential or higher time complexity would be handled with the recursive structure. 

% Based on the two assumptions, the time complexity of $g$ is as follows.
% \[
%     O\left(\nk \left(\Ta(\szi)+ \ns \Tc(\szs)\right)\right)
% \] 
% %Here $T(n)$ represents the time complexity of $g$ and $n$ represents the length of the input list. 
% Here \nk denotes the number of keys that $k$ could possibly return, \ns denotes the number of solutions returned by a recursive call, \szi denotes the size of the search state, \szs denote the size of a partial solution, \Ta denotes the time complexity function of \textit{ana}, and \Tc denotes the time complexity function of \textit{cata}.
% The execution time of $g$ is a product of the number of invocations and the execution time of a single invocation excluding the recursive call. The former is further confined by \nk. The latter consists of the execution time of \textit{ana} and the invocations to \textit{cata}. Please note that the size and number of solution fragments are constant and thus do not affect the complexity.

% Our approach reduces the four variables in the above formula, namely, \ns, \szs, \nk, \szi. Our goal is to reduce \szs and \szi to $O(1)$. Since \Ta and \Tc are polynomial, the total time complexity becomes $O(\nk\ns)$. For the remaining two variables, we reduce them as much as possible.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% To ensure the optimized program is still a memoization, we retain the recursive and memoization structure and optimize the operations performed within.
% We first analyze the factors affect the performance of \textit{prog}. 
% Most of the execution time is spent on the invocations to $g$, where the total time is a product of the number of invocations and the execution time of a single invocation excluding the recursive call. 
% The former is further confined by the number of keys that $k$ could possibly return. 
% The latter is a function over the scale of the input to $g$. For a single invocation excluding the recursive call, the input includes the search state $is$, and the list of partial solutions returned from the recursive call. 
% Therefore, the execution time of $g$ is affected by the factors controlling the scale of the input. Putting together, we identify four factors affecting the performance of \textit{prog}, as follows.
% \begin{tabular}{|l|p{7cm}|}
%     \hline
%     \ns & the number of partial solutions returned by an invocation to $g$\\
%     \szs & the size of a partial solution\\
%     \nk & the number of keys that $k$ could possibly return\\
%     \szi & the size of a search state\\
%     \hline
% \end{tabular}\\
% Note that the four factors do not cover all places that we can optimize. For example, the time complexity of $g$ is not only controlled by the scale of the input but also how $g$ is implemented. However, as our evaluation would show later, optimizing the four factors could lead to satisfactory results in most cases. For our example program, \mainname can reduce the time complexity from exponential to linear.



\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\textwidth]{fig/overview2.png}
    \caption{The running procedure for \mainname to synthesize efficient memoization for 0/1 knapsack}%, where $\textit{sumw}\ is$ and $\textit{sumv}\ is$ calculates the weight sum and the value sum for item list $is$ respectively, and the capacity of the knapsack and the whole item list can be referred via global variable $W$ and $is$ respectively.}
    \label{fig:overview}
\end{figure*}

%\yxcomment{The figure should be updated. (1) renaming P, S, m. (2) adding the parameter g. (3) replacing $f_p$. (4) rewriting the body of P to be consistent with the previous example, as follows. (5) removing colors for distinguishing modifications and queries.
%}
%\begin{verbatim}
%    g = \g. \is. if |is| = 0 then [[]]
%        else cup [ if sumw f + sumw s <= W then [f++s] else []
%            | f in [[head is], []], s in g (tail is)]
%    \end{verbatim}   
    
Figure \ref{fig:overview} shows the process of optimizing our example in \mainname. %For compactness, we inlined the variables and functions in $g$ and made a slight simplification. 
For simplicity, we omit the first parameter of $g$.
\mainname has four steps, each optimizes one variable. 

% to synthesize efficient memoization for this problem, where each row describes one step of the transformation system and the corresponding synthesis task. 
% \begin{itemize}[leftmargin=*]
% \item \textit{Initial Program} lists the program to be optimized.
% \item \textit{Intermediate Program} lists the result of rewriting the initial program with the new program fragments (marked as \red{red}). 
% \item \textit{Example} lists some examples for the fragments, which are extracted from the running procedure on instance $(is, W)$.
% \item \textit{Synthesis Result} lists the assignment to the program fragments found by the synthesizer.  
% \end{itemize}


\noindent \textbf{Step 1}. This step optimizes \ns, the number of partial solutions, using the \textit{thinning} method proposed by \citet{DBLP:journals/mscs/Moor94}. %To distinguish, we use \textit{partial solutions} to denote the solutions constructed by a recursive invocation of generator $P$. A partial solution will be transferred to several \textit{global solutions} for the instance.
Thinning uses a preorder $R$ to represent the dominant relationship between partial solutions returned by the recursive invocation to $g$, where $p_1Rp_2$ represents that partial solution $p_1$ can never lead to the global optimal solution if $p_2$ exists. If such a preorder exists, the result of $(g\ xs)$ can be simplified to $(\textit{thin}\ R\ (g\ xs))$, where $\textit{thin}$ is a function returning all minimal values in $(g\ xs)$ in the sense of $R$. 

In program $(g_1, o_1, m_1)$, partial solution $p_1$ is dominated by $p_2$ if $p_1$ not only consumes more capacity but also gains smaller value. For any global solution leaded by $p_1$, a better solution can be obtained by replacing items in $p_1$ with $p_2$. Such a relation can be described by the following preorder.
$$
p_1Rp_2 \iff \textit{sumw}\ p_1 \geq \textit{sumw}\ p_2 \wedge \textit{sumv}\ p_1 \leq \textit{sumv}\ p_2
$$

Because the weight sum of partial solutions must be an integer in $[0, W]$, the size of $(\textit{thin}\ R\ (P\ xs))$ is at most $W + 1$. %Therefore, thinning could exponentially reduce \ns if $W$ and $|is|$ are in the same order. 
Since normally $W$ and $|xs|$ are in the same order, thinning could reduce the complexity of \ns from exponential to polynomial. 
Furthermore, for our example, $\textit{thin}\ R$ could be implemented in linear time, and thus does not increase the time complexity. 

As shown in Figure \ref{fig:overview}, \mainname applies thinning by inserting an invocation of \textit{thin} with an unknown preorder $\red{?R}$ to $g_1$, which is found via program synthesis.

\noindent \textbf{Step 2}. This step optimizes \szs, the size of a partial solution, using \textit{incrementalization} proposed by \citet{DBLP:journals/lisp/LiuS03}. % to remove costly operations on solution in $(P_2, S_2, m_2)$. 
The goal of incrementalization is to change the representation of a solution from a list to another data structure, so that \szs could be reduced. 

To achieve this goal, \mainname identifies all functions in the original program that access a solution, i.e., either take a solution as input or return a solution as output. Then \mainname synthesize new functions to replace them. The new function could take/return a new data type, and thus effectively change the representation. 

In this example, \mainname would use a tuple of scalar values, the sum of weights and the sum of values, to replace the list for representing a partial solution. Thus, \szs reduces to $O(1)$.

Note that a COP may require to return a concrete solution. After changing the representation, the optimal solution can be determined by tracing back the calculation that leads to the optimal solution. This is a standard technique, and thus we omit it throughout this paper.

As will be discussed later, our synthesis algorithm is inductive and relies on runtime values collected from the execution of the original program. Since the collected solutions are in the original representation, we synthesize a \emph{converting function} $\red{?f_p}$ that converts a solution from the original representation to the new representation.

% To achieve this goal, \mainname tries to wrap all expressions accessing a solution, and synthesize new expressions to replace them. In particular, \mainname identifies two types of expressions: \emph{modifications} (marked as \green{green}), which are maximal expressions returning a solution, and \emph{queries} (marked as \blue{blue}), which are minimal expression taking a solution as input and returning a tuple of scalar value. \yxcomment{The definitions of modification and query are probably wrong. The expressions returning a solution include a single variable.}
% Since a generator rarely constructs another data structure from a solution, the two types effectively cover all expressions accessing a solution. 
% \mainname replaces modifications and queries with unknown fragments $\red{?q}$ and $\red{?c}$ respectively, and uses synthesizers to find proper assignments to these fragments.\footnote{Though $g_2'$ does not return concrete solutions, the optimal solution can be determined by tracing back the calculation that lead to the optimal solution. This is a standard technique, and thus we omit it throughout this paper.}


% Concretely, \mainname tries to rewrite all usages of solution $p$ with $(\red{?f_p}\ p)$, where $\red{?f_p}$ is an unknown fragment mapping solutions, which are lists of items, to simpler structures, such as tuples of scalar values. To do so, \mainname identifies all queries (marked as \blue{blue}), which calculate cared values for solutions, and modifications (marked as \green{green}), which generate new solutions, in program $(P_2, S_2, m_2)$ and replaces them with unknown fragments $\red{?q}$ and $\red{?c}$ respectively\footnote{Though $P_2'$ does not return concrete solutions, the optimal solution can be determined by tracing back the calculation that lead to the optimal solution. This is a standard technique, and thus we omit it throughout this paper.}. \mainname uses synthesizers to find proper assignments to these fragments.

\noindent \textbf{Step 3}. This step optimizes \nk, the number of keys that $k$ possibly returns. \mainname synthesizes a new key function $\red{?f_m}$ to replace the original function.
%To remove redundant information, \mainname synthesizes a new key function $\red{?f_m}$ and thus allows sharing results between different search states of $P$. 

In program $(g_3, o_3, m_3)$, the search state is a list of items, but only the size of the search state matters. %However, only the size of the search states matters, as search states must be suffixes of the whole item list. 
\mainname synthesizes $\red{?f_m}$ as $\lambda xs. |xs|$. Note that though \nk is not reduced in this example, the synthesized key function still optimizes the program as comparing two keys requires $O(1)$ instead of $O(n)$, where $n$ represents the number of the items.

\noindent \textbf{Step 4}. This step optimizes \szi, the size of a search state. Similar to Step 2, \mainname uses \textit{incrementalization} to find a new representation for the search state. In this example, \mainname would use the length of the list to represent a search state, reducing \szi from $O(n)$ to $O(1)$. 

%to remove costly operations on states in program $(P_4, S_4, m_4)$. \mainname tries to rewrite search states with $\red{?f_s}$, related queries with $\red{?q}$, and related modifications with $\red{?c}$. \mainname uses synthesizers to find proper assignments to these fragments.

At last, an efficient program $(g^*, o^*, m^*)$ is obtained. Under the assumption that $|xs|$ and $W$ are in the same order,
%each invocation to $g^*$ returns $O(n)$ solution, the size of the solutions and the search states are constant, and $g^*$ is invoked $O(n)$ times. Therefore, the total time complexity is $O(n^2)$. 
$\szi=\szs=O(1)$ and $\nk=\ns=O(n)$ in this program, and thus the total time complexity is $O(n^2)$.
% \begin{itemize}[leftmargin=*]
% \item The number of solutions returned by $P^*$ is $O(W)$.
% \item After memoization, $P^*$ is invoked at most $O(|is|)$ times.
% \item Operators on solutions and states run in constant time.
% \end{itemize}
% Because function $\textit{thin}$ in $P^*$ can be implemented as linear time, the time complexity of $(P^*, S^*, m^*)$ is $O(W|is|)$. When $W$ and $|is|$ are in the same order, $(P^*, S*, m^*)$ is exponentially faster than the input program $(P_1, S_1, m_1)$. 

\subsection{Correctness Specification Extraction for Program Synthesis}
A basic correctness specification is that the new program should be equivalent to the input program. However, such a specification is too complex for program synthesis. To solve this problem, we decompose the correctness requirement for each synthesis task.

\noindent \textbf{Step 1}. To ensure the correctness of $(g_1', o_1', m_1')$, \mainname requires $\red{?R}$ to satisfy the following two conditions. 
\begin{enumerate}[leftmargin=*]
    \item Let $p \twoheadrightarrow_s p'$ denote a partial solution $p'$ for state $s$ is constructed from another solution $p$. Let $(g_1\ xs), (g_1\ (\textit{tail}\ xs))$ be two consecutive invocations, $p_1, p_2 \in g_1\ (\textit{tail}\ xs)$ and $p_1' \in (g_1\ xs)$ be three solutions returned by the two invocations such that $p_1 \twoheadrightarrow_{\textit{xs}} p_1'$. The following condition holds.
    % \begin{equation*}  \forall p_1', \big(p_1 \twoheadrightarrow_{\textit{xs}} p_1' \rightarrow \exists \ p_2', \big(p_2 \twoheadrightarrow_{\textit{xs}} p_2' \wedge p_1'\red{?R}p_2'\big)\big)\end{equation*}
    \begin{equation*}p_1\red{?R}p_2 \rightarrow \exists p_2' \in (g_1\ xs),\ p_2 \twoheadrightarrow_{\textit{xs}} p_2' \wedge p_1'\red{?R}p_2'\label{formula:spec-s1}\end{equation*}
    % which requires partial solutions constructed from $p_1$ to be smaller than those constructed from $p_2$ in $\red{?R}$.
    %\item Let $p \twoheadrightarrow p'$ denote a solution $p'$ is constructed from another solution $p$. Let $(g_1\ xs), (g_1\ (\textit{tail}\ xs))$ be two consecutive invocations, $p_1, p_2 \in g_1\ (\textit{tail}\ xs)$ and $p_1' \in (g_1\ xs)$ be three solutions returned by the two invocations. The following condition holds. \begin{equation}p_1\red{?R}p_2 \implies \exists p_2' \in (g_1\ xs),\ p_2 \twoheadrightarrow p_2' \wedge p_1'\red{?R}p_2'\label{formula:spec-s1}\end{equation}
    % \item For any two consecutive invocations $(g_1\ is), (g_1\ (\textit{tail}\ is))$, any two partial solutions $p_1, p_2 \in g_1\ (\textit{tail}\ is)$ such that $p_1\ \red{?R}\ p_2$, and any $p_1' \in (g_1\ is)$ that is constructed from $p_1$, there exists $p_2' \in (g_1\ is)$ that is constructed from $p_2$ and $p_1'\ \red{?R}\ p_2'$.
    \item For any set of solutions $ps$, the solution with the largest objective value in $ps$ is always maximal in $\red{?R}$.
\end{enumerate}

The first condition ensures that $(g_1'\ xs)$ is always equal to $(\textit{thin}\ \red{?R}\ (g_1\ xs))$, and the second condition ensures that the solution with the largest objective value is always reserved. Therefore, they together imply the correctness of $(g_1', o_1', m_1')$.

To ensure the second condition, \mainname limits the form of $\red{?R}$ to be $\lambda p_1. \lambda p_2. \textit{o}\ p_1 \leq \textit{o}\ p_2 \wedge p_1\red{?R'}p_2$, where $\red{?R'}$ is another unknown preorder, and then requires only the first condition.% on $\red{?R'}$.

\noindent \textbf{Step 2 and Step 4}. %The correctness specification for these two steps are simple. The synthesized function should produce the same output for the same input as the original version. 
In these two steps, the synthesized function should behave the same as the original function. However, since the input and output type of the synthesized function may be different from the original version, we rely on the synthesized converting function for the comparison. Suppose $A$ is the type to be replaced and $\red{?f_p}$ is the converting function to be synthesized. For example, given a function $q$ taking $A$ as input, the synthesized function $\red{?q}$ should satisfy $\red{?q}\circ \red{?f_p} = q$. Similarly, given a function $c$ producing $A$ as output, the synthesized function $\red{?c}$ should satisfy $\red{?c} = \red{?f_p} \circ q$.

\noindent \textbf{Step 3}. To ensure the correctness of $(g_3', o_3', m_3')$, \mainname requires that $\red{?f_m}$ maps two search states $is_1$ and $is_2$ to the same key only if $(g_3\ xs_1)$ and $(g_3\ xs_2)$ are exactly the same:
\begin{equation*}\red{?f_m}\ xs_1 = \red{?f_m}\ xs_2 \rightarrow g_3\ xs_1 = g_3\ xs_2\end{equation*}

\smallskip
Our synthesis algorithms use inductive synthesis~\cite{DBLP:journals/acta/JhaS17}, and thus we need to collect examples for synthesis. To make the synthesis effective, the examples should reflect a situation that could possibly appear during the program execution. Therefore, we randomly generate inputs to the whole program, and collect runtime values related to the specification.
%satisfy two criteria: (1) the examples should reflect a situation that could possibly appear during the program execution, and (2) an example should constrain the program space, i.e., not all programs can satisfy the example. 

%To satisfy the first requirement, we randomly generate inputs to the whole program, and collect runtime values.

To enable efficient synthesis for Step 1 and Step 3, we eliminate the logical implication in their specifications and collect simpler examples for $\red{?R}$ and $\red{?f_m}$. 

%For Step 1, since a part of $\red{?R}$ has been fixed to $\lambda p_1. \lambda p_2$ by the second condition, $\red{?R}$ has the following property.
For Step 1, the fixed form of $\red{?R}$ implies the following property.
$$\forall p_1, p_2, (o\ p_1 > o\ p_2) \rightarrow \neg p_1 \red{?R} p_2$$
With the first condition, we obtain the following formula.
% \begin{align*}
% \exists p_1',\big(p_1 \twoheadrightarrow_{\textit{xs}}p_1' \wedge \forall p_2', (p_2 \twoheadrightarrow_{\textit{xs}} p_2' \rightarrow (o\ p_1 > o\ p_2))\big)&\\  \rightarrow \neg p_1\red{?R}p_2&
% \end{align*}
$$\left(\forall p_2' \in (g_1\ xs), \neg p_2 \twoheadrightarrow_{\textit{xs}} p_2' \vee o\ p_1' > o\ p_2'\right) \rightarrow \neg p_1 \red{?R} p_2$$
The premise of the implication does not contain $\red{?R}$, and thus we can collect all pairs of partial solutions $(p_1, p_2)$ where there exists $p_1'$ to satisfy the premise. In this way, we obtain a set of negative examples. Note that when other parts of $\red{?R}$ are synthesized, \mainname will collect a new set of examples similarly. More details can be found in Section \ref{section:psolver}.

%we can collect examples only when the premise is satisfied. In this way, a set of negative examples of $\red{?R}$ is obtained. 

%To satisfy the second requirement, we adopt different strategies for different steps. For step 1, we notice that the form of $\red{?R}$ implies the following property. 
%$$\forall p_1, p_2, o\ p_1 > o\ p_2 \implies \neg p_1 \red{?R} p_2$$
%Combining this with the first condition, we obtain the following condition.
%$$\left(\forall p_2' \in (g_1, is), \neg p_2 \twoheadrightarrow p_2' \vee o\ p_1 > o\ p_2\right) \implies \neg p_1 \red{?R} p_2$$
%The premise of the implication does not contain the synthesized relation, and thus we can collect consecutive invocations to $g_1$ where the returned solutions satisfy the premise. In this way, we obtain a set of negative examples. 

%For steps 2 and 4, we directly collect the inputs to the function being replaced. 
 
For Step 3, we transform the original condition to the following equivalent form.
$$g_3\ \textit{xs}_1 \neq g_3\ \textit{xs}_2 \rightarrow \red{?f_m}\ \textit{xs}_1 \neq \red{?f_m}\ \textit{xs}_2$$
Same as Step 1, the premise of the implication does not contain the synthesized function, and we can collect search state pairs that satisfy the premise. %Note that $\red{?f_m}$ induces a preorder $\red{?R_m}$ where $\textit{xs}_1\red{?R_m}\textit{xs}_2 \iff \red{?f_m}\ \textit{xs}_1 = \red{?f_m}\ \textit{xs}_2$. At this time, the examples for $\red{?f_m}$ can be regarded as negative examples for preorder $\red{?R_m}$. In this way, this synthesis task can be unified with the task of Step 1.

% To use synthesizers, a specification on the introduced fragments is necessary. A natural specification here is to ensure the correctness of the transformation result: The resulting program should always find a solution with the largest possible value sum for all instances of 0/1 knapsack.

% However, such a specification is too complex for program synthesis, where the synthesis targets are wrapped in the recursive structure of the plan generator $P$. To extract simpler specifications, \mainname decomposes the correctness requirement to each step of the recursion and collects direct examples for the introduced program fragments from the running procedure on concrete instances. 

% We still use instance $([(3, 3), (2, 3), (1, 2)], 4)$ of 0/1 knapsack to show how these examples are extracted.

% \noindent \textbf{Step 1}. To ensure the correctness of $(P_1', S_1', m_1')$, \mainname requires $\red{?R}$ to satisfy the following two conditions. 
% \begin{enumerate}[leftmargin=*]
%     \item For any two consecutive invocations $(P_1\ is), (P_1\ (\textit{tail}\ is))$, for any partial solutions $p_1, p_2$ returned by $(P_1\ (\textit{tail}\ is))$, $p_1\ \red{?R}\ p_2$ implies that solutions in $(P_1\ is)$ constructed from $p_1$ are worse than solutions constructed from $p_2$ in $\red{?R}$. 
% \item For any set of solutions $ps$, the solution with the largest value sum in $ps$ is always a local maximum in $\red{?R}$.
% \end{enumerate}

% The first condition ensures that $(P_1'\ is)$ is always equal to $(\textit{thin}\ \red{?R}\ (P_1\ is))$, and the second condition ensures that the solution with the largest value sum is always reserved. Therefore, they together imply the correctness of $(P_1', S_1', m_1')$.

% For the second condition, \mainname limits the form of $\red{?R}$ to be $\lambda p_1. \lambda p_2. \textit{o}\ p_1 \leq \textit{o}\ p_2 \wedge p_1\red{?R'}p_2$, where $\red{?R'}$ is another unknown preorder, and then extracts examples for $\red{?R'}$ according to the first condition.

% Let us consider two consecutive invocations $P_x = P\ [(3, 3),
% $ $(2,3), (1,2)]$ and $P_y = P\ [(2, 3), (1, 2)]$, and partial solutions $p_1 = [(1, 2)]$ and $p_2 = [(2, 3)]$ generated by $P_y$. In $P_x$, $p_1$ is extended to two solutions $p_{1,1} = [(1, 2)]$ and $p_{1, 2} = [(3, 3), (1, 2)]$, while $p_2$ is extended to $p_{2,1} = [(2, 3)]$ only. 

% Note that the value sum of $p_{1,2}$, which is equal to $4$, is larger than the value sum $p_{2,1}$, which is equal to $2$. Therefore, no matter what $\red{R'}$ is, $p_{1, 2}$ is always no worse than $p_{2,1}$ in the sense of $\red{R}$. At this time, according to the second constraint, $p_1$ must be no worse than $p_2$ in the sense of $\red{R}$. In this way, example $\neg ([(1, 2)]\ \red{?R}\ [(2, 3)])$ for preorder $\red{?R}$ is obtained. 

% \noindent \textbf{Step 2}. To ensure the correctness of $(P_2', S_2', m_2')$, \mainname requires $\red{?f_p}, \red{?q}$ and $\red{?c}$ to keep the running procedure of $(P_2, S_2, m_2)$ unchanged, except each solution is replaced by the corresponding output of $\red{?f_p}$. At this time, examples can be extracted from the execution of $(P_2, S_2, m_2)$.

% Let us consider modification $\green{(\textit{head}\ is):: p}$, which is replaced with $(\red{?c}\ (\textit{head}\ is)\ p)$ in $P_2'$. In $(P_2\ [(3, 3), $ $(2, 3), (1, 2)])$, this modification constructs solution $[(3, 3), (1, 2)]$ from solution $[(1, 2)]$. Because the running procedure is unchanged, we know that there will be a corresponding invocation of $\red{?c}$ where the input is $(3, 3)$ and $\red{?f_p}\ [1, 2]$, and the output is $\red{?f_p}\ [(3, 3), (1, 2)]$. In this way, an example on $\red{?c}$ is obtained. 

% \noindent \textbf{Step 3}. To ensure the correctness of $(P_3', S_3', m_3')$, \mainname requires that only search states where the results are exactly the same are mapped into the same key via $\red{?f_m}$.  

% Extracting examples for $\red{?f_m}$ is direct. For example, the result of $P_3\ [(2, 3), (1, 2)]$, which is $[(0,0), (1, 2), (2, 3), (3,5)]$, is different from the result of $P_3\ [(1, 2)]$, which is $[(0, 0), (1, 2)]$. Therefore, $\red{?f_m}\ [(2, 3), (1, 2)] \neq \red{?f_m}\ [(1, 2)]$ is obtained.

% \textbf{Step 4}. Similar with the Step 2, to ensure the correctness of $(P_4', S_4', m_4')$, \mainname requires $\red{?f_s}, \red{?q}$ and $\red{?c}$ to keep the running procedure of $(P_4, S_4, m_4)$ unchanged, except each state is replaced by the corresponding output of $\red{?f_s}$. The examples here can be extracted similarly with Step 2. 

\subsection{Synthesizing Fragments from Examples}
The four synthesis tasks can be divided into two categories. 

\noindent \textbf{Step 1 and Step 3}. The task in this category is to synthesize a preorder $\red{?R}$ satisfying a set of negative examples $(a_i, b_i)$ such that $\neg (a_i\red{?R}b_i)$ holds. The synthesis task for Step 3 can be unified into this form because key function $\red{?f_m}$ can be regarded as an equivalence relation for states, which is a special case of preorders.

% The task in this category is to synthesize a preorder $\red{?R}$ satisfying the following two conditions.
% \begin{itemize}[leftmargin=*]
% \item (Correctness) $\red{?R}$ satisfies a set of negative examples $(a_i, b_i)$, which represent that $\neg (a_i\red{?R}b_i)$.
% \item (Efficiency) The time complexity of the result program should be as small as possible.
% \end{itemize}
% The synthesis task for Step 3 can be unified into this form because key function $\red{?f_m}$ can be regraded as an equivalence relation for states, which is a special case of preorders.

\mainname uses an iterative synthesis algorithm to solve this task. To optimize the efficiency of the synthesis algorithm,
\mainname synthesizes $\red{?R}$ in the following form, which is a conjunction of comparisons on several key functions. 
$$
a\ R\ b \iff \wedge_{i} (\red{?key_i}\ a)\ \red{?op_i}\ (\red{?key_i}\ b)
$$
where $\red{?op_i}$ is in $\{\leq, =\}$ and $\{=\}$ in Step 1 and 3 respectively. %Besides, for simplicity, we temporarily assume that $\red{?key_i}$ is taken from a finite program space. 

In this form, $\red{?R}$ satisfies a negative example $(a_i, b_i)$ if and only if at least one comparison is evaluated to be false on $(a_i, b_i)$. Therefore, for any preorder that satisfies all examples with $n_c$ comparisons, there must be a comparison that is evaluated to false on at least $1/n_c$ portion of examples. 

Motivated by this property, \mainname synthesizes with a limit $n_c$ on the number of comparisons. While determining the $i$th comparison, only those that are evaluated to false on at least $1/(n_c-i+1)$ portion of examples are considered. In this way, the search space of preorders is greatly reduced. 

Besides satisfying the correctness specification, the other goal of synthesis is to minimize \ns and \nk. We design two objective functions to estimate the effects of the synthesized preorder on minimizing the two variables and then optimize the objective functions via \textit{branch-and-bound}, a commonly used method to solve synthesis problems with an optimization goal~\cite{DBLP:journals/pacmpl/JiS0H20, DBLP:conf/pldi/LeeHAN18}.  

% To find a preorder leading to an efficient result, \mainname designs objective functions for preorders that approximate the time cost. For Step 1, the objective function comes from the time cost of implementing $\textit{thin}\ R$, which is related to the ranges of the key functions. For Step 3, the objective function is naturally set to the number of equivalence classes of states. Both objective functions increase monotonically while enlarging the set of comparisons such that it can be efficiently optimized via \textit{branch-and-bound}.


%To efficiently find a preorder with a few local minima, \mainname uses the range of each key function to approximate the number of local minima. The following are two examples.
%\begin{itemize}[leftmargin=*]
%\item For the preorder $R$ used in $(P_2, S_2, m_2)$, the number of local minima is at most $\max(\textit{range}(\textit{maxw}), \textit{range}(\textit{maxv}))$. 
%\item For the equivalence relation induced by the key function $m_4$, the number of local minima is at most $\textit{range}(m_4)$.
%\end{itemize}

%On the one hand, such an approximation is effective in practice: It is accurate in both above examples. On the other hand, this approximation monotonically increases while enlarging the set of comparisons such that it can be efficiently optimized via \textit{branch-and-bound}. \rycomment{Make this story consistent with Approach, which starts directly from the time cost instead of approximation.}

% \mainname selects $n_c$ and deals with infinite program space by iteration, which will be discussed in Section \ref{section:synthesizer}.

%\todo{mod}
\noindent \textbf{Step 2 and Step 4}. In this task, we need to synthesize a series of functions, where each function is independently specified except for the converting function $\red{?f}$, which is shared in all specifications. %To solve the problem, we first assume the function $\red{?f}$ takes the form of $\lambda a. (f_1 a,\ldots, f_n a)$. Then we solve each specification as an independent synthesis problem, and then combine the synthesized converting functions into $\red{?f}$ by treating each one as a component $f_i$ in the above form. 
These specifications follow the same form, which requires the composition of an unknown function and $\red{?f}$ to be equal to some known function or the composition of $\red{?f}$ and some known function. 

This task is a hybrid instance of \textit{lifting problem} and \textit{partial lifting problem}, and some of the authors propose an efficient solver, \emph{AutoLifter}, for both problems in an independent submission to PLDI~\cite{lifting}\footnote{Based on our discussion with the program chair, we cite the other submission anonymously. To facilitate reviewing, we provide an anonymized version of the other submission in the supplementary material.}. In \mainname, {\it AutoLifter} is applied to solve this task. There are some details remaining on merging the results of partial lifting problems and listing problems, which are left to Section \ref{section:incre}.

\textit{AutoLifter} uses grammars to guarantee the efficiency of the synthesis results. Under its default setting, $\red{?f}$ is synthesized from a grammar including only polynomial-time programs that output only scalar values, and other functions are synthesized from a grammar including only constant-time operators. In this way, the time complexities of all synthesis results except $\red{?f}$ are guaranteed to be $O(1)$. In our transformation system, because $\red{?f}$ is a converting function and is invoked only once to process the instance, such a guarantee already ensures the efficiency of the transformation result. 

%Here we apply {\it AutoLifter} to solve these lifting problems.

%Then we need to solve synthesize tasks where the specification is an equation that involves the composition of two functions to be synthesized, and/or has one of the functions appearing in both sides of the equation. Such a synthesis problem is called a \emph{lifting problem}, and some of the authors propose an efficient solver, \emph{AutoLifter}, for this problem in an independent submission to PLDI~\cite{lifting}\footnote{Based on our discussion with the program chair, we cite the other submission anonymously. To facilitate reviewing, we provide an anonymized version of the other submission in the supplementary material.}. Here we apply {\it AutoLifter} to solve these lifting problems.

% Both of these two tasks are for applying \textit{incrementalization}. The unified characterization of these two tasks refers to functors in the category theory. Therefore, we leave it to Section \ref{section:trans} and illustrate the idea of \mainname using the specific task generated from $(P_4, S_4, m_4)$. 

% The task here is about rewriting queries $q_l = \lambda s. |s|$,  $q_h = \lambda s. (\textit{head}\ s)$, and modification $c_t = \lambda s. (\textit{tail}\ s)$. Given three set of examples $E_1, E_2, E_3$, the task is to find $\red{?f_s}, \red{?q_l}, \red{?q_h}$ and $\red{?c_t}$ satisfying the following conditions.
% \begin{gather*}
% \forall s \in E_1, \red{?q_l}\ (\red{?f_s}\ s) = q_l\ s \qquad 
% \forall s \in E_2, \red{?q_h}\ (\red{?f_s}\ s) = q_h\ s \\
% \forall s \in E_3, \red{?c_t}\ (\red{?f_s}\ s) = \red{?f_s}\ (c_t\ s)
% \end{gather*}

% First, the tasks for $q_l$ and $q_r$ are about synthesizing two functions from their composition. These tasks are instances of \textit{partial lifting problems} studied by \citet{lifting}. Therefore, \mainname invokes their approach, \textit{AutoLifter}, on these two tasks and thus gets a solution where $\red{?f_s} = \lambda s. |s|$, $\red{?q_l} = \lambda s. s$ and $\red{?q_h} = \lambda s. is[-s]$.

% To make this solution valid for the third task,  \mainname fixes $\red{?f_s}$ to $\red{?f_s}\ s \coloneq (f_s, \red{?f_s'})\ s$, where $f_s$ is $\lambda s. |s|$ found in the previous step. At this time, $\red{?f_s}$, $\red{?q_l} = \lambda s. (s.1)$ and $\red{?q_h} = \lambda s. is[-s.1]$ must be a solution for the first two tasks.

% Now, the remaining task is to synthesize $\red{?f_s'}$ and $\red{?c_t}$.
% $$\forall s \in E_3, \red{?c_t}\ (f_s\ s, \red{?f_s'}\ s) = (f_s\ (c_t\ s), \red{?f_s'}\ (c_t\ s))
% $$
% This task can be regarded as to make the calculation of $f_s$ incremental with respect to modification $c_t$ via $\red{?c_t}$ and $\red{?f_s'}$. Such a problem has also been studied by \citet{lifting} as \textit{lifting problems}. Therefore, \mainname invokes \textit{AutoLifter} again and thus gets a solution where $\red{?f_s'}$ is an empty program and $\red{?c_t} = \lambda s. (s.1 - 1)$. \mainname simplifies this solution by removing the empty component induced by $\red{?f_s'}$, resulting in the solution reported in Figure \ref{fig:overview}.

==> sections/Related.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Related Work} \label{section:related}
\noindent \textbf{Program Calculation}. \mainname is related to those studies for deriving dynamic programming in program calculation.

First, \citet{DBLP:conf/plilp/Moor95, DBLP:conf/flops/MorihataKO14,DBLP:conf/pepm/Mu08,DBLP:books/daglib/0096998} derives dynamic programming via \textit{thinning}. All of their approaches are manual and work only for a subclass of hylomorphism, namely \textit{sequential decision procedure}, where the search state is a recursive data structure and the anamorphism simply unfolds the structure of the state. \mainname generalizes \textit{thinning} to general hylomorphism and automates its application via program synthesis.

Second, \citet{DBLP:journals/lisp/LiuS03} uses \textit{incrementalization} and \textit{memoization} to derive dynamic programming from simple recursions, which is also a subclass of hylomorphism. Their approach is semi-automated and cannot generalize to general hylomorphism as it does not reduce the scale of the output, which can be exponential. \mainname applies to \textit{incrementalization} to program fragments in the hylomorphism and automates the application via program synthesis. 

Last, there are other approaches proposed for deriving dynamic programming~\cite{DBLP:conf/oopsla/PuBS11, DBLP:journals/scp/GiegerichMS04, DBLP:journals/csur/PettorossiP96, DBLP:conf/sigsoft/0003ML21, DBLP:conf/ppdp/SauthoffJG11}. Most of them are manual or semi-automated. The only automated approach we know is a transformation rule that automatically generates dynamic programming for a sequential decision procedure on lists when several conditions are satisfied~\cite{DBLP:conf/sigsoft/0003ML21}. However, the scope of this rule is narrow in contrast to hylomorphism: $27$ out of $37$ programs, accounting for $73.0\%$, in our dataset are not even sequential decision procedures.

\noindent \textbf{Program Synthesis}. There have been many synthesizers proposed for automatically synthesizing algorithms or efficient programs~\cite{DBLP:conf/pldi/SmithA16,DBLP:conf/pldi/MoritaMMHT07,toronto21,DBLP:conf/pldi/FedyukovichAB17,acar2005self,DBLP:conf/pldi/KnothWP019,DBLP:conf/cav/HuCDR21}, but none of them are for dynamic programming.

\mainname uses program synthesizers to (1) synthesize a keyword preorder from negative examples, and (2) synthesize program fragments for incrementalization. 

As discussed in Section \ref{section:incre}, \mainname solves the second task via our previous approach \textit{AutoLifter}~\cite{lifting}. Besides, \textit{AutoLifter} uses a method namely \textit{observational covering} to find a set of key functions covering a set of negative examples, which has a similar form to our first task. However, this method is applicable only when the set of examples is fixed and thus cannot be applied to our first task, where new negative examples will occur while adding key functions.

\mainname is related to \textit{Relish}~\cite{DBLP:journals/pacmpl/0001WD18}, a general solver for relational specifications. Both our tasks are instances of relational specifications and thus are in the scope of \textit{Relish}. However, because the \textit{Finite Tree Automata} used by \textit{Relish} does not directly support lambda expressions, \textit{Relish} cannot be applied to our grammar. 

\mainname is also related to the approach proposed by \citet{DBLP:conf/icfp/ZhangL98}, which is a deductive synthesizer for \textit{incrementalization}. However, this approach is available only when the input of queries includes only scalar values and thus cannot be applied to our second task, where the solutions (states) involve recursive data structure.

There are also many mainstream synthesizers for input-output specifications~\cite{DBLP:journals/pacmpl/JiS0H20, DBLP:conf/popl/Gulwani11, DBLP:conf/pldi/FeserCD15, DBLP:conf/pldi/OseraZ15, DBLP:conf/iclr/BalogGBNT17, DBLP:journals/pacmpl/WangDS18}. However, such specifications do not exist for either key functions in our first task or fragments in our second task, and thus all these synthesizers are unavailable.

==> sections/Synthesizer.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Synthesizer} \label{section:synthesizer}
\subsection{Preorder Synthesis} \label{section:psolver}
For the synthesis task of Steps 1 and 3, we start with a subproblem where a finite set of comparisons $C$ and a size limit $n_c$ are provided. In this subproblem, the search space of $\red{?R}$ is fixed to preorders constructed by $(\leq, o)$, which is necessary according to Theorem \ref{theorem:step1}, and at most $n_c$ comparisons in $C$.
\SetKwFunction{Search}{BestPreorder}
\SetKwFunction{CC}{CandidateComps}
\begin{algorithm}[t]
    \small
    \caption{Synthesizing preorder $\red{?R}$ for Step 1.}
    \KwIn{Input program $(h, o)$ for Step 1, a set of instances $I$, a set of comparisons $C = \{(op_i,k_i)\}$, and a size limit $n_c$.}
    \KwOut{A keyword preorder $\red{?R} \subseteq C$ for $(h, S)$.}
    \label{alg:preorder}
    \LinesNumbered
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{$\Search{$R, lim, \textit{costLim}$}$}{
        $es \gets \cup_{i \in I}CE(R, i)$; \\
        \lIf{$\textit{es} = \emptyset$}{\Return $R$} 
        \lIf{$lim = 0$}{\Return $\top$}
        $cList \gets \CC(C, lim, es)$; \\
        Sort $cList$ in the increasing order of $\textit{cost}(R \cup \{c\}, I)$; \\
        $\textit{res} \gets \bot$; \\
        \ForEach{$c \in cList$}{
            \lIf{$\textit{cost}(R \cup \{c\}, I) \geq \textit{costLim}$}{\textbf{continue}}
            $R' \gets \Search{$R \cup\{c\},lim-1, \textit{costLim}$}$; \\
            \lIf{$R' \neq \bot$}{$(\textit{res}, \textit{costLim}) \gets R', (\textit{cost}(R', I))$}
        }
        \Return $\textit{res}$;
    }
    \Return $\Search{$\{(\leq, o)\}, n_c, +\infty$}$;
\end{algorithm}

As shown in Algorithm \ref{alg:preorder}, \mainname solves this subproblem via \textit{branch-and-bound}. \Search decides comparisons used in $\red{?R}$ one by one with an upper bound on the cost (Lines 1-14). In each turn, a set of candidate comparisons is identified via $\CC$ (Line 5) and they are considered in the increasing order of the size (Line 6). For each comparison $c$, if its cost is smaller than the bound (Line 9), preorders including $c$ will be considered recursively (Line 10). Results of recursions will be used to update the bound (Line 11).

According to Lemma \ref{lemma:candidatecmp}, $\CC{$C, lim, es$}$ returns comparisons that satisfy at least $|es|/lim$ examples.

\begin{lemma}\label{lemma:candidatecmp} Given a set of instances $I$, for any two keyword preorders $R_1 \subseteq R_2$ where $\forall i \in I, CE(R_2, i) = \emptyset$, there exists a comparison $(op, k) \in R_2/R_1$ satisfying at least $1/(|R_2| - |R_1|)$ portion of examples in $CE(R_1, I) =\cup_{i \in I} CE(R_1, i)$, i.e., 
\begin{align*}
\left|\left\{(p_1, p_2)\in CE(R_1, I)\ \big|\ \neg \big((k\ p_1)op(k\ p_2)\big)\right\}\right| \geq  \frac{|CE(R_1, I)|}{|R_2|-|R_1|}\\
\end{align*}
\end{lemma}

There are several details remaining to make Algorithm \ref{alg:preorder} useful in \mainname. We describe these details below.

\noindent \textbf{Decide a finite set of comparisons}. In practice, the set of comparisons is usually provided by a grammar, in which the number of comparisons is infinite. Due to the difficulty of finding the optimal preorder from an infinite set of comparisons, \mainname approximates it via the principle of \textit{Occam's Razor}. Concretely, \mainname selects a parameter $s_c$ and takes the smallest $s_c$ comparisons in the grammar as set $C$. 

\noindent \textbf{Decide $s_c$ and $n_c$}. In practice, both $s_c$ and $n_c$ are not given. \mainname decides them iteratively with two parameters $s_c^*$ and $n_c^*$. In each turn, \mainname considers the subproblem where $n_c = n_c^*$ and  $s_c = s_c^*$. If there is no solution, $s_c^*$ will be doubled and $n_c^*$ will be increased by $1$ in the next iteration.

\noindent \textbf{Accelerate \CC}. A direct implementation of \CC{$C, lim, es$} in Algorithm \ref{alg:preorder} (Line 5) is to evaluate all comparisons in $C$ on all examples in $es$. Such an implementation is inefficient because both $C$ and $es$ can be large. \mainname improves this point by sampling. 

In \mainname, a comparison will be evaluated on all examples only when it satisfies $k_t = \lfloor lim/2 \rfloor$ examples among $lim \times n_t$ random examples, where $n_t$ is a parameter of \mainname. By Chernoff bound, the probability for a comparison that satisfies at least $1/lim$ portion of examples in $es$ to fail on this condition is at most $\exp(-n_t/8)$. Specially, $k_t$ is set to $lim \times n_t$, i.e., the number of samples, when $lim = 1$.

Note that though the sampling method may incorrectly exclude some comparisons, it does not affect the completeness %of the whole synthesizer 
as Algorithm \ref{alg:preorder} is wrapped in an iterator.

\noindent \textbf{Exclude redundant comparisons}. Each comparison $c$ that passes to the second stage of \CC will be evaluated on all examples. At this time, if there exists a comparison with a smaller range satisfying the same set of examples with $c$, $c$ will be excluded from $C$ as its effect is dominated.

Theorem \ref{theorem:complete} shows the completeness of \mainname while solving the synthesis task for Step 1.

\begin{theorem} \label{theorem:complete} Given program $(h, o)$, a set of instances $I$ and a grammar $G$ for available comparisons, if there exists a keyword preorder $R$ satisfying (1) $(\leq, o) \in R$, (2) $\forall i \in I, CE(R, i) = \emptyset$, and (3) $R$ is constructed by $(\leq, o)$ and comparisons in $G$, then \mainname must terminate and return such a keyword preorder.
\end{theorem}

\subsection{Synthesis Incrementalization} \label{section:incre}
To solve the synthesis task for Step 2 and Step 4, we first rewrite the condition for a query $q$ into Formula \ref{formula:si-query}
\begin{gather}
(q \circ id)\ e = (\red{?q[q]} \circ \F[q](\textit{null} \triangle \red{?f_p}))\ e \label{formula:si-query}
\end{gather}
where $id$ is the identity function, i.e., $\lambda x. x$, and $\textit{null}$ is a dummy function that outputs nothing.

Comparing with Definition \ref{def:lifting}, Formula \ref{formula:si-query} is the specification of partial lifting problem $\mathsf {PLP}(\{id\}, q, \textit{null}, \cup RE(q, i))$. Therefore, for each query $q$, \mainname invokes \textit{AutoLifter} to find a solution $(q[q], f_p[q])$ to Formula \ref{formula:si-query}.

Then, \mainname merges these results by fixing $\red{?f_p}$ to $f_q \triangle \red{?f_p'}$, where $f_q = \triangle_{q \in Q}f_p[q]$ and $Q$ represents the set of queries. For each query $q$, such a $\red{?f_p}$ and $q[q]$ can be converted into a solution to Formula \ref{formula:si-query} by adjusting the input type of $q[q]$. 

Next, we substitute $\red{?f_p}$ into the condition for constructors and rewrite the condition into Formula \ref{formula:si-mod}. 
\begin{gather}
\!\!\!\forall m \in M, ((f_q \triangle \red{?f_p'}) \circ m)\ e = (\red{?c[m]} \circ \F[m](f_q \triangle \red{?f_p}))\ e 
\label{formula:si-mod}
\end{gather}
where $M$ represents the set of constructors.

Comparing with Definition \ref{def:lifting} gain, Formula \ref{formula:si-mod} is the specification of lifting problem $\mathsf {LP}(M, f_p, f_p, E)$, where $E[m]$ is equal to $\cup RE(m, i)$. Therefore, the remaining part $\red{?f_p'}$ in $\red{?f_p}$ and $\red{?c}$ can be synthesized by invoking \textit{AutoLifter} again.

% \subsection{Synthesis Key Function}
% \mainname converts the task for Step 3 into the same form as Step 1 and then solves it by applying Algorithm \ref{alg:preorder}. 

% The conversion is based on the observation that $\red{?f_m}$ is usually in the form of $\red{?k_1} \triangle \dots \red{?k_n}$, where $\red{k_i}$ is some simpler key function. This is because the result of the generator is usually related to multiple attributes of the state.

% At this time, $\red{?f_m}$ can be regarded as keyword preorder $\{(=, k_i)_{i=1}^n\}$, and as shown below, examples in $ME(i)$ can be regarded as negative examples for the keyword preorder.
% $$
% \forall (s_1, s_2), (\red{?f_m}\ s_1 \neq \red{?f_m}\ s_2) \leftrightarrow \neg \left(\bigwedge_{i=1}^n k_i \ s_1 = k_i \ s_2 \right)
% $$
% Because the set of examples $ME(i)$ are fixed for all candidate $\red{?f_m}$, it is easy to verify Lemma \ref{lemma:monoce} also holds in Step 4.

% Based on the above correspondences, \mainname solves the synthesis task for Step 4 uniformly via Algorithm \ref{alg:preorder}.

\subsection{Properties of \mainname} \label{section:solver-property}
First, Theorem \ref{theorem:correct} guarantees the result of \mainname to be correct on all given instances. %Such a guarantee can be generalized to a probabilistic correctness guarantee on unseen instances via an iterative verification algorithm proposed by some of the authors~\cite{lifting}.

\begin{theorem} \label{theorem:correct} Given input program $(h, o)$ where $h$ is a relational hylomorphism and a set of instances $I$, let $p^*$ be the program synthesized by $\mainname$. Then $\forall i \in I$, $(h, o) \sim_i p^*$.
\end{theorem}

Second, Theorem \ref{theorem:efficiency} shows that under some assumptions, the program synthesized by \mainname is guaranteed to run in pseudo-polynomial time, which means that the time complexity is polynomial to the size and values in the input.

\begin{theorem} \label{theorem:efficiency} Given input program $(\hylo{\phi, \psi}_{\F}, o)$ and a grammar $G$ specifying the program space for synthesis tasks, the program synthesized by \mainname must be pseudo-polynomial time if the following assumptions are satisfied: (1) $\phi$, $\psi$ and programs in $G$ runs in pseudo-polynomial time, (2) each value and the size of each recursive data structure generated by the input program are pseudo-polynomial, (3) all operators in $G$ are linear, i.e., their outputs are bounded by a linear expression with respect to the input. 
\end{theorem}

==> sections/Transformation.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Transformation System} \label{section:trans}
The transformation system in \mainname converts the task of deriving efficient memoization to several simpler synthesis tasks for program fragments. As discussed in Section \ref{section:overview}, to simplify the specifications of the generated synthesis, both the transformation system and these synthesis tasks are based on examples. The examples for the transformation system is a set of concrete instances of the COP, and the examples for the synthesis task are extracted from the running procedure of the input hylomorphism on these instances.

\subsection{Notations for Running Procedure}
Given hylomorphism $h = \hylo{\psi, \phi}_{\mathsf F}: B \rightarrow \mathsf PA$, we use the following notations to record the running procedure of $h$.
\begin{itemize}[leftmargin=*]
\item $T_h: B \rightarrow \mathsf PB$ records direct recursions for $h\ s$ respectively. The definition of $T_h$ is shown as Equation \ref{equation:th}, where $\textit{ss}[\F]: \mathsf {F}B \rightarrow \mathsf PB$ is defined as the following.
\begin{gather*}
    \textit{ss}[\mathsf I]\ x \coloneq \{x\} \quad \textit{ss}[!A] \coloneqq \emptyset \quad \textit{ss}[\F_1 + \F_2]\ (i, x) \coloneqq \textit{ss}[\F_i]\ x \\
\textit{ss}[\F_1 \times \F_2]\ (x_1, x_2) \coloneqq (\textit{ss}[\F_1]\ x_1) \cup (\textit{ss}[\F_2]\ x_2)\\
\end{gather*}

\item $S_h: B \rightarrow \mathsf PB$ records all recursions (possibly indirect) for $h\ s$, which is the smallest arrow satisfying Equation \ref{equation:sh}.

{\centering \hspace{-9pt}
    \begin{minipage}{.46\linewidth}
    \begin{equation}
        T_h\ s \coloneqq \bigcup_{t \in (\psi s)} (\textit{ss}[\F]\ t) \label{equation:th}
    \end{equation} \qquad 
  \end{minipage}
  \begin{minipage}{.55\linewidth} \vspace {-5pt}
  \begin{equation}S_h\ s = \bigcup_{s' \in (T_h s)} (S_h\ s') \cup \{s\} \label{equation:sh}
  \end{equation}
\end{minipage}
}

\item $P_h: (B \times B \times A) \rightarrow \mathsf PA$ records the set of results that are constructed from some specific substate. Given state $s$, direct substate $s' \in (T_h\ s)$, and result $p \in (h\ s')$, for any invocation $(\phi\ sp)$ (Line 6 in Algorithm \ref{alg:hylo}) for transition $t$, $(\phi\ sp)$ is included in $P_h\ (s, s', p)$ if and only if $s'$ is used in $t$ and $p$ is used at the corresponding place in $sp$.  
\end{itemize}

\begin{example} Consider hylomorphism $h= \hylo{\phi, \psi}_{\mathsf F}$ in Figure \ref{fig:p1}, and instance $(is = [(3, 3), (2, 3), (1, 2)], W = 4)$. The following lists some results of the above notations.
\begin{itemize}[leftmargin=*]
\item $T_h\ is = \{is' = [(2, 3), (1, 2)]\}, T_H\ [] = \{\}$.
\item $S_h\ is = \{is, is', [(1, 2)], []\}, S_H\ [] = \{[]\}$.
\item $P_h\ (is, is', [(1, 2)]) = \{[(1, 2)], [(3, 3), (1, 2)]\}$.
\item $P_h\ (is, is', [(2, 3)]) = \{[(2, 3)]\}$.
\end{itemize}
\end{example}

\subsection{Synthesis Tasks}
The transformation system generates two types of synthesis tasks. We name them as \textit{preorder synthesis} ($\mathsf{PS}$) and \textit{incrementalization synthesis} ($\mathsf{IS}$) respectively. 

\begin{definition} An instance of \textit{preorder synthesis}, denoted as $\mathsf{PS}(R_0, g, E)$, is described by keyword preorder $R_0$ on object $A$, generator $g$ for negative examples, and set $E \subseteq A$. Generator $g$ is a function mapping keyword preorders on $A$ to $\mathsf P(A \times A)$, which satisfying the following two conditions.
\begin{itemize}[leftmargin=*]
\item (Counter-Negativity) $\forall (a, b) \in g\ R, aRb$.
\item (Monotonicity) $\forall R \subseteq R', (a,b) \in g\ R, aR'b \rightarrow (a, b) \in g\ R'$.
\end{itemize}
The task of $\mathsf {PS}(R_0, g, E)$ is to find a keyword preorder $\red{?R} \supseteq R_0$ such that (1) $g\ \red{?R} = \emptyset$, and (2) $N_\red{?R}(E)$ (introduced in Theorem \ref{theorem:thinning}) is minimized. \label{def:ps}
\end{definition}

The actual objective while synthesizing preorders is to minimize the number of objects returned by $\textit{thin}\ R$ in practice. In the definition of $\mathsf{PS}$, we have approximated this objective via $N_R(E)$ according to Theorem \ref{theorem:thinning}.

\begin{definition} An instance of $\textit{incrementalization synthesis}$, denoted as $\mathsf{IS}(A, Q, M, E)$ is described by object $A$, set $Q$ of queries, set $M$ of modifications and example space $E$, where $E[p]$ is a set of examples related to arrow $p \in Q \cup M$. For each arrow $p$ in $Q \cup M$, a functor $\mathsf F_p$ is attached.
\begin{itemize}[leftmargin=*]
\item For each query $p \in Q$, the input type is $\mathsf F_pA$.
\item For each modification $p \in M$, the signature is $\mathsf F_pA \rightarrow A$. 
\end{itemize}
The task of $\mathsf{IS}(A, Q, M, E)$ is to find $\red{?f}$, $\red{?q[p]}$ for each $p \in Q$ and $\red{?c[p]}$ for each $p \in M$ satisfying the following conditions.
\begin{gather*}
    \forall p \in Q, \forall e \in E[p], p\ e = (\red{?q[p]}\ \circ \mathsf F_p\red{?f})\ e \\
    \forall p \in M, \forall e \in E[p], (\red{?f} \circ p)\ e = (\red{?c[p]} \circ \mathsf F_p\red{?f})\ e
\end{gather*}
\end{definition}

\subsection{Step 1: Thinning}

Given program $(h = \hylo{\phi, \psi}_{\mathsf F}, S)$ and set $I$ of instances, \mainname generates task $\mathsf{PS}(R_0, g, E)$ in the following way.
\begin{itemize}[leftmargin=*]
\item $R_0$ is the key preorder of comparison $\{(\leq, S)\}$.
\item $g\ R$ is extracted from the running procedure of $P$ on instances in $I$. For each $i \in I$, each transition $(s, s')$ where $s \in (S_h\ i), s' \in (T_h\ i)$, and each pair of solutions $p_1, p_2 \in (h\ s')$, $(p_1, p_2)$ is included in $g\ R$ if the following formula is satisfied, which represented that (1) $p_1$ is smaller than $p_2$ in the sense of $R$, and (2) the solutions in $s$ constructed from $p_1$ is \textbf{not} dominated by that constructed from $p_2$.
$$p_1Rp_2 \wedge \big(\exists p_1' \in P_h\ (s, s', p_1), \forall p_2' \in P_h\ (s, s', p_2), \neg(p_1'Rp_2')\big)$$
\item $E$ includes all visited solutions when running $h$ on $I$.
$$
E = \bigcup_{i \in I} \bigcup_{s \in (S_h\ i)} (h\ i)
$$
\end{itemize}

Let $R$ be the preorder synthesized from task $\mathsf{PS}(R_0, g, E)$, \mainname returns program $(rg(\phi', \psi)_{\F}, S)$ as the result, where $\phi'$ is defined as $(\textit{thin}\ R) \circ \textit{cup} \circ \mathsf {P}\phi$.

\begin{lemma} Given program $(h, S)$ and set $I$ of instances, $\mathsf{PS}(R_0, g, E)$ constructed above is valid for preorder synthesis.
\end{lemma}

\begin{theorem} Given program $(h, S)$ and set $I$ of instances, let $r$ be the recursive generator synthesized in Step 1, then $(r, S)$ performs equally with $(h, S)$ on all instances in $I$.
    $$
    \forall i \in I, \big(\max (S\ p), p \in h\ i\big) =   \big(\max (S\ p), p \in r\ i\big)
    $$
\end{theorem}
\subsection{Step 2: Incrementalization for Plans}
After Step 1, the program must be in the following form.
$$(r = rg((\textit{thin}\ R) \circ \textit{cup}\circ \mathsf P \phi, \psi)_{\F}, S)$$
where $R$ is a keyword preorder and the body of $\phi$ and $\psi$ are statements in language $\mathcal L_H$ (Figure \ref{fig:syntax}).

Given such a program and set $I$ of instances, let $h$ be the corresponding hylomorphism $\hylo{\phi, \psi}_{\F}$. \mainname generate synthesis task $\mathsf{IP}(A, Q, M, E)$ in the following way. 

First, $A$ is the type of solutions generated by $r$. Concretely, let $B \rightarrow \mathsf PA'$ be the signature of $r$. Then $A$ is set to $A'$.

Second, For each key $k_i$ in $R$, $k_i$ is included in $Q$.
\begin{itemize}[leftmargin=*]
\item Functor $\F_{k_i}$ of $k_i$ is set to the constant functor $\mathsf I$.
\item Examples $E[k_i]$ includes all visited solutions when running program $r$ on $I$, i.e., $\cup_{i \in I} \cup_{s \in (S_h\ h)}(r\ s)$.
\end{itemize}

\SetKwFunction{ES}{ExtractS}
\SetKwFunction{EE}{ExtractE}
\SetKwFunction{Child}{Children}
\SetKwFunction{Insert}{Insert}
\begin{algorithm}[t]
    \small
    \caption{\small Extract queries and modifications from $\psi$.}
    \KwIn{A program $\phi = \lambda s. \phi_s$, where $p_s$ is a statement in $\mathcal L_H$.}
    \KwOut{A set of queries $Q$ and a set of modifications $M$.}
    \label{alg:extract}
    \LinesNumbered
    \SetKwProg{Fn}{Function}{:}{}
    $Q \gets \emptyset; \ \ M \gets \emptyset;$ \\
    \Fn{$\EE{$p_e$}$}{
        \lIf{$p_e = |s|$}{\Return \textit{true}}
        $\textit{related} \gets \textit{false}$; \\
        \ForEach{$sp_e \in \Child{$p_e, \mathbb E$}$}{
            $\textit{related} \gets \textit{related}\ \vee\  \EE{$sp_e$}$
        }
        \If{$\textit{related} \wedge \text{ the output of }p_e\text{ has a constant size}$}{
            $Q.\Insert{$p_e$}$;\ \ \Return \textit{false}; \\
        }
        \Return \textit{related};
    }
    \Fn{$\ES{$p_s$}$}{
        \If{$p_2 = |\text{collect}\ sp_e|$}{
            $M.\Insert{$sp_e$}$; \ \ \Return;
        }
        \ForEach{$sp_e \in \Child{$p_e, \mathbb E$}$}{
            \lIf{$\EE{$p_e$}$}{
                Extraction Failed
            }
        }    
        \ForEach{$sp_s \in \Child{$p_s, \mathbb S$}$}{
            \ES{$sp_s$};

        }   
    }
    $\ES{$\phi_s$}$; \\
    \Return $Q, M$; 
\end{algorithm}

\SetKwFunction{Construct}{C}
\begin{algorithm}[t]
    \small
    \caption{\small Construct example collector for a subprogram.}
    \KwIn{Program $\phi = \lambda s. \phi_s$ and a subprogram $sp$ of $\phi_s$. }
    \KwOut{A program collects examples for $sp$ from an instance.}
    \LinesNumbered
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{$\Construct{$p_s, sp$}$}{
        $t_1, \dots, t_n \gets $ temporary variables in $sp$; \\
        \lIf {$p_s = sp$}{\Return $|\text{collect}\ (s, t_1, \dots, t_n)|$}
        \ForEach{$sp_e \in \Child{$p_s, \mathbb E$}$}{
            \lIf {$sp \in sp_e$} {\Return $|\text{collect}\ (s, t_1, \dots, t_n)|$}
        }
        \Switch{$p_s$}{
            \Case{$|sp_{s, 1}\ sp_{s, 2}|$}{
                \lIf{$sp \in sp_{s, 1}$}{\Return \Construct{$sp_{s, 1}, sp$}}{\Return \Construct{$sp_{s, 2}, sp$};}
            }
            \Case{$|\text{if } sp_e\text{ then }sp_{s, 1}\text{ else }sp_{s, 2}|$}{
                \If{$sp \in sp_{s, 1}$}{\Return $|\text{if }sp_e\text{ then }\Construct{$sp_{s,1}, sp$}\text{ else skip;}|$}
                \Return $|\text{if }sp_e\text{ then skip; else }\Construct{$sp_{s,2}, sp$}|$;
            }
            \Case{$|\text{foreach }x \in sp_e\text{ in }sp_s|$}{
                \Return $|\text{foreach }x \in sp_e\text{ in }\Construct{$sp_s,sp$}|$;
            }
        }
    }
\end{algorithm}

Third, \mainname extracts queries and modifications from the body of $\psi$. Intuitively, queries in $\psi$ are those expressions that 

\subsection{Step 3: Compacting Memoization}

\subsection{Step 4: Incrementalization for States}

==> sections/Transformation2.tex <==
%!TEX root = ../DPSynthesis.tex
\section{Transformation System} \label{section:trans}
% The transformation system converts the task of deriving efficient memoization to synthesis tasks for program fragments. 
%As discussed in Section \ref{section:overview}, to simplify the specifications, both the system and synthesis tasks are based on examples. The examples for the system are a set of instances of the COP, and the examples for a synthesis task are extracted from the running procedure on these instances.

Given a recursive generator $r$ and a search state $s$, invoking $r$ on $s$ without memoization generates a search tree where each vertex corresponds to a search state. We use two notations $T_r$ and $S_r$ to access the structure of this tree, where $T_r\ s$ and $S_r\ s$ represent the set including all direct children of $s$ and the set including all states in the subtree of $s$ respectively. 
%In this section, we used two notations $T_r$ and $S_r$ to represent the relations between the search states generated by a given recursive generator $r = rg(\phi, \psi)_{\mathsf F}$.  
%\begin{itemize}[leftmargin=*]
%\item Given a search state $s$, $T_r\ s$ is defined as $\cup (ss[\F]\ t), t \in \psi\ s$, where $ss[\F]$ (defined as the following) extracts all components corresponding to functor $\mathsf I$ in $\mathsf F$ from $t$. Intuitively, $T_r\ s$ includes all children of state $s$ in the search tree.
%\begin{gather*}
%    \textit{ss}[\mathsf I]\ x \coloneq \{x\} \quad \textit{ss}[!A] \coloneqq \emptyset \quad \textit{ss}[\F_1 + \F_2]\ (i, x) \coloneqq \textit{ss}[\F_i]\ x \\
%\textit{ss}[\F_1 \times \F_2]\ (x_1, x_2) \coloneqq (\textit{ss}[\F_1]\ x_1) \cup (\textit{ss}[\F_2]\ x_2)\\
%\end{gather*}
%\item $S_r$ is the smallest fixed point of equation $S_r\ s = $
%\end{itemize}

%\subsection{Notations for Running Procedure}
%Given recursive generator $r = rg(\psi, \phi)_{\mathsf F}: B \rightarrow \mathsf PA$, we use the following notations to refer the running procedure of $r$.
%\begin{itemize}[leftmargin=*]
%\item $T_r: B \rightarrow \mathsf PB$, defined in Equation \ref{equation:th}, records direct substates for a given state $s$, where function $\textit{ss}$ defined as the following collects all substates from a transition.
%\begin{gather*}
%    \textit{ss}[\mathsf I]\ x \coloneq \{x\} \quad \textit{ss}[!A] \coloneqq \emptyset \quad \textit{ss}[\F_1 + \F_2]\ (i, x) \coloneqq \textit{ss}[\F_i]\ x \\
%\textit{ss}[\F_1 \times \F_2]\ (x_1, x_2) \coloneqq (\textit{ss}[\F_1]\ x_1) \cup (\textit{ss}[\F_2]\ x_2)\\
%\end{gather*}

%\item $S_r: B \rightarrow \mathsf PB$ records all substates (possibly indirect) for state $s$, which is the smallest arrow satisfying Equation \ref{equation:sh}.

%{\centering \hspace{-9pt}
%    \begin{minipage}{.46\linewidth}
%    \begin{equation}
%        T_r\ s \coloneqq \bigcup_{t \in (\psi\ \!s)} (\textit{ss}[\F]\ t) \label{equation:th}
%    \end{equation} \qquad 
%  \end{minipage}
%  \begin{minipage}{.55\linewidth} \vspace {-5pt}
%  \begin{equation}S_r\ s = \bigcup_{s' \in (T_r\ \!s)} (S_r\ s') \cup \{s\} \label{equation:sh}
%  \end{equation}
%\end{minipage}
%}
%\end{itemize}

%\begin{example} \label{example:notation}Consider hylomorphism $h= \hylo{\phi, \psi}_{\mathsf F}$ in Figure \ref{fig:p1}, and instance $(is = [(3, 3), (2, 3), (1, 2)], W = 4)$. The following lists some results of the above notations.
%    \begin{itemize}[leftmargin=*]
%\item $T_h\ is = \{is' = [(2, 3), (1, 2)]\}, T_H\ [] = \{\}$.
%\item $S_h\ is = \{is, is', [(1, 2)], []\}, S_H\ [] = \{[]\}$.
%\end{itemize}
%\end{example}

\subsection{Step 1: Thinning} \label{section:trans1}
Given program $(h = \hylo{\phi, \psi}_{\mathsf F}, o)$ and a set of instances $I$, \mainname returns a program in the following form while keeping the correctness on set $I$, where $\red{?R}$ is a keyword preorder.
\begin{align}(rg((\textit{thin}\ \red{?R}) \circ \textit{cup} \circ \mathsf P \phi, \psi)_{\F}, o)\label{form:step1}\end{align}

%\begin{example} Continuing Example \ref{example:notation}, the following are two examples of notation $NP(s, s', p)$.
%    \begin{itemize}[leftmargin=*]
%    \item $P_h\ (is, is', [(1, 2)]) = \{[(1, 2)], [(3, 3), (1, 2)]\}$.
%\item $P_h\ (is, is', [(2, 3)]) = \{[(2, 3)]\}$.
%   \end{itemize}
%\end{example}

First, Lemma \ref{theorem:step1} provides a sufficient condition for $\red{?R}$ to guarantee the correctness of the result. Recall that notation $p \twoheadrightarrow_s p'$ is introduced in Section \ref{section:overview} to represent that partial solution $p'$ in $(h\ s)$ is constructed from partial solution $p$.
\begin{lemma} \label{theorem:step1}Given instance $i$ and program $(h\!= \!\hylo{\phi, \psi}_{\F},o)$, $(rg((\textit{thin} \ \red{?R}) \circ \textit{cup} \circ \mathsf P \phi, \psi)_{\F}, o) \sim_i (\hylo{\phi, \psi}_{\F}, o)$ for keyword preorder $\red{?R}$ if $\red{?R}$ satisfies that (1) $(\leq, o) \in \red{?R}$, and (2) for each pair $(p_1, p_2)$ of partial solutions generated from the same invocation of $h$, $p_1\red{?R}p_2$ implies that $p_1$ is dominated by $p_2$ in the sense of $R$ when constructing new solutions, i.e.,
\begin{align}
\forall s \in (S_h\ i), \forall s' \in (T_h\ s), \forall p_1, p_2 \in (h\ s'), p_1\red{?R}p_2 \rightarrow& \nonumber \\
\forall p_1', \big(p_1 \twoheadrightarrow_s p_1' \rightarrow \exists p_2', p_2 \twoheadrightarrow_s p_2' \wedge p_1' \red{?R} p_2'\big)& \label{equation:ce} 
\end{align}
\end{lemma}

Given a preorder $R$ and an instance $i$, a set of counterexamples $CE(R, i)$ can be extracted via Lemma \ref{theorem:step1}, which includes all pairs of partial solutions $(p_1, p_2)$ that violates Equation \ref{equation:ce}. Note that $CE(R, i)$ changes with the choice of $R$.

 Lemma \ref{lemma:monoce} shows that to find a correct keyword preorder $R_2$ by enlarging a keyword preorder $R_1$, all counterexamples of $R_1$ must be rejected by new comparisons in $R_2$.

\begin{lemma}\label{lemma:monoce} Given instance $i$, for any two keyword preorders $R_1 \subseteq R_2$, the following formula is always satisfied.
    $$
    \forall (p_1, p_2) \in CE(R_1, i), (p_1, p_2) \notin CE(R_2, i) \leftrightarrow \neg p_1(R_2/R_1) p_2
    $$
where $R_2/R_1$ represents the keyword preorder formed by the new comparisons in $R_2$ compared with $R_1$.
\end{lemma}

Second, for efficiency of the result, the number of plans returned by $(\textit{thin}\ \red{?R})$ and its time cost should be minimized. By Theorem \ref{theorem:thinning}, \mainname defines this cost as the following.
\begin{equation*}
\textit{cost}(\red{?R}, I) \coloneqq N_{\red{?R}}(P), \quad P = \big\{p\big|i \in I, s \in S_h\ i, p \in h\ s\big\} 
\end{equation*}
where $P$ represents all partial solutions related to set $I$.

In summary, the task for Step 1 is to synthesize a keyword preorder $\red{?R}$ satisfying the following requirement. 
\begin{itemize}[leftmargin=*]
\item (Correctness) $(\leq, o) \in R$ and $\forall i \in I, CE(\red{?R}, i) = \emptyset$.
\item (Efficiency) $\textit{cost}(\red{?R}, I)$ is minimized.
\end{itemize}

\subsection{Step 2: Incrementalization for Plans} \label{subsection:rule1}
The initial program for Step 2 is in Form \ref{form:step1}, where the body of $\phi$ and $\psi$ are statements ($\mathbb S$) in language $\mathcal L_H$ (Figure \ref{fig:syntax}).

\mainname performs Step 2 only when the partial solutions generated by $\phi$ includes recursive data structures such as lists and trees. Concretely, \mainname constructs a program $\textit{prog}_2'$ that performs almost the same with $\textit{prog}_2$ except each partial solution $p$ in $\textit{prog}_2$ is stored as $\red{?f_p}\ p$, where the output of $\red{?f_p}$ is limited to a tuple of scalar values. The construction rewrites two types of solution-related functions in $\textit{prog}_2$.
\begin{itemize}[leftmargin=*]
\item Queries, which returns a tuple of scalar values.
\item Constructors, which constructs a new partial solution.
\end{itemize}

The following shows the content of $\textit{prog}_2'$.
\begin{equation}
\textit{prog}_2' = (rg((\textit{thin}\ R') \circ \textit{cup}\circ \mathsf P \phi', \psi)_{\F}, \red{?q[o]}) \label{form:prog2new}
\end{equation}
\begin{itemize}[leftmargin=*]
\item Both $o$ and keywords in $\red{?R}$ are queries. In $\textit{prog}_2'$, $o$ and $R$ are replaced with $\red{?q[o]}$ and $R' = \{(op, \red{?q[k]})\ |\ (op, k) \in R\}$.
\item Constructors and other queries are extracted from $\phi$. In $\textit{prog}_2'$, $\phi$ is replaced with function $\phi'$ constructed from $\phi$.
\end{itemize}
\SetKwFunction{ES}{RewriteS}
\SetKwFunction{EE}{RewriteE}
\SetKwFunction{Child}{Children}
\SetKwFunction{Insert}{Insert}
\SetKwFunction{Rewrite}{Clone}
\begin{algorithm}[t]
    \small
    \caption{ Construct $\phi'$ from $\phi$.}
    \KwIn{A program $\phi = \lambda s. \phi_s$, where $p_s$ is a statement in $\mathcal L_H$.}
    \KwOut{Queries $Q$, Constructors $M$, and $\phi'$ in $\textit{prog}_2$.}
    \label{alg:extract}
    \LinesNumbered
    \SetKwProg{Fn}{Function}{:}{}
    $Q \gets \emptyset; \ \ M \gets \emptyset;$ \\
    \Fn{$\EE{$p_e$}$}{
        \lIf{$|s| \notin p_e$}{\Return $p_e$}
        \lIf{$p_e = |s|$}{\Return $\bot$}
        $sp_e' \gets \{\EE{$sp_e$}\ |\ sp_e \in \Child{$p_s, \mathbb E$}\}$; \\
        \If{$\bot \in sp_e'$}{
            \If{$p_e$ output a tuple of scalar values}{
            $t_1, \dots, t_m \gets $ temporary variables in $p_e$; \\
            $Q.\Insert{$p_e$}$;\ \ \Return $|\red{?q[p_e]}\ (s, t_1, \dots, t_m)|$; 
            }
            \Return $\bot$;
        }
        \Return \Rewrite{$p_e, sp_e'$};
    }
    \Fn{$\ES{$p_s$}$}{
        \If{$p_2 = |\text{collect}\ sp_e|$}{
            $t_1, \dots, t_n \gets$ temporary variables in $p_s$; \\
            $M.\Insert{$sp_e$}$; \ \ \Return $|\red{?c[p_s]}\ (s, t_1, \dots, t_n)|$;
        }
        $sp_e' \gets [\EE{$sp_e$}\ |\ sp_e \in \Child{$p_s, \mathbb E$}]$; \\
        $sp_s' \gets [\ES{$sp_s$}\ |\ sp_e \in \Child{$p_s, \mathbb S$}]$; \\
        \Return \Rewrite{$p_s, sp_e' \cat sp_s'$}.
    }
    $\phi'_s \gets \ES{$\phi_s$}$;\ \ \Return $Q, M, \lambda s. \phi'_s$;
\end{algorithm}

$\phi'$ is constructed via a structural recursion on the AST of $\phi$. This procedure is shown as Algorithm \ref{alg:extract}.
\begin{itemize}[leftmargin=*]
\item $|s|$ corresponds to the input variable of $\phi$.
%\item We use $|p|$ to denote an expression $p$ in language $\mathcal L_H$, and $|s|$ corresponds to the input variable of $\phi$. 
\item \EE and \ES corresponds to non-terminal $\mathbb E$ and $\mathbb S$ in $\mathcal L_H$ respectively. Specially, $\EE$ returns $\bot$ if the current expression in $\textit{prog}_2$ is inside a query.
\item $\Child{$p, \mathbb N$}$ returns all children of AST node $p$ corresponding to non-terminal $\mathbb N$, and $\Rewrite{$p, c$}$ constructs a new AST node by replaces the children of $p$ with list $c$.
\end{itemize}

To characterize the specification of $\red{?f_p}, \red{?q}$ and $\red{?c}$, we introduce two notations $\F[p]$ and $E(p, i)$.
\begin{itemize}[leftmargin=*]
\item For each query (or constructor) $p$, functor $\F[p]$ indicates partial solutions in the input of $p$. For queries extracted from $R$ and $S$, $\F[p] \coloneqq \mathsf I$; For functions extracted from $\phi$, $\F[p] \coloneqq \F \times !T_1 \times \dots !T_n$, where $\F$ is the functor in $\textit{prog}_2$ and $!T_i$ is the type of the $i$th temporary variable used by $p$. 
\item Given instance $i$, for each query (or constructor) $p$, set $RE(p, i)$ records the inputs on which $p$ is invoked during $(\textit{prog}_2\ i)$, which can be obtained by instrumenting $\textit{prog}_2$.
\end{itemize} 

Lemma \ref{theorem:step2} provides a sufficient condition for $\red{?f_p}, \red{?q}$ and $\red{?c}$ to guarantee the correctness of $\textit{prog}_2'$. 

\begin{lemma}\label{theorem:step2} Given instance $i$ and program $\textit{prog}_2$ in Form \ref{form:step1}, let $\textit{prog}_2'$ be the program constructed by \mainname in Step 2. $\textit{prog}_2 \sim_i \textit{prog}_2'$ if for any query $q$ and any constructor $m$, Formula \ref{formula:2q} and Formula \ref{formula:2m} are satisfied respectively.
\begin{gather}
    \forall e \in RE(q, i), q\ e = \red{?q[q]}\ (\mathsf F[q]\red{?f_p}\ e)  \label{formula:2q}\\
    \forall e \in RE(m, i), \red{?f_p}\ (m\ e) = \red{?c[m]}\ (\F[m]\red{?f_p}\ e)   \label{formula:2m}
\end{gather}
\end{lemma}

In summary, the synthesis task for Step 2 is to find $\red{?f_p}, \red{?q}$ and $\red{?c}$ satisfying the following two requirements.
\begin{itemize}[leftmargin=*]
\item (Correctness) Lemma \ref{theorem:step2} is satisfied for any $i \in I$. 
\item (Efficiency) The output of $\red{?f_p}$ is a tuple of scalar values.
\end{itemize}

\subsection{Step 3: Memoization} \label{section:trans3}
In Step 3, given program $(r, o)$, where $r$ is a recursive generator, and a set of instances $I$, \mainname returns $(r^{\red{?f_m}}, o)$, i.e., memoizes $r$, while keeping the correctness on set $I$.

For the correctness, Lemma \ref{theorem:step3} provides a sufficient condition for $\red{?f_m}$ to guarantee the correctness of $(r^{\red{?f_m}}, o)$.

\begin{lemma}\label{theorem:step3} Given instance $i$ and program $(r, o)$, where $r$ is a recursive generator, $(r^{\red{?f_m}}, o) \sim_i (r, o)$ if for any two states $s_1, s_2 \in (S_r\ i)$, $(\red{?f_m}\ s_1 = \red{?f_m}\ s_2) \rightarrow (r\ s_1 = r\ s_2)$.
\end{lemma}

Given an instance $i$, a set of examples $EM(i)$ can be extracted according to Lemma \ref{theorem:step3}. Each example in $EM(i)$ is a set of states $(s_1, s_2)$, representing that $\red{?f_m}$ should output differently on these two states.

For efficiency, the number of stored results, which is the number of different outputs produced by $\red{?f_m}$, should be minimized. This objective leads to a cost function for $\red{?f_m}$.
$$
\textit{cost}(\red{?f_m}, I) \coloneqq \big|\left \{\red{?f_m}\ s\ \big|\ i \in I, s \in (S_r\ i) \right\} \big|
$$

In summary, the synthesis task of Step 3 is to find $\red{?f_m}$ satisfying the following two requirements.
\begin{itemize}[leftmargin=*]
\item (Correctness) $\forall i \in I, \forall (s_1, s_2) \in EM(i)$, $\red{?f_m}\ s_1 \neq \red{?f_m}\ s_2$.
\item (Efficiency) $\textit{cost}(\red{?f_m}, I)$ is minimized.
\end{itemize}
 
\subsection{Step 4: Incrementalization for States}
After Step 3, the program must be in the following form.
$$
\textit{prog}_4 = (r, o), \quad  r = rg\big((\textit{thin}\ R) \circ \textit{cup} \circ \mathsf P\phi, \psi\big)_{\F}^{f_m}
$$ 
where the body of $\phi$ and $\psi$ are statements ($\mathbb S$) in $\mathcal L_H$.

\mainname performs Step 4 only when the type of states includes recursive data structures. Similar to Step 2, \mainname rewrites all state-related queries and constructors in $\textit{prog}_4$ with $\red{?q}$ and $\red{?c}$ respectively, and thus constructs a program $\textit{prog}_{4}'$ that performs almost the same with $\textit{prog}_4$ except each state $s$ in $\textit{prog}_4$ is stored as $\red{?f_s}\ s$. To guarantee the efficiency, the output of $\red{?f_s}$ is limited to a tuple of scalar values. 

In $\textit{prog}_4$, key function $f_m$ is identified as a query. Other queries and constructors are extracted from $\psi$ similarly with Algorithm \ref{alg:extract}. The only difference is that in $\psi$, the parameter $sp_e$ of $|\textit{collect}\ sp_e|$ is a structure including substates, on which $r$ will be recursively applied, and decision values, which will be directly passed to $\phi$. Because $\F$ is a polynomial functor, these components can be extracted from $sp_e$ via the access operator, i.e., $|sp_e.i_1.i_2\dots i_n|$. Those components corresponding to substates and decision values are identified as constructors and queries respectively. 

We omit the specification of $\red{?f_s}, \red{?q}, \red{?c}$ and the synthesis tasks here because they are almost the same as Step 2.
